A general and sharp regularity condition for integro-differential equations with non-dominated measures

The aim of this work is to present the regularity condition (also known in the literature as structure condition) an integro-differential operator may satisfy in order for the domination principle to hold for (sub-,super-) solutions of polynomial growth. More precisely, the framework presented in Hollender [13], in which power functions are used in order to determine the integrability conditions, is weakened by substituting the power functions with Young functions. The use of Young functions allows for sharp integrability conditions, which are crucial when one deals with limit theorems. As an immediate application, it is considered the case of parabolic Hamilton-Jacobi-Bellman (HJB) operators, for which the regularity condition is satisfied and, consequently, the comparison principle as well. The parabolic HJB operator presented in this work can be associated to second-order (decoupled) forward-backward stochastic differential equations with jumps.

==> Auxiliary_lemmata_HJB_Regularity_Condition.tex <==
%!TEX root = main.tex

We are now ready to prove the lemmata mentioned in the proof of \cref{HJB:Regularity_Condition}. 

\begin{lemma}\label{lemma_appendix:regularity_f_nonlinearities}
Under the framework of \cref{HJB:Regularity_Condition} and given the introduced notation \eqref{def:penalization_function}-\eqref{def:delta_x_phi}, \eqref{def:A_epsilon} and assumptions \eqref{supremum_penalized}-\eqref{reg_cond:assumption_ineq} of the proof of \cref{HJB:Regularity_Condition}, it holds 
\begin{align*}
    &\begin{multlined}[c][0.9\textwidth]
    \sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}} \Big\{ 
        f_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\bar{x}), \sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}))\\
        - f_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\bar{y}),-\sigma^T_\alpha(\bar{t},y) D_y\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\bar{x},\cdot)\circ\tau_{\bar{y}-y})) 
        \Big\}  
    \end{multlined}\\
    &\hspace{2em}\le 
    \overline{\omega}_{{}_R}\big( |\bar{x} - \bar{y}| \big) 
    +\lambda C_{\ell,m} |\bar{x}-\bar{y}|^2
    +\gamma e^{\mu \bar{t}} C_{p,T, \Upsilon,\sigma,m,\ell}
        \big\{1 + \big[\Upsilon(|\bar{x}|^p)+\Upsilon(|\bar{y}|^p)\big] \big\}
    +     \varrho^1_{\gamma,\lambda,\varepsilon,\kappa},
\end{align*}
with 
    \begin{align*}
    % \limsup_{\gamma\downarrow 0}
    \limsup_{\lambda\to +\infty}
    \limsup_{\varepsilon \downarrow 0} 
    \limsup_{\kappa \downarrow 0} 
    \varrho^1_{\gamma,\lambda,\varepsilon,\kappa} = 0,
    \end{align*}
for some non-negative constants which may depend on $p, T, \Upsilon$ and the families $\{\sigma_{\alpha}\}_{\alpha\in\mathcal{A}}$, $\{\ell_{\alpha}\}_{\alpha\in\mathcal{A}}$ and $\{m_{\alpha}\}_{\alpha\in\mathcal{A}}$.
\end{lemma}


\begin{proof}
For the closed ball of radius $R=R(\gamma)$ assumed in \cref{rem_append:aux_properties}.\ref{regularity_aux_remark:limsup_lambda_varepsilon_barx_bary} and for $0< \varepsilon\leq \varepsilon_0$
  \begin{align*}
    &\begin{multlined}[c][\textwidth]
    \sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}} \Big\{ 
        f_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\bar{x}), \sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}))\\
        - f_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\bar{y}),-\sigma^T_\alpha(\bar{t},y) D_y\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y},-\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\bar{x},\cdot)\circ\tau_{\bar{y}-y})) 
        \Big\}  
    \end{multlined}\\
    &\begin{multlined}[c][\textwidth]
    =
    % \overset{\phantom{\text{\ref{HJB:monotonicity}.\ref{HJB:monotonicity_2}}}}{\underset{\phantom{\text{\eqref{gradient_penalized_y}}}}{=}}
    \sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}} \Big\{ 
        f_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\bar{x}), \sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}))\\
        -f_\alpha(\bar{t},x,v_\varepsilon(\bar{t},\bar{y}), \sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}))\\
        +f_\alpha(\bar{t},x,v_\varepsilon(\bar{t},\bar{y}), \sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}))\\
        -f_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\bar{y}), \sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}))\\
        +f_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\bar{y}), \sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}))\\
        - f_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\bar{y}),-\sigma^T_\alpha(\bar{t},y) D_y\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y},-\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\bar{x},\cdot)\circ\tau_{\bar{y}-y})) 
        \Big\}
    \end{multlined}\\
    &\begin{multlined}[c][\textwidth]
    \leq
    % \overset{\phantom{\text{\ref{HJB:monotonicity}.\ref{HJB:monotonicity_2}}}}{\underset{\phantom{\text{\eqref{gradient_penalized_y}}}}{\le}} 
    \sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}}\Big\{ 
      \overline{\omega}_{{}_R}\big(|x-y|(1+|\sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}) |)\big)
      \\ 
      + C |\sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}) +\sigma^T_\alpha(\bar{t},y) D_y\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}) |
      \\
      +C \Big[ \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}) 
          -\mathcal{K}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y},-\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\bar{x},\cdot)\circ\tau_{\bar{y}-y})\Big]^+
      \Big\}  
    \end{multlined}
    \\
    &
    \begin{multlined}[0.9\textwidth]
    \leq
    % \overset{\phantom{\text{\ref{HJB:monotonicity}.\ref{HJB:monotonicity_2}}}}{\underset{\phantom{\text{\eqref{gradient_penalized_y}}}}{\le}} 
    \sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}} 
        \overline{\omega}_{{}_R}\big(
        |x-y|(1+|\sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}) |)
        \big)
        \\ 
    + 
    \sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}}\big\{
        |\sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}) +\sigma^T_\alpha(\bar{t},y) D_y\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}) |
        \big\}    
        \\
    +\sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}}\Big\{
        \big[ \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x})\\ 
                        -\mathcal{K}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y},-\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\bar{x},\cdot)\circ\tau_{\bar{y}-y})\big]^+\Big\},
    \end{multlined}
        \numberthis\label{HJB:reg_cond_nonlinearities_aux_part_a}
  \end{align*}
where we omitted the constants for notational simplicity, since this will cause no harm later when limits will be evaluated.
In the first inequality it was utilized the fact that $u^{\varepsilon}(\bar{t},\bar{x}) - v_{\varepsilon}(\bar{t},\bar{y}) \ge 0$, see \eqref{supremum_penalized}, in conjunction with the monotonicity assumed in the second spatial variable; see \ref{HJB:monotonicity}.\ref{HJB:monotonicity_2}.
  Additionally, it was used the continuity assumptions \ref{HJB:coef_continuity} and \ref{HJB:monotonicity}.\ref{HJB:monotonicity_1}.
  Also, the positive part appears because of the monotonicity of the non-linearities $f_\alpha$ in their last argument; see \ref{HJB:monotonicity}.\ref{HJB:monotonicity_2}.

  Let us, now, separately consider each summand of \eqref{HJB:reg_cond_nonlinearities_aux_part_a}:
  % \begin{enumerate}[label=\textbullet]
  % \item

\textbullet\hspace{0.3em}
 For the first summand of \eqref{HJB:reg_cond_nonlinearities_aux_part_a} we have
    \begin{align*}
      &\sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}}\Big\{ 
      \overline{\omega}_{{}_R}\big(|x-y|(1+|\sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}) |)\big)
      \\
      &\hspace{0.7em}
      \overset{\eqref{gradient_penalized_x}}{\underset{\eqref{gradient_penalized_y}}{\le}}
      \sup_{(a,x,y)\in\mathcal{A}_{\varepsilon}} 
      \overline{\omega}_{{}_R}\big(
      (
      |x- y|
      )(
      1+ [2\lambda |\bar{x}-\bar{y} | + p\gamma e^{\mu \bar{t}} \Upsilon'(|\bar{x}|^p) |\bar{x} |^{p-1}]\times |\sigma_\alpha(\bar{t},x)|  
      )
      \big)\\
      &\hspace{0.5em}
      \begin{multlined}[0.9\textwidth]
      \overset{\eqref{bound:norm_x_y}}{\underset{\ref{HJB:coef_continuity}}{\le}} 
      \sup_{(a,x,y)\in\mathcal{A}_{\varepsilon}} 
      \overline{\omega}_{{}_R}\big(
      |\bar{x} - \bar{y}|
      + 2^{(\frac{p}{2}\vee1)-1}
      \varepsilon^{\frac12} 
      (\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}
      \big)
      \\
      %
      +
      \sup_{(a,x,y)\in\mathcal{A}_{\varepsilon}} 
      \overline{\omega}_{{}_R}\big(
      \big[
      |\bar{x}-\bar{y}| + 2^{(\frac{p}{2}\vee1)-1}
      \varepsilon^{\frac12} 
      (\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}
      \big]
      2\lambda |\bar{x}-\bar{y} | \times[ |\sigma_\alpha(\bar{t},\bar{x})| + C|x - \bar{x}| ]
      \big)
      \\
      %
      +
      \sup_{(a,x,y)\in\mathcal{A}_{\varepsilon}} 
      \overline{\omega}_{{}_R}\big(
      \big[
      |\bar{x}-\bar{y}| 
      +2^{(\frac{p}{2}\vee1)-1}
      \varepsilon^{\frac12} 
      (\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}
      \big]
      p\gamma e^{\mu \bar{t}} \Upsilon'(|\bar{x}|^p) |\bar{x} |^{p-1} [ |\sigma_\alpha(\bar{t},\bar{x})| + C|x - \bar{x}| ]
      \big)
      \end{multlined}
      \\
      &\hspace{0.5em}
      \overset{\eqref{ineq:norm_to_delta}}{\underset{\phantom{\ref{HJB:coef_continuity}}}{\leq }} 
      \overline{\omega}_{{}_R}\big( |\bar{x} - \bar{y}| \big) 
      + \bar{\varrho}^1_{\gamma,\lambda,\varepsilon},
      \numberthis
      \label{lem_app:f_nonlinearities_first}
    \end{align*}
    where 
    \begin{multline*}
    \bar{\varrho}^1_{\gamma,\lambda,\varepsilon}:=
    \overline{\omega}_{{}_R}\big(
    2^{(\frac{p}{2}\vee 1)-1}
    \varepsilon^{\frac{1}{2}} (\delta(\bar{x})^{\frac{1}{2}} + \delta(\bar{y})^{\frac{1}{2}})
    \big)
    \\
    %
    +
    \overline{\omega}_{{}_R}\big(
    [
    |\bar{x}-\bar{y}| + 2^{(\frac{p}{2}\vee 1)-1}\varepsilon^{\frac{1}{2}} (\delta(\bar{x})^{\frac{1}{2}} + \delta(\bar{y})^{\frac{1}{2}})
    ]
    2\lambda |\bar{x}-\bar{y} | \times
    [ |\sigma_\alpha(\bar{t},\bar{x})| 
    + C2^{(\frac{p}{2}\vee 1)-1}\varepsilon^{\frac{1}{2}} \delta(\bar{x})^{\frac{1}{2}} ]
    \big)
    \\
    %
    +
    \overline{\omega}_{{}_R}\big(
    [|\bar{x}-\bar{y}| + 2^{(\frac{p}{2}\vee 1)-1}\varepsilon^{\frac{1}{2}} (\delta(\bar{x})^{\frac{1}{2}} + \delta(\bar{y})^{\frac{1}{2}})]
    p\gamma e^{\mu \bar{t}} \Upsilon'(|\bar{x}|^p) |\bar{x} |^{p-1} 
    [ |\sigma_\alpha(\bar{t},\bar{x})| 
    + C 2^{(\frac{p}{2}\vee 1)-1}\varepsilon^{\frac{1}{2}} \delta(\bar{x})^{\frac{1}{2}} ]
    \big)
    \end{multline*}
    with 
    \begin{align}
    % \limsup_{\gamma\downarrow 0}
    \limsup_{\lambda\to +\infty}
    \limsup_{\varepsilon \downarrow 0} 
    \bar{\varrho}^1_{\gamma,\lambda,\varepsilon} = 0.
    \label{limsup_lambda_epsilon_bar_rho_1}
    \end{align}
    Before we argue about the validity of \eqref{limsup_lambda_epsilon_bar_rho_1}, we underline that in the extraction of \eqref{lem_app:f_nonlinearities_first} we used that every modulus of continuity has been assumed to be increasing, continuous and subadditive.
% 
    We argue now about the validity of \eqref{limsup_lambda_epsilon_bar_rho_1}.
    Given \cref{rem_append:aux_properties}.\ref{regularity_aux_remark:limsup_lambda_varepsilon_barx_bary} we have that 
    % \begin{align}
    % \end{align}
    \begin{align*}
    \limsup_{\varepsilon\downarrow 0}\bar{\varrho}^1_{\gamma,\lambda,\varepsilon} = 
    \overline{\omega}_{{}_R}\big(
    2\lambda |\hat{x}-\hat{y} |^2  |\sigma_\alpha(\hat{t},\hat{x})|
    \big)
    %
    +
    \overline{\omega}_{{}_R}\big(
    |\hat{x}-\hat{y}|
    p\gamma e^{\mu \hat{t}} \Upsilon'(|\hat{x}|^p) |\hat{x} |^{p-1} 
    |\sigma_\alpha(\hat{t},\hat{x})| 
    \big),
    \end{align*}
    for some limit point $(\hat{t}(\gamma,\lambda),\hat{x}(\gamma,\lambda),\hat{y}(\gamma,\lambda))$ of the family $(\bar{t}(\gamma,\lambda,\varepsilon),\bar{x}(\gamma,\lambda,\varepsilon),\bar{y}(\gamma,\lambda,\varepsilon))_{\varepsilon\in(0,\varepsilon_0]}$.
    Arguing analogously to \eqref{regularity_aux_remark:sigma_bound} for a convergent sequence 
    $(\hat{t}(\gamma,\lambda_n),\hat{x}(\gamma,\lambda_n),\hat{y}(\gamma,\lambda_n))$ and using \eqref{limsup_lambda_limit_point} we conclude the desired property \eqref{limsup_lambda_epsilon_bar_rho_1}.
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 

    % \item 
\textbullet\hspace{0.3em}
    For the second summand of \eqref{HJB:reg_cond_nonlinearities_aux_part_a}, using \eqref{gradient_penalized_x}, \eqref{gradient_penalized_y} and \ref{HJB:coef_continuity},  we have
    \begin{align*}
      &\sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}}
      \big\{
        |\sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}) +\sigma^T_\alpha(\bar{t},y) D_y\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}) | 
        \big\}\\
      &\hspace{1em} \overset{\phantom{\text{\eqref{ineq:norm_to_delta}}}}{\leq}
        \sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}}
        \big\{
          2\lambda C|\bar{x}-\bar{y}|\times |x-y|
          +p\gamma e^{\mu \bar{t}}\big[\Upsilon'(|\bar{x}|^p) |\bar{x}|^{p-2} |\sigma^T_\alpha(\bar{t},x) \bar{x}| 
          +\Upsilon'(|\bar{y}|^p) |\bar{y}|^{p-2} |\sigma^T_\alpha(\bar{t},y) \bar{y}| \big] 
        \big\}\\
      &\hspace{1em}
      \begin{multlined}[0.88\textwidth]
        \overset{\eqref{bound:norm_x_y}}{\underset{\ref{HJB:coef_continuity}}{\leq}}
        2\lambda C |\bar{x}-\bar{y}|^2
        +
        2^{(\frac{p}{2}\vee 1)} 
        \varepsilon^{\frac 12}
        \lambda C |\bar{x}-\bar{y}|
        (
        \delta(\bar{x})^{\frac{1}{2}} + \delta(\bar{y})^{\frac{1}{2}}
        )
        \\
        +
        p\gamma e^{\mu \bar{t}}
        \big\{
          \big[\Upsilon'(|\bar{x}|^p) |\bar{x}|^{p-1} 
          +\Upsilon'(|\bar{y}|^p) |\bar{y}|^{p-1}  \big] 
        \big\}
        \sup_{\alpha\in\mathcal{A}} |\sigma_\alpha(\bar{t},0)|
        \\
        +
        2^{(\frac {p}{2}\vee 1)-1}
        \varepsilon^{\frac12}
        p\gamma e^{\mu \bar{t}}
          \big[\Upsilon'(|\bar{x}|^p) |\bar{x}|^{p-1} \delta(\bar{x}) 
          +\Upsilon'(|\bar{y}|^p) |\bar{y}|^{p-1} \delta(\bar{y}) \big] 
        \\
        +
        p\gamma e^{\mu \bar{t}}
        \big\{
          \big[\Upsilon'(|\bar{x}|^p) |\bar{x}|^{p} 
          +\Upsilon'(|\bar{y}|^p) |\bar{y}|^{p} \big] 
        \big\}
      \end{multlined}\\
      &\hspace{1em}
      \begin{multlined}[0.88\textwidth]
        \overset{\text{\eqref{reg_cond:Upsilon_moderate}}}{\underset{\ref{HJB:coeff_boundedness}}{\leq}}
        2\lambda C |\bar{x}-\bar{y}|^2
        +
        \gamma e^{\mu \bar{t}}
        C_{p,T,\Upsilon,\sigma}
          \big[1 + \Upsilon(|\bar{x}|^p) +\Upsilon'(|\bar{y}|^p) \big]
        \\
        +
        \varepsilon^{\frac12}
        2^{(\frac {p}{2}\vee 1)-1} 
        3 \widebar{c}_{{}_\Upsilon}
        p\gamma e^{\mu \bar{t}}
          \big[1 + \Upsilon(|\bar{x}|^p)  \delta(\bar{x}) 
          +\Upsilon'(|\bar{y}|^p) \delta(\bar{y}) \big] 
        \\
        +
        2^{(\frac{p}{2}\vee 1)} 
        \varepsilon^{\frac 12}
        \lambda C |\bar{x}-\bar{y}|
        (
        \delta(\bar{x})^{\frac{1}{2}} + \delta(\bar{y})^{\frac{1}{2}}
        )
      \end{multlined}      
      \\
      &\hspace{1em} 
      \overset{\phantom{\text{\eqref{ineq:norm_to_delta}}}}{=}
       2\lambda C |\bar{x}-\bar{y}|^2
        +
        \gamma e^{\mu \bar{t}}
        C_{p,T, \Upsilon,\sigma}
          \big\{1 + \big[\Upsilon(|\bar{x}|^p)+\Upsilon(|\bar{y}|^p)\big] \big\}
          +\bar{\varrho}^2_{\gamma,\lambda,\varepsilon},
      \numberthis
      \label{lem_app:f_nonlinearities_second}
    \end{align*}
    where $C_{p,T,\Upsilon,\sigma}$ is a positive constant which depends on $p,T,\Upsilon$ and $\sup_{\alpha\in\mathcal{A}} |\sigma_\alpha(0,0)|$, while it was defined
    \begin{multline*}
    \bar{\varrho}^2_{\gamma,\lambda,\varepsilon}:=
            \varepsilon^{\frac12}
        \big\{2^{(\frac {p}{2}\vee 1)-1} 
                3 \widebar{c}_{{}_\Upsilon}
                p\gamma e^{\mu \bar{t}}
                  \big[1 + \Upsilon(|\bar{x}|^p)  \delta(\bar{x}) 
                  +\Upsilon'(|\bar{y}|^p) \delta(\bar{y}) \big] 
                +
                2^{(\frac{p}{2}\vee 1)} 
                \lambda C |\bar{x}-\bar{y}|
                (
                \delta(\bar{x})^{\frac{1}{2}} + \delta(\bar{y})^{\frac{1}{2}}
                )\big\}.
    \end{multline*}
We clarify that in order to derive the second inequality it was used \eqref{ineq:norm_to_delta} twice and for the last inequality before \eqref{lem_app:f_nonlinearities_second} it was used the fact that
\begin{align*}
     \sup_{\alpha\in\mathcal{A}} |\sigma_\alpha(\bar{t},0)|
     \leq \omega(\bar{t}) +  \sup_{\alpha\in\mathcal{A}} |\sigma_\alpha(0,0)|
     \overset{\ref{HJB:coeff_boundedness}}{<}+\infty.
\end{align*}
Finally, in view of the properties described in \cref{rem_append:aux_properties}.\ref{regularity_aux_remark:limsup_lambda_varepsilon_barx_bary}, which essentially guarantee the boundedness of the curly bracket of $\bar{\varrho}^2_{\gamma,\lambda,\varepsilon}$, 
and the continuity of $\Upsilon$, we have that
    \begin{align}
    % \limsup_{\gamma\downarrow 0}
    % \limsup_{\lambda\to +\infty}
    \limsup_{\varepsilon \downarrow 0} 
    \bar{\varrho}^2_{\gamma,\lambda,\varepsilon} = 0.
    \label{limsup_lambda_epsilon_bar_rho_2}
    \end{align}


    % \item 
\textbullet\hspace{0.3em}
    For the third summand of \eqref{HJB:reg_cond_nonlinearities_aux_part_a} we have
    \begin{align*}
      &\sup_{(\alpha,x,y) \in \mathcal{A}_{\varepsilon}} 
      \Big(\mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}) 
            -\mathcal{K}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y},-\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\bar{x},\cdot)\circ\tau_{\bar{y}-y})\Big)^+\\
      &\hspace{2em}
      \begin{multlined}[c][0.9\textwidth]
      \le 
      \bar{\varrho}^3_{\gamma,\lambda,\varepsilon,\kappa}
      +\sup_{(\alpha,x,y) \in \mathcal{A}_{\varepsilon}}\Big(
      \overline{\mathcal{K}}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x}) 
            -\overline{\mathcal{K}}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y})\Big)^+.
      \end{multlined}
      \numberthis\label{lem_app:f_nonlinearities_third_1}
    \end{align*}
    where we defined
    \begin{gather*}
      \bar{\varrho}^3_{\gamma,\lambda,\varepsilon,\kappa}:=
       \sup_{(\alpha,x,y) \in \mathcal{A}_{\varepsilon}}\big| 
      \check{\mathcal{K}}^\kappa_\alpha(\bar{t},x,\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}) \big|
      + \sup_{(\alpha,x,y) \in \mathcal{A}_{\varepsilon}}\big| 
            \check{\mathcal{K}}^\kappa_\alpha(\bar{t},y,-\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\bar{x},\cdot)\circ\tau_{\bar{y}-y})\big|
    \end{gather*}

    We consider initially the term $\bar{\varrho}^3_{\gamma,\lambda,\varepsilon,\kappa}$, \emph{i.e.}, we we will work on the set $\{z: |z|\le \kappa\}$ with $\kappa\le 1$. 
    Given the Mean Value Theorem, we have that 
    \begin{align*}
      &\limsup_{\kappa \downarrow 0} \sup_{(\alpha,x,y)\in\mathcal{A}_{\varepsilon}}
        \big|\check{\mathcal{K}}^\kappa_\alpha(\bar{t},x,\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x})\big|\\
 %
 %
      &
      \overset{\phantom{\ref{HJB:cond_jump}.\ref{HJB:cond_jump_partB}}}{\underset{\phantom{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partA}}}{\leq}}
      \limsup_{\kappa \downarrow 0}\sup_{(\alpha,x,y)\in\mathcal{A}_{\varepsilon}}
        \int_{\{z: |z|\le \kappa\}} 
        \big|\phi_{\gamma,\delta,\mu}^\lambda(\bar{t}, \bar{x} + j_\alpha(\bar{t},x,z),\bar{y}) - \phi_{\gamma,\delta,\mu}^\lambda(\bar{t}, \bar{x} ,\bar{y})\big|\,\delta_{\alpha}(\bar{t},x,z)\, m_\alpha(\textup{d}z)\\
 %
 %
      &
      \overset{\phantom{\ref{HJB:cond_jump}.\ref{HJB:cond_jump_partB}}}{\underset{\phantom{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partA}}}{\leq}}
      \limsup_{\kappa \downarrow 0}\sup_{(\alpha,x,y)\in\mathcal{A}_{\varepsilon}}
      \int_{\{z: |z|\le \kappa\}} \Big| \Big(\int_0^1 D_x\phi_{\gamma,\delta,\mu}^\lambda(\bar{t}, \bar{x} + \xi j_\alpha(\bar{t},x,z),\bar{y})\textup{d}\xi\Big)^Tj_\alpha(\bar{t},x,z)\Big| \cdot  \delta_{\alpha}(\bar{t},x,z) m_\alpha(\textup{d}z)\\
 %
 %
      &\begin{multlined}[c][0.95\textwidth]
      \overset{\ref{HJB:cond_jump}.\ref{HJB:cond_jump_partB}}{\underset{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partA}}{\leq }}
      C\limsup_{\kappa \downarrow 0}
      \sup_{(\alpha,x,y)\in\mathcal{A}_{\varepsilon}} 
      \Big\{\sup_{|\zeta|\le 1, \xi\in[0,1]} 
        \big|D_x\phi_{\gamma,\delta,\mu}^\lambda\big(\bar{t}, \bar{x} + C\xi (1+|x|)\zeta,\bar{y}\big)\big| C(1+|x|) 
      \Big\} \\
            \times \Big(\sup_{\alpha\in\mathcal{A}}\int_{\{z: |z|\le \kappa\}} \ell_\alpha^2(z) m_\alpha(\textup{d}z)\Big)
            \times \Big(\sup_{\alpha\in\mathcal{A}}\int_{\{z: |z|\le \kappa\}} |z|^2 m_\alpha(\textup{d}z)\Big)
      \end{multlined}\\
      &\hspace{0.2em}
      \overset{\ref{HJB:UI}}{\underset{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partA}}{=}}
      0
    \end{align*}
    where we used Cauchy--Schwarz inequality and the boundedness of a continuous function on a compact set which contains the bounded set\footnote{Use \cref{rem_append:aux_properties}.\ref{regularity_aux_remark:limsup_lambda_varepsilon_barx_bary}.}
    \begin{align*}
      \{(\bar{t},\bar{x}+C\xi (1+|x|)\zeta,\bar{y}) : \xi \in[0,1], |\zeta|\le 1, x \text{ is s.t. } \varphi(x-\bar{x})\le \varepsilon \delta(\bar{x}), \bar{x},\bar{y} \text{ for }\lambda >0 \text{ and }\varepsilon\le\varepsilon_0 \}
    \end{align*} 
    and the fact that we work on the set $\{z: |z|\le \kappa\}$ with $\kappa\le 1$, with $\kappa \leq 1$.
    We have the analogous property for the term $\big|\check{\mathcal{K}}^\kappa_\alpha(\bar{t},y,\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\bar{x},\cdot)\circ\tau_{\bar{y}-y})\big|$.
    Thus, combining the two pieces of information just extracted in the above computations we have
    \begin{align}\label{limsup_lambda_epsilon_bar_rho_3}
      \limsup_{\kappa \downarrow 0}
      \bar{\varrho}^3_{\gamma,\lambda,\varepsilon,\kappa}
      =0
    \end{align}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
    We proceed with the second summand of the right-hand side of Inequality \eqref{lem_app:f_nonlinearities_third_1}, which means that we will work on the set $\{ z : \kappa <|z|\}$.
    Because of the (possible) singularity of the family of measure $\{m_\alpha\}_{\alpha\in\mathcal{A}}$ at the origin, we consider separately the cases $\{z: \kappa <|z|\le 1\}$ and $\{z: 1<|z|\}$.

    Let us deal with the integrands of the difference 
    \begin{align*}
    \overline{\mathcal{K}}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x}) 
            -\overline{\mathcal{K}}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y}),
    \end{align*}
    working on the set $\{z: \kappa <|z|\le 1\}$.
    To this end, one has for $(\alpha, x,y)\in \mathcal{A}_\varepsilon$:
    \begin{align*}
      &\big[u^\varepsilon(\bar{t},\bar{x}+j_\alpha(\bar{t},x,z)) - u^\varepsilon(\bar{t},\bar{x})\big] \delta_\alpha(\bar{t},x,z) 
      -
      \big[v_\varepsilon(\bar{t},\bar{y}+j_\alpha(\bar{t},y,z)) - v_\varepsilon(\bar{t},\bar{y})\big] \delta_\alpha(\bar{t},y,z)\\
%
%
%
      & \begin{multlined}[c][0.9\textwidth]
      \overset{\phantom{\eqref{supremum_penalized}}}{\underset{\phantom{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partC}}}{=}} 
      \big\{\big[u^\varepsilon(\bar{t},\bar{x}+j_\alpha(\bar{t},x,z)) - u^\varepsilon(\bar{t},\bar{x})\big]   
                - \big[v_\varepsilon(\bar{t},\bar{y}+j_\alpha(\bar{t},y,z)) - v_\varepsilon(\bar{t},\bar{y})\big]
            \big\}\delta_\alpha(\bar{t},x,z)\\
      +\big[v_\varepsilon(\bar{t},\bar{y}+j_\alpha(\bar{t},y,z)) - v_\varepsilon(\bar{t},\bar{y})\big] 
      \big[\delta_\alpha(\bar{t},x,z) - \delta_\alpha(\bar{t},y,z)\big]
      \end{multlined}
      \\
%
%
%
      &\begin{multlined}[c][0.9\textwidth]
      \overset{\eqref{supremum_penalized}}{\underset{\phantom{\text{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partC}}}}{\le}} 
      \big[\phi^\lambda_{\gamma,\delta,\mu} (\bar{t},\bar{x}+j_\alpha(\bar{t},x,z),\bar{y}+j_\alpha(\bar{t},y,z)) - \phi^\lambda_{\gamma,\delta,\mu} (\bar{t},\bar{x},\bar{y})\big]\delta_\alpha(\bar{t},x,z)\\
      + \big[v_\varepsilon(\bar{t},\bar{y}+j_\alpha(\bar{t},y,z)) - v_\varepsilon(\bar{t},\bar{y})\big] 
      \big[\delta_\alpha(\bar{t},x,z) - \delta_\alpha(\bar{t},y,z)\big],
      \end{multlined}
      \numberthis\label{case_v_locally_Lipschitz}
      \\
%
%
%
      &\begin{multlined}[c][0.9\textwidth]
      \overset{\eqref{def:penalization_function}}{\underset{\text{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partC}}}{\le}} 
      \lambda\big( |\bar{x} + j_\alpha(\bar{t}, x,z) - (\bar{y} + j_\alpha(\bar{t}, y,z) )|^2 - |\bar{x} -\bar{y}|^2 \big) \delta_\alpha(\bar{t},x,z)\\
        +\gamma e^{\mu \bar{t}}
        \Big[  
        \Upsilon\big( |\bar{x}+j_\alpha(\bar{t},x,z)|^p\big) - \Upsilon\big( |\bar{x}|^p\big) 
        + \Upsilon\big( |\bar{y}+j_\alpha(\bar{t},y,z)|^p\big) - \Upsilon\big( |\bar{y}|^p\big)
        \Big] \delta_\alpha(\bar{t},x,z)\\
        +\sup_{\varepsilon\in(0,\varepsilon_0]}\Vert v_\varepsilon\Vert_p 
        (1 + |\bar{y}|^p + |j_{\alpha}(\bar{t},y,z) |^p )\times  C |x-y|  \ell_{\alpha}^2(z)
      \end{multlined}
      \\
%
%
%
      &\begin{multlined}[c][0.9\textwidth]
      \overset{\eqref{bound:norm_x_y}}{\underset{\phantom{\text{\ref{HJB:cond_jump}.\ref{HJB:growth_cond_delta_partC}}}}{\le}} 
      \lambda\big[
        |j_\alpha(\bar{t}, x,z) - j_\alpha(\bar{t}, y,z)|^2 - 2(\bar{x}-\bar{y})^T(j_\alpha(\bar{t},x,z) - j_\alpha(\bar{t},y,z)) 
      \big] 
      \delta_\alpha(\bar{t},x,z)\\
        +\gamma e^{\mu \bar{t}}
      \sup_{\xi\in[0,1]} \{\Upsilon'(|\bar{x}+\xi j_\alpha(\bar{t},x,z) |^p) \times |\bar{x}+\xi j_\alpha(\bar{t},x,z)|^{p-1} \}
      \times |j_\alpha(\bar{t},x,z)|
      \times  \delta_\alpha(\bar{t},x,z)\\
        +\gamma e^{\mu \bar{t}}
      \sup_{\xi\in[0,1]} \{\Upsilon'(|\bar{y}+\xi j_\alpha(\bar{t},y,z) |^p) \times |\bar{y}+\xi j_\alpha(\bar{t},y,z)|^{p-1} \}
      \times |j_\alpha(\bar{t},y,z)|
      \times \delta_\alpha(\bar{t},x,z)\\
        +C_p(1 + |\bar{y}|^p + (1+|y|^p)|z|^p )\big[|\bar{x}-\bar{y}| +2^{(\frac{p}{2}\vee 1)}\varepsilon^{\frac12}\big(\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}\big) \big] 
            \times \sup_{\varepsilon\in(0,\varepsilon_0]}\Vert v_\varepsilon\Vert_p\,  \ell_{\alpha}^2(z)
      \end{multlined}
      \numberthis\label{HJB:reg_cond_nonlinearities_aux_part_c_JustAfterTaylor}
      \\
%
%
%
      &\begin{multlined}[c][0.9\textwidth]
      \overset{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partA}}{\underset{\ref{HJB:cond_jump}.\ref{HJB:cond_jump_partA},\ref{HJB:cond_jump_partB}}{\le}} 
      \lambda C\big( |x-y|^2 |z|^2 + 2|\bar{x}-\bar{y}| \times |x-y| |z| \big) \ell_\alpha(z)\\
        +C\gamma e^{\mu \bar{t}}
      \sup_{\xi\in[0,1]} \{\Upsilon'(|\bar{x}+\xi j_\alpha(\bar{t},x,z) |^p) \times |\bar{x}+\xi j_\alpha(\bar{t},x,z)|^{p-1} \}
      \times (1+|x|)|z|\ell_{\alpha}(z)\\
        +C \gamma e^{\mu \bar{t}}
      \sup_{\xi\in[0,1]} \{\Upsilon'(|\bar{y}+\xi j_\alpha(\bar{t},y,z) |^p) \times |\bar{y}+\xi j_\alpha(\bar{t},y,z)|^{p-1} \}
      \times (1+|x|)|z|\ell_{\alpha}(z)\\
        +C_p(1 + |\bar{y}|^p + \varepsilon^{\frac{p}{2}} \delta(\bar{y})^{\frac{p}{2}})
        \big[|\bar{x}-\bar{y}| +2^{(\frac{p}{2}\vee 1)}\varepsilon^{\frac12}\big(\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}\big) \big]
        \times \sup_{\varepsilon\in(0,\varepsilon_0]}\Vert v_\varepsilon\Vert_p\,  \ell_{\alpha}^2(z)
      \end{multlined}\\
%
%
%
      &\begin{multlined}[c][0.9\textwidth]
      \overset{\eqref{bound:norm_x_y}}{\underset{\ref{HJB:cond_jump}.\ref{HJB:cond_jump_partA},\ref{HJB:cond_jump_partB}}{\le}} 
      \lambda C\big( |\bar{x}-\bar{y}|^2 |z|^2 + 2|\bar{x}-\bar{y}|^2 |z| \big) \ell_\alpha(z)\\
      +\lambda C\big( 2^{(\frac{p}{2}\vee1)}
      \varepsilon 
      (\delta(\bar{x}) + \delta(\bar{y})) |z|^2 
      + 2^{(\frac{p}{2}\vee1)}|\bar{x}-\bar{y}|
      \varepsilon^{\frac12} 
      (\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12})
       |z| \big) (1+|x|)\ell_\alpha(z)\\
        +C\gamma e^{\mu \bar{t}}
      \sup_{\xi\in[0,1]} \{\Upsilon'(|\bar{x}+\xi j_\alpha(\bar{t},x,z) |^p) \times |\bar{x}+\xi j_\alpha(\bar{t},x,z)|^{p-1} \}
      \times (1+|x|)|z|\ell_{\alpha}(z)\\
        +C \gamma e^{\mu \bar{t}}
      \sup_{\xi\in[0,1]} \{\Upsilon'(|\bar{y}+\xi j_\alpha(\bar{t},y,z) |^p) \times |\bar{y}+\xi j_\alpha(\bar{t},y,z)|^{p-1} \}
      \times (1+|x|)|z|\ell_{\alpha}(z)\\
        +C_p(1 + |\bar{y}|^p + \varepsilon^{\frac{p}{2}} \delta(\bar{y})^{\frac{p}{2}})\big[|\bar{x}-\bar{y}| +2^{(\frac{p}{2}\vee 1)}\varepsilon^{\frac12}\big(\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}\big) \big]
        \times \sup_{\varepsilon\in(0,\varepsilon_0]}\Vert v_\varepsilon\Vert_p\,  \ell_{\alpha}^2(z)
      \end{multlined}\\
%
%
%
     &\begin{multlined}[c][0.9\textwidth]
      \overset{\eqref{bound:supremum_Upsilon_xi_unit_ball}}{\underset{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partB}}{\leq}}
      \lambda C\big(\sup_{\alpha\in\mathcal{A}}\|\ell_\alpha\|_{\infty}\times |\bar{x}-\bar{y}|^2 |z|^2 
      + 2|\bar{x}-\bar{y}|^2 |z|\ell_\alpha(z) \big)\\
      +\lambda C\big( 2^{(\frac{p}{2}\vee1)}
      \varepsilon 
      (\delta(\bar{x}) + \delta(\bar{y})) |z|^2 
      + 2^{(\frac{p}{2}\vee1)}|\bar{x}-\bar{y}|
      \varepsilon^{\frac12} 
      (\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12})
       |z| \big)\ell_\alpha(z)\\
        +\gamma e^{\mu \bar{t}}
        \big\{C_{p,\Upsilon}\big[1 + \Upsilon(|\bar{x}|^p)\big] + 
                \vartheta^1_{\gamma, \lambda,\varepsilon}(\bar{x},x)\big\}|z|\ell_{\alpha}(z)\\
        +\gamma e^{\mu \bar{t}}
        \big\{C_{p,\Upsilon}\big[1 + \Upsilon(|\bar{y}|^p)\big] + 
                \vartheta^1_{\gamma, \lambda,\varepsilon}(\bar{y},y)\big\}|z|\ell_{\alpha}(z)\\
        +C_p(1 + |\bar{y}|^p + \varepsilon^{\frac{p}{2}} \delta(\bar{y})^{\frac{p}{2}})
        \big[|\bar{x}-\bar{y}| +2^{(\frac{p}{2}\vee 1)}\varepsilon^{\frac12}\big(\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}\big) \big] 
            \times \sup_{\varepsilon\in(0,\varepsilon_0]} \Vert v_\varepsilon\Vert_p\,  \ell_{\alpha}^2(z)
      \end{multlined}\\
%
%
%
% \shortintertext{\todo[inline]{Continue here}}
    &\begin{multlined}[c][0.9\textwidth]
      \overset{\eqref{bound:convolution_p_norms}}{\underset{\phantom{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partB}}}{\leq}}
      C_{\ell} \lambda |\bar{x}-\bar{y}|^2 \big(|z|^2  +|z|\ell_\alpha(z) \big)
      +\gamma e^{\mu \bar{t}} C_{p,\Upsilon} \big[1 + \Upsilon(|\bar{x}|^p) + \Upsilon(|\bar{y}|^p)\big] |z| \ell_{\alpha}(z)
      +\bar{\theta}^1_{\gamma,\lambda,\varepsilon}(z)
    \end{multlined}
    \numberthis\label{lem_app:f_nonlinearities_third_2}
    \end{align*}
    where 
    \begin{align}
    \begin{multlined}[0.9\textwidth]
    \bar{\theta}^1_{\gamma,\lambda,\varepsilon}(z):=
      \lambda C_{p,\ell}
      \varepsilon 
      (\delta(\bar{x}) + \delta(\bar{y})) |z|^2 
      + C_p |\bar{x}-\bar{y}|
      \varepsilon^{\frac12} 
      (\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12})
       |z| \ell_\alpha(z)\\
        +\gamma e^{\mu \bar{t}}
        C_{p,\Upsilon}\big[
                \vartheta^1_{\gamma, \lambda,\varepsilon}(\bar{x},x)
              + \vartheta^1_{\gamma, \lambda,\varepsilon}(\bar{y},y)
                \big]
                |z|\ell_{\alpha}(z)\\
        +C_{p,v}(1 + |\bar{y}|^p + \varepsilon^{\frac{p}{2}} \delta(\bar{y})^{\frac{p}{2}})
        \big[
        |\bar{x}-\bar{y}| 
        +2^{(\frac{p}{2}\vee 1)}\varepsilon^{\frac12}\big(\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}\big) 
        \big] 
        \times  \ell_{\alpha}^2(z).
    \end{multlined}
    \label{def:bar_theta_1}
    \end{align}
%
%
%
%
%
%
%
Finally, we consider the case $\{z: |z|>1 \}$ and we initially manipulate the respective integrands just like the case $\{z:\kappa<|z|\leq 1\}$. 
Then we proceed as follows:
    \begin{align*}
      &\big[u^\varepsilon(\bar{t},\bar{x}+j_\alpha(\bar{t},x,z)) - u^\varepsilon(\bar{t},\bar{x})\big] \delta_\alpha(\bar{t},x,z) 
      -
      \big[v_\varepsilon(\bar{t},\bar{y}+j_\alpha(\bar{t},y,z)) - v_\varepsilon(\bar{t},\bar{y})\big] \delta_\alpha(\bar{t},y,z)\\
%
%
%
    &\begin{multlined}[c][0.9\textwidth]
      \overset{\eqref{case_v_locally_Lipschitz}}{\underset{\phantom{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partC}}}{\le}} 
      \lambda\big( |\bar{x} + j_\alpha(\bar{t}, x,z) - (\bar{y} + j_\alpha(\bar{t}, y,z) )|^2 - |\bar{x} -\bar{y}|^2 \big) \delta_\alpha(\bar{t},x,z)\\
        +\gamma e^{\mu \bar{t}}
        \Big[  
        \Upsilon\big( |\bar{x}+j_\alpha(\bar{t},x,z)|^p\big) - \Upsilon\big( |\bar{x}|^p\big) 
        + \Upsilon\big( |\bar{y}+j_\alpha(\bar{t},y,z)|^p\big) - \Upsilon\big( |\bar{y}|^p\big)
        \Big] \delta_\alpha(\bar{t},x,z)\\
        +C  \sup_{\varepsilon\in(0,\varepsilon_0]}\Vert v_\varepsilon\Vert_p\,
        (1 + |\bar{y}|^p + |j_{\alpha}(\bar{t},y,z) |^p ) |x-y| \ell_{\alpha}(z)
    \end{multlined}
      \\
%
%
%
    &\begin{multlined}[c][0.9\textwidth]
      \overset{{\eqref{bound:norm_x_y}}}{\underset{\text{Lem. \ref{prep_aux_lemma:bound_through_submultiplicativity}}}{\le}} 
      \lambda\big[
        |j_\alpha(\bar{t}, x,z) - j_\alpha(\bar{t}, y,z)|^2 - 2(\bar{x}-\bar{y})^T(j_\alpha(\bar{t},x,z) - j_\alpha(\bar{t},y,z)) 
      \big] 
      \delta_\alpha(\bar{t},x,z)\\
        \begin{multlined}[0.75\textwidth]
            +\gamma e^{\mu \bar{t}}
            C_{p,\Upsilon} \big[1 
            +\Upsilon(|\bar{x}|^p)+ \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{x}^{\frac p2})\big)
            +\Upsilon(|\bar{y}|^p)+ \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{y}^{\frac p2})\big)\big]
            \big[1+\Upsilon(|z|^p)\big] 
             \sup_{\alpha\in\mathcal{A}}\|\ell_{\alpha}\|_{\infty}
        \end{multlined}\\
        +C_{p,v} |x-y|
        \big[ 
        \big(1 + |\bar{y}|^p + (1 + |\bar{y}|^p + \varepsilon^{\frac{p}{2}} \delta(\bar{x})^{\frac{p}{2}})|z|^p \big) 
        \big]
       \sup_{\alpha\in\mathcal{A}}\|\ell_{\alpha}\|_{\infty}
    \end{multlined}\\
%
%
%
    &\begin{multlined}[c][0.9\textwidth]
      \overset{\ref{HJB:cond_jump}.\ref{HJB:cond_jump_partC}}{\underset{{\ref{HJB:growth_cond_delta}}}{\le}} 
      \lambda C \big[|x-y|^2 + |\bar{x} -\bar{y}|\times |x-y|\big] 
        \times |z|^p \sup_{\alpha\in\mathcal{A}}\|\delta_\alpha(\bar{t},x,z)\|_{\infty}\\
        \begin{multlined}[0.75\textwidth]
            +\gamma e^{\mu \bar{t}}
            C_{p,\Upsilon,\ell} \big[1 + \Upsilon(|\bar{x}|^p)+ \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{x}^{\frac p2})\big)
            +\Upsilon(|\bar{y}|^p)+ \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{y}^{\frac p2})\big)\big]
            \times
            \big[1+\Upsilon(|z|^p)\big] 
        \end{multlined}\\
        +C_{p,v,\ell} \big[|\bar{x}-\bar{y}| + C_p \varepsilon^{\frac12} \big(\delta(\bar{x})^\frac12  + \delta(\bar{y})^\frac12 \big)\big]
        (1 + |\bar{y}|^p + \varepsilon^{\frac{p}{2}} \delta(\bar{y})^{\frac{p}{2}})(1+ |z|^p )  
    \end{multlined}\\
%
%
%
   &\begin{multlined}[c][0.9\textwidth]
      \overset{{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partB}}}{\underset{{\eqref{bound:norm_x_y}}}{\le}} 
       C_\ell  \lambda|\bar{x} -\bar{y}|^2 \times |z|^p
      +\gamma e^{\mu \bar{t}}
      C_{p,\Upsilon} \big[1 + \Upsilon(|\bar{x}|^p) +\Upsilon(|\bar{y}|^p)\big]
      \times \big[1+\Upsilon(|z|^p)\big] \\
      + C_{p,\ell}  \lambda|\bar{x} -\bar{y}| \varepsilon^{\frac12}\big(\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}\big) \times |z|^p\\
      +\gamma e^{\mu \bar{t}}
      C_{p,\Upsilon} \big[ \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{x}^{\frac p2})\big)
                + \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{y}^{\frac p2})\big)\big]
      \times \big[1+\Upsilon(|z|^p)\big] \\
      +C_{p,v,\ell} \big[|\bar{x}-\bar{y}| 
      + C_p \varepsilon^{\frac12} \big(\delta(\bar{x})^\frac12  + \delta(\bar{y})^\frac12 \big)\big]
      \big(1 + |\bar{y}|^p + (1 + |\bar{y}|^p + \varepsilon^{\frac{p}{2}} \delta(\bar{y})^{\frac{p}{2}})|z|^p \big) 
    \end{multlined}\\
%
%
%
    &\begin{multlined}[c][0.9\textwidth]
      \overset{\phantom{\eqref{bound:supremum_Upsilon_xi_unit_ball}}}{\underset{\phantom{\text{\ref{HJB:growth_cond_delta}\ref{HJB:growth_cond_delta_partC}}}}{=}} 
      C_{\ell}  \lambda |\bar{x}-\bar{y}|^2 \times |z|^p 
        +\gamma e^{\mu \bar{t}}C_{p,\Upsilon}
            \big[1 + \Upsilon(|\bar{x}|^p) +\Upsilon(|\bar{y}|^p)\big]
            [1 + \Upsilon(|z|^p)]
      +\bar{\theta}^2_{\gamma,\lambda,\varepsilon}(z)
    \end{multlined}
    \numberthis\label{lem_app:f_nonlinearities_third_3}
    \end{align*}
    where 
\begin{align}
\begin{multlined}[0.85\textwidth]
\bar{\theta}^2_{\gamma,\lambda,\varepsilon}(z):=
C_{p,\ell}  \lambda|\bar{x} -\bar{y}| \varepsilon^{\frac12}\big(\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}\big) \times |z|^p\\
      +\gamma e^{\mu \bar{t}}
      C_{p,\Upsilon} \big[ \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{x}^{\frac p2})\big)
                + \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{y}^{\frac p2})\big)\big]
      \times \big[1+\Upsilon(|z|^p)\big] \\
      +C_{p,v,\ell} \big[|\bar{x}-\bar{y}| 
      + C_p \varepsilon^{\frac12} \big(\delta(\bar{x})^\frac12  + \delta(\bar{y})^\frac12 \big)\big]
      \big(1 + |\bar{y}|^p + (1 + |\bar{y}|^p + \varepsilon^{\frac{p}{2}} \delta(\bar{y})^{\frac{p}{2}})|z|^p \big).
\end{multlined}
\end{align}
In the second inequality of the computations above, it was used \cref{prep_aux_lemma:bound_through_submultiplicativity}.
In the third inequality we distinguished between the cases $p\in[1,2)$ and $p\ge 2$ for the first two summands.
In the former case, for the first summand we used \ref{HJB:cond_jump}.\ref{HJB:cond_jump_partC}, while for the second summand we used that $\frac{p}{2}<p$.
In the later case, we did not need any further assumptions.

Collecting all the terms from \eqref{lem_app:f_nonlinearities_third_2} and \eqref{lem_app:f_nonlinearities_third_3} we obtain 
\begin{align*}
    &\hspace{-1em}\sup_{(\alpha,x,y) \in \mathcal{A}_{\varepsilon}}
    \Big(
    \overline{\mathcal{K}}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x}) 
        -\overline{\mathcal{K}}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y})\Big)^+\\
    &
    \begin{multlined}[0.95\textwidth]
    \overset{\eqref{lem_app:f_nonlinearities_third_2}}{\underset{\eqref{lem_app:f_nonlinearities_third_3}}{\leq}}
    \sup_{\alpha \in \mathcal{A}}
    \Big\{
        \lambda C_{\ell}
            |\bar{x}-\bar{y}|^2 \int_{\{z: \kappa< |z| \le 1\}}  \big(|z|^2 + |z| \ell_{\alpha}(z)\big)m_{\alpha} \textup{d}(z)\\
            +\gamma e^{\mu \bar{t}}C_{p,\Upsilon}\big[1 + \Upsilon(|\bar{x}|^p) +\Upsilon(|\bar{y}|^p)\big]
            \int_{\{z: \kappa< |z| \le 1\}} |z|\ell_{\alpha}(z) m_{\alpha} \textup{d}(z)\\
                + \lambda C_{\ell} |\bar{x}-\bar{y}|^2 
                \int_{\{z: 1< |z|\}} |z|^p m_{\alpha} \textup{d}(z) \\
                +\gamma e^{\mu \bar{t}}C_{p,\Upsilon}
                \big[1 + \Upsilon(|\bar{x}|^p) +\Upsilon(|\bar{y}|^p)\big]
                \int_{\{z: 1< |z|\}}[1 + \Upsilon(|z|^p)] m_{\alpha} \textup{d}(z)\\
                +\int_{\{z: \kappa< |z| \le 1\}}\bar{\theta}^1_{\gamma,\lambda,\varepsilon}(z) m_{\alpha} \textup{d}(z)
                +\int_{\{z: 1< |z|\}}\bar{\theta}^2_{\gamma,\lambda,\varepsilon}(z) m_{\alpha} \textup{d}(z)\Big\}
      \end{multlined}\\
    &
    \begin{multlined}[0.95\textwidth]
    \overset{\phantom{\eqref{lem_app:f_nonlinearities_third_2}}}{\underset{\phantom{\eqref{lem_app:f_nonlinearities_third_3}}}{=}}
      \lambda C_{\ell} |\bar{x}-\bar{y}|^2 
    \sup_{\alpha \in \mathcal{A}}
    \Big\{
      \int_{\{z:  |z| \le 1\}}  \big[|z|^2 + |z| \ell_{\alpha}(z)\big]m_{\alpha} \textup{d}(z)
      +  
      \int_{\{z: 1< |z|\}} |z|^p m_{\alpha} \textup{d}(z) 
    \Big\}
    \\
    \begin{multlined}[0.85\textwidth]
    +\gamma e^{\mu \bar{t}}C_{p,\Upsilon}\big[1 + \Upsilon(|\bar{x}|^p) +\Upsilon(|\bar{y}|^p)\big]\times\\
    \times\sup_{\alpha \in \mathcal{A}}
    \Big\{
      \int_{\{z:  |z| \le 1\}} |z|\ell_{\alpha}(z) m_{\alpha} \textup{d}(z)
      +\int_{\{z: 1< |z|\}}[1 + \Upsilon(|z|^p)] m_{\alpha} \textup{d}(z)
    \Big\}
    \end{multlined}
    \\
      +\int_{\{z: \kappa< |z| \le 1\}}\bar{\theta}^1_{\gamma,\lambda,\varepsilon}(z) m_{\alpha} \textup{d}(z)
      +\int_{\{z: 1< |z|\}}\bar{\theta}^2_{\gamma,\lambda,\varepsilon}(z) m_{\alpha} \textup{d}(z)\\
      +\lambda C_{\ell}
        |\bar{x}-\bar{y}|^2 
        \sup_{\alpha \in \mathcal{A}}
        \int_{\{z:  |z| \le \kappa\}}  \big(|z|^2 + |z| \ell_{\alpha}(z)\big)m_{\alpha} \textup{d}(z)\\
      +\gamma e^{\mu \bar{t}}C_{p,\Upsilon}\big[1 + \Upsilon(|\bar{x}|^p) +\Upsilon(|\bar{y}|^p)\big]
      \int_{\{z: |z| \le \kappa\}} |z|\ell_{\alpha}(z) m_{\alpha} \textup{d}(z)
    \end{multlined} \\
    &
    \begin{multlined}[0.95\textwidth]
    \overset{{\ref{HJB:UI}}}{\underset{{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partB}}}{=:}}
    \lambda C_{\ell,m} |\bar{x}-\bar{y}|^2 
    \gamma e^{\mu \bar{t}}C_{p,\Upsilon,m}
        \big[1 + \Upsilon(|\bar{x}|^p) +\Upsilon(|\bar{y}|^p)\big]
        % \Big[
        % \int_{\{z: \kappa< |z| \le 1\}} |z|\ell_{\alpha}(z) m_{\alpha} \textup{d}(z)
        % +
        % \int_{\{z: 1< |z|\}}[1 + \Upsilon(|z|^p)] m_{\alpha} \textup{d}(z)
        % \Big]\\
    +\bar{\varrho}_{\gamma,\lambda,\varepsilon,\kappa}^4,
    \end{multlined} 
    \numberthis\label{lem_app:f_nonlinearities_third}
\end{align*}
where $C_{p,\Upsilon,m}$ is a non-negative constant depending on  $p$, $\Upsilon$ and the quantity
\begin{align*}
       \sup_{\alpha\in\mathcal{A}} 
       \int_{\{z:  |z| \le 1\}} |z|\ell_{\alpha}(z) m_{\alpha} \textup{d}(z)
        +
       \sup_{\alpha\in\mathcal{A}} 
        \int_{\{z: 1< |z|\}}[1 + \Upsilon(|z|^p)] m_{\alpha} \textup{d}(z)
        \overset{\ref{HJB:UI}}{\underset{\ref{HJB:growth_cond_delta}.\ref{HJB:growth_cond_delta_partB}}{<}}<\infty
\end{align*}
  and $C_{l,m}$ is a non-negative constant depending on $\sup_{\alpha\in\mathcal{A}}\|\ell_{\alpha}\|_{\infty}$ and the aforementioned finite quantity.
Moreover, it is immediate verifiable that 
\begin{align}
    \label{limsup_lambda_epsilon_bar_rho_4}
    \limsup_{\lambda\to\infty}
    \limsup_{\varepsilon\downarrow 0}
    \limsup_{\kappa\downarrow 0}
    \bar{\varrho}_{\gamma,\lambda,\varepsilon,\kappa}^4=0.
\end{align}
In other words, we can rewrite \eqref{HJB:reg_cond_nonlinearities_aux_part_a} with the help of 
\eqref{lem_app:f_nonlinearities_first},   
\eqref{lem_app:f_nonlinearities_second},
\eqref{lem_app:f_nonlinearities_third_1},
% \eqref{lem_app:f_nonlinearities_third_2}, 
% \eqref{lem_app:f_nonlinearities_third_3}
 and 
\eqref{lem_app:f_nonlinearities_third} 
as follows
\begin{align*}
  &\begin{multlined}[c][\textwidth]
  \sup_{(\alpha,x,y)\in \mathcal{A}_{\varepsilon}} \Big\{ 
      f_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\bar{x}), \sigma^T_\alpha(\bar{t},x) D_x\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},x,u^\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{x}-x},\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\cdot,\bar{y})\circ\tau_{\bar{x}-x}))\\
      - f_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\bar{y}),-\sigma^T_\alpha(\bar{t},y) D_y\phi_{\gamma,\delta,\mu}^\lambda (\bar{t},\bar{x},\bar{y}), \mathcal{K}^\kappa_\alpha(\bar{t},y,v_\varepsilon(\bar{t},\cdot)\circ\tau_{\bar{y}-y},-\phi_{\gamma,\delta,\mu}^\lambda(\bar{t},\bar{x},\cdot)\circ\tau_{\bar{y}-y})) 
      \Big\}  
  \end{multlined}\\
      &\hspace{2em}
  \begin{multlined}[0.9\textwidth]
  \leq
    \overline{\omega}_{{}_R}\big( |\bar{x} - \bar{y}| \big) 
    +2\lambda C_{\ell,m} |\bar{x}-\bar{y}|^2
    +\gamma e^{\mu \bar{t}} C_{p,T, \Upsilon,\sigma,m,\ell}
        \big\{1 + \big[\Upsilon(|\bar{x}|^p)+\Upsilon(|\bar{y}|^p)\big] \big\}\\
          +\bar{\varrho}^1_{\gamma,\lambda,\varepsilon}
          +\bar{\varrho}^2_{\gamma,\lambda,\varepsilon}  
          +\bar{\varrho}^3_{\gamma,\lambda,\varepsilon,\kappa}
          +\bar{\varrho}^4_{\gamma,\lambda,\varepsilon,\kappa}
  \end{multlined}
\end{align*}
with 
\begin{align*}
  \limsup_{\lambda\to\infty}
  \limsup_{\varepsilon\downarrow}
  \limsup_{\kappa\downarrow0}
  \big[
    \bar{\varrho}^1_{\gamma,\lambda,\varepsilon}
      +\bar{\varrho}^2_{\gamma,\lambda,\varepsilon}  
      +\bar{\varrho}^3_{\gamma,\lambda,\varepsilon,\kappa}
      +\bar{\varrho}^4_{\gamma,\lambda,\varepsilon,\kappa}
      \big]\leq 0,
\end{align*}
which can be verified in view of 
\eqref{limsup_lambda_epsilon_bar_rho_1}
\eqref{limsup_lambda_epsilon_bar_rho_2}
\eqref{limsup_lambda_epsilon_bar_rho_3} 
and
\eqref{limsup_lambda_epsilon_bar_rho_4}.
  % \end{enumerate}

\end{proof}

==> Preparatory_Auxiliary_lemmata_HJB_Regularity_Condition.tex <==
%!TEX root = main.tex

For the reader's convenience, in this subsubsection we will recall and present some facts, which appeared in the proof of \cref{theorem:Domination_Principle}, which are going to be helpful in the completion of the proof.
In this way, it will be always clearly justified the validity of the arguments used.
It is underlined that we are, indeed, eligible in using them because we work under the hypetheses of \cref{def:regularity_condition}, as we did in the proof of \cref{theorem:Domination_Principle}. 

For ease of later reference, we collect these facts and properties in the next remark:
\begin{remark}\label{rem_append:aux_properties}
Following the notation introduced in the proof of \cref{HJB:Regularity_Condition}:
  \begin{enumerate}
    \item\label{def:varepsilon_0} Since $u$,$-v$ $\in \textup{USC}_p([0,T]\times \mathbb{R}^d)$, then for $C_{u,v}:= \max\{\|u\|_p, \|v\|_p\}\geq 0$ it is true that
    \begin{align*} 
      |u(t,x)|, |v(t,x)| \leq C_{u,v} (1+|x|^p).
    \end{align*}  
    Also, for given $p>0$, we have fixed the quasidistance $\varphi_p$ (denoted simply by $\varphi$) to be the smooth variant described in \cite[Lemma 1.14]{Hollender2017}, whose multiplier is $\rho =2^{2(p\vee 2)-2}$.
    From \cite[Lemma 1.12 (iii)]{Hollender2017}, we may choose $\varepsilon_0=\varepsilon_0(p,u,v)$ such that 
    \begin{align*}
        0<\varepsilon_0 \leq \frac{1}{2 \rho C_{u,v}}
    \end{align*}
    and, among other properties, it is satisfied
    \begin{align}\label{bound:convolution_p_norms} 
      \|u^\varepsilon\|_p, \|v_\varepsilon\|_p \leq \rho C_{u,v}, \text{ for }\varepsilon\leq \varepsilon_0,
    \end{align}   
    where $u^\varepsilon$, resp. $v_\varepsilon$, is the spatial supremal, resp. infimal, convolution of $u$, resp. $v$.

    Hereinafter, whenever we use $\varepsilon_0$, it will be understood the value determined in \cite[Lemma 1.12 (iii)]{Hollender2017} and depends only on $p$,$u$ and $v$. 
    \item\label{regularity_aux_remark:phi_compact} The quasidistance $\varphi$ is continuous and such that $\{z\in\mathbb{R}^d : \varphi(z)\le c\}$ is compact, for every $c>0$; see \cite[Lemma 1.12, Lemma 1.14]{Hollender2017}. 
    Hence, the set $\{x\in\mathbb{R}^d : (\alpha,x,y)\in\mathcal{A}_{\varepsilon}\}$, resp $\{y\in\mathbb{R}^d : (\alpha,x,y)\in\mathcal{A}_{\varepsilon}\}$, is a compact neighbourhood of $\bar{x}$, resp. $\bar{y}$, for every $\varepsilon\ge0$.
    %
    %
    \item\label{regularity_aux_remark:limsup_lambda_varepsilon_barx_bary} 
    The family of points $\{\bar{x}, \bar{y}: \lambda>0,0<\varepsilon\le \varepsilon_0\}$ (for the $\varepsilon_0>0$ described in \ref{def:varepsilon_0}), lies in a closed ball whose radius depends on $\gamma$; the reader may recall \eqref{domin_principle:bounded_norms_of_maxima}.
    Combined with the information in \ref{regularity_aux_remark:phi_compact}, we can safely assume that there exists a closed ball of radius $R=R(\gamma)$ which contains $\{x\in\mathbb{R}^d : (\alpha,x,y)\in\mathcal{A}_{\varepsilon}\}$ and $\{y\in\mathbb{R}^d : (\alpha,x,y)\in\mathcal{A}_{\varepsilon}\}$, for every $\lambda>0$ and $0<\varepsilon\le \varepsilon_0$.
    Moreover, recall that
    \begin{align}
       \limsup_{\lambda\to+\infty}\limsup_{\varepsilon \downarrow 0} \lambda | \bar{x}-\bar{y}|^2=0,
     \tag{\ref{domin_principle:liminfima_limsuprema_to_0}}
     \end{align} 
    which implies that 
    \begin{align}
       \limsup_{\lambda\to+\infty} \lambda  | \hat{x}-\hat{y}|^2=0,
       \label{limsup_lambda_limit_point}
     \end{align}
    for the arbitrary limit point $(\hat{t},\hat{x},\hat{y})=\big(\hat{t}(\gamma,\lambda),\hat{x}(\gamma,\lambda),\hat{y}(\gamma,\lambda)\big)$  of $(\bar{t}(\gamma,\lambda,\varepsilon),\bar{x}(\gamma,\lambda,\varepsilon),\bar{y}(\gamma,\lambda,\varepsilon))_{\varepsilon\in(0,\varepsilon_0]}$.
    %
    %
    \item\label{regularity_aux_remark:bounded_barx_bary} 
    The continuity of $\varphi$ and the boundedness of $\{\bar{x}, \bar{y}: 0<\varepsilon\le \varepsilon_0\}$, for fixed $\gamma,\lambda>0$ (for the $\varepsilon_0>0$ describe in \ref{def:varepsilon_0}), implies that $\{\delta(\bar{x}), \delta(\bar{y}): 0<\varepsilon\le \varepsilon_0\}$ is also bounded.
    Hence, we may use later that 
    \begin{align}
    \label{limit:varepsilon_delta_to_0}
    \lim_{\varepsilon \downarrow 0} \varepsilon(\delta(\bar{x})\vee \delta(\bar{y}))=0;
    \end{align}
    for the definition of $\delta(\cdot)$ recall \eqref{def:delta_x_phi}.
    %
    %
    \item\label{regularity_aux_remark:norm_to_delta}
    For $(\alpha,x,y)\in\mathcal{A}_{\varepsilon}$, $\varepsilon \in (0,\varepsilon_0]$ it is true that 
    \begin{align}
    |x-\bar{x}| 
      \overset{\text{\eqref{quasidist:growth}}}{\leq} 
      2^{(\frac{p}{2}\vee1)-1} \varphi(x-\bar{x})^{\frac12} 
      \overset{\text{\eqref{def:A_epsilon}}}{\leq} 
      2^{(\frac{p}{2}\vee1)-1}
      \varepsilon^{\frac12} 
      \delta(\bar{x})^{\frac12};
      \label{ineq:norm_to_delta}
    \end{align}
    for the definition of $\delta(\cdot)$ recall \eqref{def:delta_x_phi}.
    Analogously, we can derive the same bounds for $|y-\bar{y}|$.
    These further imply 
    \begin{align}
    \label{limit:norm_x_barx_to_0}
    \lim_{\varepsilon \downarrow 0} (x,y) = (\bar{x},\bar{y})\text{ for }(\alpha,x,y)\in\mathcal{A}_{\varepsilon}.
    \end{align}
    Additionally, we have the bound
    \begin{align}
        |x- y| \leq |\bar{x} - \bar{y}| 
        + 2^{(\frac{p}{2}\vee1)-1}
      \varepsilon^{\frac12} 
      (\delta(\bar{x})^{\frac12} + \delta(\bar{y})^{\frac12}).
    \label{bound:norm_x_y}
    \end{align}
    %
    %
    \item\label{regularity_aux_remark:sigma} 
    Let $(\hat{t},\hat{x},\hat{y})$ be a limit point of $(\bar{t}(\gamma,\lambda,\varepsilon),\bar{x}(\gamma,\lambda,\varepsilon),\bar{y}(\gamma,\lambda,\varepsilon))_{\varepsilon\in(0,\varepsilon_0]}$ and denote by $(\varepsilon_n)_{n\in\mathbb{N}}$ the associated sequence of indices.
    We remark that the limit point and the sequence $(\varepsilon_n)_{n\in\mathbb{N}}$ depend on $\gamma,\lambda$. 
    For notational simplicity we will denote only the dependence on $\varepsilon$.
     It is true that 
    \begin{align}
    \sup_{(\alpha,x): (\alpha,x,y) \in \mathcal{A}_{\varepsilon_n}, n\in\mathbb{N}}|\sigma_{\alpha} (\bar{t}(\varepsilon_n),x)|
     <\infty.
    \label{regularity_aux_remark:sigma_bound}
    \end{align}
    Indeed, in view of \ref{HJB:coef_continuity} one gets
    \begin{align*}
    \sup_{(\alpha,x): (\alpha,x,y) \in \mathcal{A}_{\varepsilon_n}, n\in\mathbb{N}}|\sigma_{\alpha} (\bar{t}(\varepsilon_n),x)|
    &\overset{\phantom{\text{\eqref{ineq:norm_to_delta}}}}{\leq}
    \sup_{(\alpha,x): (\alpha,x,y) \in \mathcal{A}_{\varepsilon_n}, n\in\mathbb{N}}
    \big\{
    |\sigma_{\alpha} (\bar{t}(\varepsilon_n),\bar{x}(\varepsilon_n))| 
    + C | x - \bar{x}(\varepsilon_n)|
    \big\}
    \\&\overset{\text{\eqref{ineq:norm_to_delta}}}{\leq}
    \sup_{n\in\mathbb{N}}
    \big\{
    |\sigma_{\alpha} (\bar{t}(\varepsilon_n),\bar{x}(\varepsilon_n))| 
    + C 2^{(\frac{p}{2}\vee 1)-1} \varepsilon_n^{\frac12} \delta(\bar{x}(\varepsilon_n))^{\frac12}
    \big\}.
    \end{align*}
    Now, the sequence $(\bar{x}(\varepsilon_n))_{n\in\mathbb{N}}$ is bounded as convergent, hence also $\delta(\bar{x}(\varepsilon_n))$; see \eqref{def:delta_x_phi}.
    The continuity of $\sigma_{\alpha}$ implies also the boundedness of $\big(\sigma_{\alpha} (\bar{t}(\varepsilon_n),\bar{x}(\varepsilon_n))\big)_{n\in\mathbb{N}}$, for every $\alpha\in\mathcal{A}$.
    Recalling \ref{HJB:coeff_boundedness} and using \ref{HJB:coef_continuity}, we can easily get a uniform bound for the tail of the sequence; the tail is understood independent of $\alpha\in\mathcal{A}$.
    Hence, by possibly increasing the last bound by using \ref{HJB:coeff_boundedness} again, we get a bound for the family  
    $\sup_{n\in\mathbb{N}}\big\{
    |\sigma_{\alpha} (\bar{t}(\varepsilon_n),\bar{x}(\varepsilon_n))| 
    \big\}$, which proves the claim \eqref{regularity_aux_remark:sigma_bound}.
%
    \item\label{regularity_aux_remark:_6}
    Let $x$ be such that $(\alpha,x,y)\in\mathcal{A}_{\varepsilon}$ and $z\in B[0,1]$. 
    Then, by \ref{regularity_aux_remark:limsup_lambda_varepsilon_barx_bary} and \ref{regularity_aux_remark:norm_to_delta} we have
    \begin{align*}
      \limsup_{\varepsilon \downarrow 0} |x| 
    = \limsup_{\varepsilon \downarrow 0} |\bar{x}| 
    \leq \limsup_{\varepsilon \downarrow 0} \sup_{\alpha\in\mathcal{A}}\sup_{\xi \in [0,1]}|\bar{x} + \xi j_{\alpha}(\bar{t},x,z)|
    \overset{\ref{HJB:cond_jump}.\ref{HJB:cond_jump_partB}}{\leq}  
    \limsup_{\varepsilon \downarrow 0} (1+2 |\bar{x}|).
    \end{align*}
    \todo[inline]{Alternatively}
    \begin{align*}
      |x| \leq C_p \varepsilon^{\frac12} (1+\varphi(\bar{x}))^{\frac12} + |\bar{x}|
          \leq C_p \varepsilon^{\frac12} (1+\varphi(\bar{x}))^{\frac12} 
              + \sup_{\alpha \in \mathcal{A}} \sup_{\xi \in [0,1]}  |\bar{x} + \xi j_{\alpha}(\bar{t},x,z)|.
    \end{align*}
    %
    %
    %
    \item \label{regularity_aux_remark:Young_function_properties}
        We are going to make use of some properties of $\Upsilon$ proven in \cref{lemma:UI_Young_improvement}. 
        We (seemingly) need to distinguish between the cases $p\in[1,2)$ and $p\ge 2$.
        In both cases we use the moderate growth property of $\Upsilon$, \emph{i.e.}, 
        \begin{align}
            \widebar{c}_{{}_\Upsilon}:=\sup_{w>0} \frac{w \Upsilon'(w) }{\Upsilon(w)} <+\infty,
        \end{align}
        with $\widebar{c}_{{}_\Upsilon}\geq 1$,
        while for the case $p\in[1,2)$ we additionally need $\lim_{w\downarrow 0}\Upsilon'(w^p)w^{p-2}=0$, \emph{i.e.},
        \cref{lemma:UI_Young_improvement}.\ref{lemma:UI_Young_improvement:p_smaller_than_2}. 
        In total, in either case
        \begin{align}
            \Upsilon'(|z|^p)(|z|^{p-2} + |z|^{p-1} + |z|^p) \le C_{\Upsilon} (1 + \Upsilon(|z|^p) ) \text{ for every } z\in\mathbb{R}^d.\footnotemark
         \label{reg_cond:Upsilon_moderate}
        \end{align}%
        \footnotetext{The bound \eqref{reg_cond:Upsilon_moderate} holds for any $p>0$, since \cref{lemma:UI_Young_improvement}.\ref{lemma:UI_Young_improvement:p_smaller_than_2} is valid for any $p\in(0,2)$.}
    %
    %
    %
    \item \label{regularity_aux_remark:Young_function_properties_unit_Ball}
        In the course of the computations presented below, it will be needed to estimate the auxiliary quantity 
        $\Upsilon\big( [|\bar{x}| + |j_\alpha(\bar{t},x,z)|]^p\big)$
         for $x$ such that $(\alpha,x,y)\in\mathcal{A}_\varepsilon$, $z\in B[0,1]$ and $p\ge 1$. 
        We will present here the detailed derivation of a suitable upper bound.
        Obviously, an analogous bound works for $y$ such that $(\alpha,x,y)\in\mathcal{A}_\varepsilon$.
        Given the introduced assumptions we have
        \begin{align*}
            \Upsilon\big( [|\bar{x}| + |j_\alpha(\bar{t},x,z)|]^p\big)
            &\leq 2^{ p^{\widebar{c}_{{}_\Upsilon}}-1}
            \big[ \Upsilon(|\bar{x}|^p) + \Upsilon(|j_\alpha(\bar{t},x,z)|^p)\big]
            \leq C_{p,\Upsilon}
            \big[ \Upsilon(|\bar{x}|^p) + \Upsilon(1) + \Upsilon(|x|^p)\big]\\
            &\leq C_{p,\Upsilon} \big[1  + \Upsilon(|\bar{x}|^p) \big] 
                +C_{p,\Upsilon} \Upsilon(|x-\bar{x}|^p).
            \numberthis \label{bound:Upsilon_norm_unit_ball}
        \end{align*}
        where in the first inequality we used the convexity of the function $\mathbb{R}^d \ni z \longmapsto |z|^p$,
        % \footnote{We work under the assumption that $p\ge 1$.},
         the fact that $\Upsilon$ is non-decreasing, \cref{lem:Young-prprt}.\ref{lem:Young-prprt-ii-a} and the convexity of the Young function $\Upsilon$.
        In the second inequality were used similar arguments as before, in conjunction with \ref{HJB:coef_continuity}, and the fact that $z\in B[0,1]$.
        Finally, in the last inequality we used similar arguments as before and \eqref{ineq:norm_to_delta}.
        The reader may observe that, in view of \eqref{limit:norm_x_barx_to_0} and the continuity of $\Upsilon$, one has 
        \begin{align}
            \lim_{\varepsilon \downarrow 0} \Upsilon(|x-\bar{x}|^p) =
            \lim_{\varepsilon \downarrow 0} \Upsilon(|y-\bar{y}|^p) =0.
            \label{limit:varepsilon_in_Upsilon}
        \end{align}

\todo[inline]{Correct the desired expression. Is it $p-2$ or $p-1$?}
        We go one step further and we compute an upper bound for the term
        \begin{align*}
        &\sup_{\xi \in [0,1]}\big\{\Upsilon'(|\bar{x} + \xi j_\alpha(\bar{t},x,z)|^p) |\bar{x} + \xi j_\alpha(\bar{t},x,z)|^{p-1}\big\}
        (1 + |x|)(1+|\bar{x}|)\\
        %
        %
        %
        &\hspace{1em}
        \overset{\phantom{\eqref{ineq:norm_to_delta}}}{\leq} 
        \sup_{\xi \in [0,1]}\big\{\Upsilon'(|\bar{x} + \xi j_\alpha(\bar{t},x,z)|^p) |\bar{x} + \xi j_\alpha(\bar{t},x,z)|^{p-1}\big\}(1 + |x - \bar{x}| + |\bar{x}| )(1+|\bar{x}|)\\
        %
        %
        %
        &\hspace{1em}
        \begin{multlined}[0.9\textwidth]
        \overset{\eqref{ineq:norm_to_delta}}{\leq} 
        \sup_{\xi \in [0,1]}\big\{\Upsilon'(|\bar{x} + \xi j_\alpha(\bar{t},x,z)|^p) |\bar{x} + \xi j_\alpha(\bar{t},x,z)|^{p-2}\big\}\\
        %
        +C_{p}|\bar{x}|\varepsilon^{\frac12}\delta(\bar{x})^{\frac12}\sup_{\xi \in [0,1]}\big\{\Upsilon'(|\bar{x} + \xi j_\alpha(\bar{t},x,z)|^p) |\bar{x} + \xi j_\alpha(\bar{t},x,z)|^{p-2}\big\} \\
        %
        +2\sup_{\xi \in [0,1]}\big\{\Upsilon'(|\bar{x} + \xi j_\alpha(\bar{t},x,z)|^p) |\bar{x} + \xi j_\alpha(\bar{t},x,z)|^{p-1}\big\}\\
        %
        +\sup_{\xi \in [0,1]}\big\{\Upsilon'(|\bar{x} + \xi j_\alpha(\bar{t},x,z)|^p) |\bar{x} + \xi j_\alpha(\bar{t},x,z)|^{p}\big\}
        \end{multlined}\\
        %
        %
        %
        &\hspace{1em}
        \overset{\eqref{reg_cond:Upsilon_moderate}}{\leq} 
        C_{p,\Upsilon}\sup_{\xi \in [0,1]}\big[1 + \Upsilon(|\bar{x} + \xi j_\alpha(\bar{t},x,z)|^p)\big]
        + C_{p}\varepsilon^{\frac12}\delta(\bar{x})^\frac12 \sup_{\xi \in [0,1]}\big[1 + \Upsilon(|\bar{x} + \xi j_\alpha(\bar{t},x,z)|^p)\big]\\
        %
        %
        %
        &\hspace{1em}
        \overset{\phantom{\eqref{reg_cond:Upsilon_moderate}}}{\leq} 
        C_{p,\Upsilon}\big[1 + \Upsilon\big([|\bar{x}| + |j_\alpha(\bar{t},x,z)|]^p\big)\big]
        + C_{p}\varepsilon^{\frac12}\delta(\bar{x})^\frac12 
                \big[1 + \Upsilon\big([|\bar{x}| + | j_\alpha(\bar{t},x,z)|]^p\big)\big]\\
        %
        %
        %
        &\hspace{1em}
        \overset{\eqref{bound:Upsilon_norm_unit_ball}}{\leq} 
        C_{p,\Upsilon}\big[1 + \Upsilon(|\bar{x}|^p)\big]
        +C_{p,\Upsilon} \Upsilon(|x-\bar{x}|^p)
        + C_{p}\varepsilon\delta(\bar{x}) 
        \big[1 + \Upsilon(|\bar{x}|^p)\big] +  \Upsilon(|x-\bar{x}|^p)\big]\\
        %
        %
        %
        &\hspace{1em}
        \overset{\phantom{\eqref{bound:Upsilon_norm_unit_ball}}}{=:} 
        C_{p,\Upsilon}\big[1 + \Upsilon(|\bar{x}|^p)\big] + 
        \vartheta^1_{\gamma, \lambda,\varepsilon}(\bar{x},x);
        \numberthis\label{bound:supremum_Upsilon_xi_unit_ball}
        \end{align*}
% in the second inequality of the derivation above we used the first inequality of \eqref{ineq_bounds:norm_barx_xi}, 
% in the second inequality of the derivation above we used the first inequality of \eqref{ineq_bounds:norm_barx_xi}, 
% 
        where in the second inequality, resp. second but last, we used the first, resp. second\footnote{In conjunction with the fact that $\Upsilon$ is increasing.}, inequality below
        \begin{align}\label{ineq_bounds:norm_barx_xi}
        |\bar{x}| 
        \leq \sup_{\xi \in [0,1]}|\bar{x} + \xi j_\alpha(\bar{t},x,z)|
        \leq |\bar{x}| + |j_\alpha(\bar{t},x,z)|.
        \end{align}
        In view of \ref{regularity_aux_remark:limsup_lambda_varepsilon_barx_bary}, of the continuity of $\Upsilon$ and of \ref{regularity_aux_remark:norm_to_delta} we have that 
        \begin{align}
            \lim_{\varepsilon\downarrow 0}\vartheta^1_{\gamma,\lambda,\varepsilon}(\bar{x},x)=0.
            \label{limit:vartheta_1}
        \end{align}
%
%
%
%
%
        \item\label{regularity_aux_remark:Young_function_properties_unit_Ball_complement}
        In this part we will derive the analogous to \ref{regularity_aux_remark:Young_function_properties_unit_Ball} bounds for the case $z\in B[0,1]^c$.
        To this end, let $x$ be such that $(\alpha,x,y)\in\mathcal{A}_{\varepsilon}$. 
            



  \end{enumerate}  
\end{remark}      


\begin{lemma}\label{prep_aux_lemma:bound_through_submultiplicativity}
Under the framework assumed in this subsection and for $|z| > 1$, it holds
\begin{align*}
\Upsilon(|\bar{x} + j_\alpha(\bar{t},x,z)|^p) \leq C_{p,\Upsilon} \big[1 + \Upsilon(|\bar{x}|^p)+ \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{x}^{\frac p2})\big)\big]\big[1+\Upsilon(|z|^p)\big].
\shortintertext{as well as}
\Upsilon(|\bar{y} + j_\alpha(\bar{t},y,z)|^p) \leq C_{p,\Upsilon} \big[1 + \Upsilon(|\bar{y}|^p) + \Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{y}^{\frac p2})\big)\big]\big[1+\Upsilon(|z|^p)\big].
{}\end{align*}
where the constant $C_{p,\Upsilon}$ depends on $p\ge 0$ and $\Upsilon$.
% In particular, 
% % if $ (\bar{x}_{n})_{n\in\mathbb{N}}$ where $\bar{x}_n:=\bar{x}(\gamma,\lambda,\varepsilon_n)$, resp. $(\bar{y}_n)_{n\in\mathbb{N}}$ where $\bar{y}_n:=\bar{y}(\gamma,\lambda,\varepsilon_n)$, a convergent subsequence with limit $\hat{x}$, resp.$\hat{y}$, it is true that
% \begin{align*}
% \limsup_{\varepsilon \downarrow 0}
% \Upsilon(|\bar{x} + j_\alpha(\bar{t},x,z)|^p) 
% \leq  C_{p,\Upsilon} \big[1 + \Upsilon(\limsup_{\varepsilon \downarrow 0}|\bar{x}|^p)\big]\big[1+\Upsilon(|z|^p)\big].
% \shortintertext{as well as}
% \limsup_{\varepsilon \downarrow 0}
% \Upsilon(|\bar{y} + j_\alpha(\bar{t},y,z)|^p) 
% \leq  C_{p,\Upsilon} \big[1 + \Upsilon(\limsup_{\varepsilon \downarrow 0}|\bar{y}|^p)\big]\big[1+\Upsilon(|z|^p)\big].
% \end{align*}
\end{lemma}


\begin{proof}
Obviously, it is sufficient to consider the case for $x,\bar{x}$.
We will initially use the facts that $\Upsilon$ is a moderate Young function and that for $p>0$ the function $[0,\infty)\ni s\mapsto s^p$ satisfies for $s,t\ge 0$
\begin{align*}
(s+t)^p \leq 2^p (s^p + t^p).
\end{align*}
In view of the above properties and \cref{corrolary:Young_subadditive} we have
\begin{align*}
\Upsilon(|\bar{x} + j_{\alpha}(\bar{t},x,z)|^p)
 %
 &\le 2^{\overline{c}_{{}_\Upsilon}-1}\big[\Upsilon(|\bar{x}|^p) + \Upsilon(|j_{\alpha}(\bar{t},x,z)|^p)\big]\\
 &\le 2^{\overline{c}_{{}_\Upsilon}-1}\big[\Upsilon(|\bar{x}|^p) + C^{\overline{c}_{{}_\Upsilon}}\Upsilon\big((1+|x|^p)|z|^p\big)\big].
 \numberthis\label{ineq:aux_submultiplicative_1}
\end{align*}
where in the second inequality we used \ref{HJB:cond_jump}.\ref{HJB:cond_jump_partA}

Now, we will use \cref{lemma:UI_Young_improvement}.\ref{lemma:UI_Young_improvement:submultiplicativity}, \emph{i.e.} $\Upsilon$ behaves finally as a submultiplicative function.
Let $R_{\Upsilon}>1$ and $K_{\Upsilon}>0$ given by \cref{lemma:UI_Young_improvement}.\ref{lemma:UI_Young_improvement:submultiplicativity}.
Then, for $x,z$ such that $1+|x|^p, |z|^p>R_{\Upsilon}$ 
\begin{align*}
\Upsilon\big((1+|x|^p)|z|^p\big) 
	\leq K_{\Upsilon} \Upsilon(1+|x|^p)\Upsilon(|z|^p) 
	\leq K_{\Upsilon} 2^{\overline{c}_{{}_\Upsilon}-1}\max\{\Upsilon(1),1\}\big(1+\Upsilon(|x|^p)\big)\Upsilon(|z|^p).
 \numberthis\label{ineq:aux_submultiplicative_2}
\end{align*}
Let now $x,z$ be such that $\min\{1+|x|^p, |z|^p\}\leq R_{\Upsilon}$.
Then, 
\begin{align*}
\Upsilon\big((1+|x|^p)|z|^p\big)
&\leq 
	\begin{cases}
		\Upsilon(R_{\Upsilon})\Upsilon(|z|^p), &\text{if }(1+|x|^p)<R_{\Upsilon}\\
		\Upsilon(R_{\Upsilon})\Upsilon(|x|^p), &\text{if }|z|^p<R_{\Upsilon}\\
		\Upsilon(R_{\Upsilon}^2), &\text{if }(1+|x|^p),|z|^p<R_{\Upsilon}
	\end{cases}\\
&\leq \Upsilon(R_{\Upsilon}^2)\big[ 1 + \Upsilon(|x|^p)\big] \big[1 +\Upsilon(|z|^p) \big].
 \numberthis\label{ineq:aux_submultiplicative_3}
\end{align*}
Finally, in view of  
\begin{align*}
\Upsilon(|x|^p)
	\leq 
	C_{p,\Upsilon} \big[\Upsilon(|x - \bar{x}|^p) + \Upsilon(|\bar{x}|^p)\big]
	\overset{\eqref{ineq:norm_to_delta}}{\leq}
	C_{p,\Upsilon} \big[\Upsilon\big(\varepsilon^{\frac p2} \delta(\bar{x}^{\frac p2})\big) + \Upsilon(|\bar{x}|^p)\big],
\end{align*}
we can rewrite \eqref{ineq:aux_submultiplicative_1} with the help of \eqref{ineq:aux_submultiplicative_2} and \eqref{ineq:aux_submultiplicative_3} in the desired form. 
% The last part of the statement of the lemma is true because of the continuity of $\Upsilon$, the fact that $\Upsilon(0)=0$ and the boundedness of $(\delta(\bar{x}))_{n\in\mathbb{N}}$ for every fixed $\gamma$ and $\lambda$. 
\end{proof}

==> Proofs.tex <==
%!TEX root = main.tex
\appendix
\section{Proofs of of the presented results.}


==> Proofs_YoungFunctions.tex <==
%!TEX root = main.tex

\subsection{Proof of Proposition\ref{prop:UI_Young}}
\begin{proof}[Proof of \cref{prop:UI_Young}]
  The equivalence is -\emph{mutatis mutandis}- a restatement of the classical de La Vallée Poussin Theorem. 
  We provide all the details for the validity of the equivalence, since they will be crucial later for the construction of the twice continuously differentiable,  moderate Young function.
  For the equivalence, we follow \citet[Theorem II.22]{dellacherie1978probabilities}.
  % We need to separately examine the cases $p>0$ and $p=0$.
  We define 
  \begin{align}
    M:= \sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|\ge 1\}} \Upsilon(|z|^p)m_\alpha(\textup{d}z).
    \label{def:M_supremum_of_Young_integrals}
  \end{align}
% 
% \vspace{0.5em}
%   {\tiny $\blacksquare$} $p>0.$
  and we assume initially that $M$ is finite. 
  Let $\varepsilon>0$ and define $K:=\frac{M}{\varepsilon}$.
  Since $\Upsilon$ is a Young function, there exists $R>0$ such that $\displaystyle \frac{\Upsilon(x)}{x}\ge K$, for every $x>R$.
  Hence, we have 
  \begin{align*}
    \sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|>R^{\frac{1}{p}}\}} |z|^p m_\alpha(\textup{d}z)
      \le \sup_{\alpha\in\mathcal{A}} \frac{1}{K}\int_{\{z:|z|>R^{\frac{1}{p}}\}} \Upsilon(|z|^p) m_\alpha(\textup{d}z)
      \le \varepsilon.
  \end{align*}   

  In order to prove the other direction of the equivelence, \emph{i.e.}, the existence of a moderate Young function $\Upsilon$ such that $M$ is finite, we will construct a piecewise constant, non-negative, increasing function $\upsilon$, which will serve as the right-derivative of the desired Young function. 
  The construction will be based on the assumption that 
  \begin{align}
    \lim_{R\to\infty}\sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|>R\}} |z|^p m_\alpha(\textup{d}z) =0.
  \label{Uniform_Integr_Limit_zero}
  \end{align}
  The function $\upsilon$ will initially be chosen to satisfy $\upsilon(x)=\upsilon_n$, for $x\in [n,n+1)$, for $n\in\mathbb{N}\cup\{0\}$, where $0\le \upsilon_n\le \upsilon_{n+1}$ for every $n\in\mathbb{N}\cup\{0\}$.
  We are allowed to choose $\upsilon_0=0$ and we do so. 
  Before we choose the rest values $(\upsilon_n)_{n\in\mathbb{N}}$, the reader may observe that for every $n\in\mathbb{N}$,
  \begin{align*}  
    \Upsilon(x) =  \sum_{k=1}^{n-1} \upsilon_k + \upsilon_n(x-n), \text{ for }x\in[n,n+1),
  \end{align*}  
  which in particular implies 
  \begin{align*}
    \Upsilon(x) \le  \sum_{k=1}^{n} \upsilon_k, \text{ for }x\in[n,n+1).
  \end{align*}
  Let us proceed by determining an upper bound of $M$ in terms of $(\upsilon_n)_{n\in\mathbb{N}}$:
  \begin{align*}
    \int_{\{z:|z|\ge 1\}} \Upsilon(|z|^p) m_\alpha(\textup{d}z) 
    \le \sum_{n=1}^{\infty} (\sum_{k=1}^n \upsilon_k) m_\alpha(\{z:n\le |z|^p<n+1\})
    = \sum_{n=1}^{\infty} \upsilon_n m_\alpha(\{z:|z|^p\ge n\}).
  \end{align*}
  Hence,
  \begin{align}
    M=\sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|\ge 1\}} \Upsilon(|z|^p) m_\alpha(\textup{d}z) 
    \le \sup_{\alpha\in\mathcal{A}} \sum_{n=1}^{\infty} \upsilon_n m_\alpha(\{z:|z|^p\ge n\}).
    \label{ineq:M_upperBound}
  \end{align}
  As a next step, we intend to find a way to control the quantity on the right-hand side of Inequality \eqref{ineq:M_upperBound} for sequences $(\upsilon_n)_{n\in\mathbb{N}}$ with desired properties, namely $(\upsilon_n)_{n\in\mathbb{N}}$ is non-decreasing and non-negative. 
  To this end, let us initially fix a decreasing sequence $(d_n)_{n\in\mathbb{N}}$ of positive numbers which is summable, \emph{e.g.} $d_n:=2^{-n}$ for every ${n\in\mathbb{N}}$. 
  We further define the set 
  \begin{align*}
    \mathcal{N}_n:=\Big\{k\in \mathbb{N}: \sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|^p\ge k\}} |z|^p m_\alpha(\textup{d}z) < d_n\Big\}, \text{ for every }n\in \mathbb{N}.
  \end{align*}
  In view of \eqref{Uniform_Integr_Limit_zero} it is immediate that for each $n\in\mathbb{N}$ the set $\mathcal{N}_n$ contains all but finitely many integers and that $(\mathcal{N}_n)_{n\in\mathbb{N}}$ is a decreasing sequence of sets.
  % This permits us to later apply a diagonal argument.
%   
% 
  Let $n\in\mathbb{N}$ and $c_n \in \mathcal{N}_n$.
  Then, observe that
  \begin{align*}
    \sum_{k=c_n}^{\infty} m_\alpha(\{z:|z|^p \ge k\}) 
    &\le c_n m_\alpha (\{z: |z|^p\ge c_n\}) + \sum_{k=c_n+1}^{\infty} m_\alpha(\{z: |z|^p\ge k\})\\
    &= \sum_{k=c_n}^{\infty} k m_\alpha(\{z: k\le |z|^p <k+1\})\\
    &\le \int_{\{z:|z|^p\ge c_n\}} |z|^p m_\alpha(\textup{d}z)<d_n.
  \end{align*}
In other words, by applying a diagonal argument, we can choose an increasing sequence $(c_n)_{n\in\mathbb{N}}$,\footnote{By increasing we mean $c_{n}<c_{n+1}$ for every $n\in\mathbb{N}$. Hence, $c_n\ge n$ and consequently $\lim_{n\to+\infty} c_n=+\infty$.} such that $c_n\in\mathcal{N}_n$ for every $n\in\mathbb{N}$,  in order to obtain
 \begin{align*}
  \sup_{\alpha \in\mathcal{A}}\sum_{n=1}^{\infty} \sum_{k=c_n}^{\infty} m_\alpha(\{z:|z|^p \ge k\}) <\sum_{n=1}^{\infty} d_n <+\infty.
 \end{align*}
 It is only left to observe that the double series can be written as a series of the form 
 $\sum_{k=1}^{\infty} \upsilon_k m_\alpha(\{z:|z|^p \ge k\})$, where 
 \begin{align*}
   \upsilon_k := |\{n\in\mathbb{N} : c_n\le k\}|,\footnotemark \text{ for every }k\in\mathbb{N};
 \end{align*}%
 \footnotetext{\label{footnote:comparison_of_upsilon_n}Since we chose the sequence $(c_n)_{n\in\mathbb{N}}$ to be increasing, we immediately have that $\upsilon_n\le \upsilon_{n+1}\le \upsilon_n +1$, for every $n\in\mathbb{N}$, where exactly one of the comparisons is a true equality.}
  $|A|$ denotes the cardinality of the set $A$.
% 
% 
 % the quantity $\upsilon_k$ equals the cardinality of the set $\{n\in\mathbb{N} : c_n\le k\}$,. 
 The equivalence has been proven. 
\end{proof}	



% \begin{proof}[Proof of \cref{prop:UI_Young_p_equals_0}]
%   One has simply to notationally modify the proof of \cref{prop:UI_Young} as follows:
%   \begin{enumerate}[label=\textbullet]
%    \item For the necessity part, instead of the property $\frac{\Upsilon(x)}{x}\ge K$, one should use the property $\Upsilon(x)\ge K$ and integrate the function $z\mapsto \Upsilon(|z|)$ over the set $\{z:|z|>R\}$.
%    \item For the sufficiency part, the integration is taking place over sets of the form $\{n\le |z|<n+1\}$ or $\{z:|z|\ge n\}$, for $n\in\mathbb{N}$, and the Young function $\Upsilon$ is evaluated at $|z|$ instead of $|z|^p$, whenever $\Upsilon$ serves as integrand.
%    As a result, sets of the form $\{z:|z|\ge n\}$ appear in the analogous to \eqref{ineq:M_upperBound} inequality as well as quantities of the form $m_\alpha(\{z:|z|\ge k\})$, $k\in\mathbb{N}$ and $\alpha\in\mathcal{A}$. 
%    In the same spirit,
%   \begin{align*}
%       \mathcal{N}_n:=
%       \Big\{k\in \mathbb{N}: \sup_{\alpha\in\mathcal{A}} m_\alpha(\{z:|z|\ge k\}) < d_n\Big\}, \text{ for every }n\in \mathbb{N}.
%     \end{align*}
%   \end{enumerate}
% \end{proof} 
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\subsection{Proof of Lemma \ref{lemma:UI_Young_improvement}}
\begin{remark}\label{rem:preparatory_proof}
  % \begin{enumerate}
  %   \item\label{rem:prep_proof:1}
      In order to prove \cref{lemma:UI_Young_improvement}, we will suitably choose the right-derivative of the Young function $\Upsilon$, denoted by $\upsilon$.
      In the next lines we will try to explain intuitively the procedure.
      To this end, we follow the notation introduced in the proof of \cref{prop:UI_Young}.
      In \citet[Lemme, p. 770]{meyer1978sur} it is described how to alter the sequence $(\upsilon_n)_{n\in\mathbb{N}}$ in order to obtain the stronger integrability described in \cref{corollary:UI_Young_improvement:StrongerIntegrability} and to obtain a moderate Young function.
      For the former, it is chosen a new sequence which is dominated by the sequence $(\upsilon_n)_{n\in\mathbb{N}}$, \emph{i.e.}, the right derivative is ``pushed downwards''.
      For the latter, the newly chosen sequence applies to intervals of increasing length, \emph{i.e.}, the right derivative is ``stretched''. 
      Inspired by \citet[Lemme, p. 770]{meyer1978sur}, we will initially follow the arguments presented there, but we will need go beyond \citet{meyer1978sur} in order to choose more conveniently some values. 
      Following the intuition introduced in the previous lines, the idea for proving \cref{lemma:UI_Young_improvement} is to repeatedly alter the right derivative of the Young function by initially properly ``pushing it downwards'', afterwards ``stretching it'', then making it continuous and finally smoothing it.
  %   \item\label{rem:prep_proof:2}   
  %     When we will be called to prove the regularity conditions for the non-local operator under interest, the quantities 
  %     \begin{align*}
  %       \Upsilon''(|y|^p)|y|^p \text{ and }\Upsilon'(|y|^p)|y|^{p-2}
  %     \end{align*}
  %     need to be controlled.
  %     The former can be universally, \emph{i.e.}, for any $p>0$, remedied by a condition as described in \cref{lemma:UI_Young_improvement}.\ref{lemma:UI_Young_improvement:second_derivative_properties}. 
  %     The latter is innocuous for $p\ge 2$, because $\Upsilon'$ is bounded in a neighborhood of zero.
  %     Consequently $\lim_{|y|\downarrow 0}\Upsilon'(|y|^p)|y|^{p-2}=0$, for $p>2$.
  %     Therefore, due to continuity of $\Upsilon'$, the quantity $\Upsilon'(|y|^p)|y|^{p-2}$ is bounded for any $p\ge 2$ on any compact interval containing $0$.
  %     However, for $p\in(0,2)$, we wish to avoid an``explosion'' because of the term $|y|^{p-2}$.
  %     In this case, we will need to further modify the (right) derivative in a neighborhood of $0$, so that the quantity $\Upsilon'(|y|^p)$ decreases faster than $|y|^{p-2}$; this justifies the existence of \cref{lemma:UI_Young_improvement}.\ref{lemma:UI_Young_improvement:p_smaller_than_2}.    
  % \end{enumerate}
\end{remark}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\begin{proof}[Proof of \cref{lemma:UI_Young_improvement}]
  In view of \cref{rem:preparatory_proof}, the current proof should be seen as a continuation of the proof of \cref{prop:UI_Young}.
  To this end, we will assume that the sequence $(\upsilon_n)_{n\in\mathbb{N}}$ is the one described in the second half of the proof of \cref{prop:UI_Young}.
  Without loss of generality, we may assume that $\upsilon_1 =1$.\footnote{Indeed, we can assign to $d_1$ (see proof of \cref{prop:UI_Young}) the value $2\sup_{\alpha\in\mathcal{A}}\int_{\{z:|z|\ge 1\}} |z|^p m_\alpha(\textup{d}z)$ and then choose $c_1=1$, since $\mathcal{N}_n=\mathbb{N}$.}
  Essentially, we will use the fact that 
  \begin{align}\label{property:upsilon_inequalities}
    \upsilon_k \le \upsilon_{k+1} \le \upsilon_{k} + 1, \text{ for every }k\in\mathbb{N},
  \end{align}
  where exactly one of the comparisons is a true equality; hence, the other is a strict inequality. 
  We choose to present the construction of the (right) derivative step by step, so that it is intuitively clear to the reader the final choice of the (right) derivative.
  As a result, we sacrifice the compactness of the proof.   

\vspace{0.5em}
 Following \citet{meyer1978sur}, we ``push downwards'' the right derivative by  passing to a new\footnote{This choice will later allow for the property $\lim_{R\to\infty} \sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|>R\}}\Upsilon(|z|^p) m_\alpha(\textup{d}z)=0,$ \emph{i.e.}, the uniform integrability of the function $\Upsilon(|z|^p)$ with respect to the family $(m_\alpha)_{\alpha\in\mathcal{A}}$. One can verify it by checking the proof of \cite[Lemme]{meyer1978sur} and modifying the arguments properly, \emph{i.e.}, as we did in the proof of the equivalence of \cref{prop:UI_Young}. For completeness, we provide the full details in the proof of \cref{corollary:UI_Young_improvement:StrongerIntegrability}.} 
 sequence $(\bar{\upsilon}_n)_{n\in\mathbb{N}}$ which is defined by $\bar{\upsilon}_n:=\sqrt{\upsilon_n}$.\footnote{Instead of the square root, it could be any increasing, positive function $g$ such that $\lim_{x\to\infty}\frac{g(x)}{x}=0$. Additional properties may be required later.} for every $n\in\mathbb{N}$.
 In view of \eqref{property:upsilon_inequalities} we get 
 \begin{align*}
    \bar{\upsilon}_n \le \bar{\upsilon}_{n+1}< \bar{\upsilon}_n+\frac{1}{2}, \text{ for every }n\in\mathbb{N}.
 \end{align*}
 Then, we define the function $\bar{\upsilon}$
  \begin{gather*}
    \bar{\upsilon}(x) := 
      \begin{cases}
        % \frac{1}{4},        &\text{ for }x\in[0,\frac{3}{2})\\
        % \frac{1}{2},        &\text{ for }x\in[\frac{3}{2},2)\\
        \frac{1}{2},        &\text{ for }x\in[0,2)\\
        \bar{\upsilon}_n,   &\text{ for }x\in[2^{n},2^{n+1}), n\in\mathbb{N}
      \end{cases}.
  \end{gather*}
 Obviously, the function $\bar{\upsilon}$ is right-continuous and non-decreasing.
 Recalling the description in \cref{rem:preparatory_proof}, the above definition amounts to ``stretching'' the right derivative.
 For the sake of unified notation, we re-define $\bar{\upsilon}_0:=\frac{1}{2}$, for which choice $\bar{\upsilon}_0<\bar{\upsilon}_1=\bar{\upsilon}_0+\frac{1}{2}$.


 \vspace{0.5em}
 We proceed by constructing a continuous function which is dominated by $\bar{\upsilon}$.
 To this end, we will linearly interpolate between suitable points.
 % On the interval $[0,2]$ the origin and the point $(2,\bar{\upsilon}_0)$ will be interpolated.
 % The rest interpolation points could be described as the right-end points of intervals of constancy of $\bar{\upsilon}$.
 % The precise arguments are presented in the next lines. 
 We start by defining the set 
 \begin{align*}
   \mathbb{K}:=\{k\in\mathbb{N}\backslash\{1\} : \upsilon_{k-1}<\upsilon_{k}\}=\{k\in\mathbb{N}\backslash\{1\} : \bar{\upsilon}_{k-1}<\bar{\upsilon}_{k}\};
 \end{align*}%
 let $(k_n)_{n\in\mathbb{N}}$ be the ordered enumeration of $\mathbb{K}$, \emph{i.e.}, $k_{n}<k_{n+1}$ for every $n\in\mathbb{N}$.
 Given the set $(k_n)_{n\in\mathbb{N}}$, we can alternatively write the function $\bar{\upsilon}$ as
 \begin{gather*}
    \bar{\upsilon}(x) := 
      \begin{cases}
        % \frac{1}{4},        &\text{ for }x\in[0,\frac{3}{2})\\
        % \frac{1}{2},        &\text{ for }x\in[\frac{3}{2},2)\\
        \frac{1}{2},        &\text{ for }x\in[0,2)\\
        \bar{\upsilon}_1,   &\text{ for }x\in[2,2^{k_1})\\
        \bar{\upsilon}_{k_n},   &\text{ for }x\in[2^{k_{n-1}},2^{k_n}) \text{ and } n\ge2
      \end{cases}.
  \end{gather*}
 We define now the function
 \begin{align*}
   \hat{\upsilon}(x) :=
    \begin{cases}
      % \frac{1}{6}x,                                 &\text{for }x\in[0,\frac{3}{2})\\
      % \frac{1}{2}(x-1),                             &\text{for }x\in[\frac{3}{2},2)\\
      \frac{1}{4}x,                             &\text{for }x\in[0,2)\\
      \frac{1}{2} + \frac{\bar{\upsilon}_1}{2 (2^{k_1}-2)}(x-2),   &\text{for }x\in[2,2^{k_1})\\
      \bar{\upsilon}_{k_n} +\frac{ \bar{\upsilon}_{k_{n+1}}-\bar{\upsilon}_{k_{n}}}{2^{k_{n+1}}-2^{k_n}}(x - 2^{k_n}), 
                                                    &\text{for }x\in[2^{k_n},2^{k_{n+1}}), n>1
    \end{cases}.
 \end{align*}

Some remarks are in order:
\begin{enumerate}[label=(\arabic*)]
  \item $\upsilon_{1}= \bar{\upsilon}_{1}=1$, $\upsilon_{k_1}=2$ and $\upsilon_{k_{n+1}} - \upsilon_{k_n}=1,$ for every $n\in\mathbb{N}$.
  \item The function $\hat{\upsilon}$ is continuous
  % , convex on $[0,2]$ 
  and concave on $[0+\infty)$. 
  This can easily be seen, since $\hat{\upsilon}$ is piecewise linear with %increasing slopes on $(0,2)$ and 
  decreasing slopes on $(0,+\infty)$. 
  Indeed, one can see that the slopes are decreasing by examining the sequence of nominators and denominators.
  More precisely, we have (by definition) that
  \begin{align*}
       \bar{\upsilon}_{k_{n+1}} = \sqrt{\upsilon_{k_{n+1}}} =\sqrt{\upsilon_{k_{n}}+1}, \text{ for every }n\in\mathbb{N}.  
  \end{align*}
  Given that the function $(1,+\infty)\ni x\mapsto \sqrt{x+1}-\sqrt{x}$ is decreasing and bounded between $0$ and $\frac{1}{2}$, we have that 
  \begin{align}\label{property:diff_bar_upsilon}
    0<\bar{\upsilon}_{k_{n+2}}-\bar{\upsilon}_{k_{n+1}} \le \bar{\upsilon}_{k_{n+1}} - \bar{\upsilon}_{k_{n}}<\frac{1}{2} = \frac{\bar{\upsilon}_1}{2} = \bar{\upsilon}_0, \text{ for every }n\in\mathbb{N}.
  \end{align}
  Moreover, for every $n\in\mathbb{N}$,
  \begin{gather*}
     2^{k_2}-2^{k_1}  > 2^{k_1} - 2
  \shortintertext{as well as}
    2^{k_{n+2}} - 2^{k_{n+1}} 
      = 2^{k_{n+1}}(2^{k_{n+2}-k_{n+1}} - 1) 
      > 2^{k_{n+1}}(1 - 2^{k_{n}-k_{n+1}})
      =2^{k_{n+1}} - 2^{k_{n}}.
  \end{gather*}
  Hence, $\frac{ \bar{\upsilon}_{k_{2}}-\bar{\upsilon}_{k_{1}}}{2^{k_{2}}-2^{k_1}} <\frac{ \bar{\upsilon}_{k_1}}{2(2^{k_1}-2)}\le \frac{1}{4} $ and the sequence $(\frac{ \bar{\upsilon}_{k_{n+1}}-\bar{\upsilon}_{k_{n}}}{2^{k_{n+1}}-2^{k_n}})_{n\in\mathbb{N}}$ is decreasing, since the nominators decrease and the denominators increase, as $n$ increases.
\end{enumerate}


\vspace{0.5em}
We proceed to define the derivative of the the desired Young function, but we need to treat separately the cases $p\ge 2$ and $p\in(0,2)$:

\vspace{0.5em}
{\tiny $\blacksquare$} $p\ge 2$. We will smooth the function $\hat{\upsilon}$\footnote{The function $\hat{\upsilon}$ is continuous, but not everywhere differentiable. Hence, the associated Young function will not be twice continuously differentiable.}  by standard tools.
More precisely, for $0<\varepsilon<\frac{1}{2^3}$ we use the standard mollifier $\eta_{\varepsilon}$, \emph{i.e.},
\begin{align*}
 \eta_\varepsilon(x):= \frac{C}{\varepsilon} \exp\Big(\frac{1}{\varepsilon^{-2}x^2-1}\Big) \mathds{1}_{[-\varepsilon,\varepsilon]}(x),
\end{align*}
where $C$ is the normalizing constant.
We define
  \begin{align*}
   \hat{\upsilon}_\varepsilon(x) :=
   \begin{cases}
     \hat{\upsilon}(x), &\text{ for }x\in[0,1]\\
     \displaystyle \int_{[-\varepsilon, \varepsilon]} \hat{\upsilon}_\varepsilon (x+y) \eta_\varepsilon(y)\textup{d}y, &\text{ for } x> 1.
   \end{cases}
  \end{align*}
Hereinafter, we \emph{fix} an $0<\varepsilon<\frac{1}{2^3}$ such that
\begin{align}\label{property:error_bound}
 | \hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x)|<\frac{1}{2^4}, \text{ for every }x\in[0,+\infty).
\end{align}
We present in \cref{comput:error_hat_u} the elementary arguments for the determination of an $\varepsilon$ with the aforementioned property, despite this can be seen as a special case of a general approximation result.
The function $\hat{\upsilon}_\varepsilon$ (for the $\varepsilon$ we fixed) will be the derivative of the desired Young function $\Upsilon$.
Before we prove that $\Upsilon$ possesses the desired properties, some remarks are in order:
\begin{enumerate}[label=(\arabic*)]
\setcounter{enumi}{2}
 \item $\hat{\upsilon}_{\varepsilon}(0)=0$ and $\hat{\upsilon}_{\varepsilon}(x)>0$ for $x>0$. 

 \item\label{property:identical_on_linear} For $x\in(1,2-\varepsilon)\cup(2+\varepsilon,2^{k_1}-\varepsilon) \cup \big(\bigcup_{k\in\mathbb{N}} (2^{k_n}+\varepsilon, 2^{k_{n+1}}-\varepsilon)\big)$ 
 it is true that $\hat{\upsilon}_\varepsilon(x)=\hat{\upsilon}(x)$, because of the linearity of $\hat{\upsilon}$ on the interval $(x-\varepsilon,x+\varepsilon)$.

\item
% On $(0,2-\varepsilon)$, the function $\hat{\upsilon}_\varepsilon$ is convex, with $\hat{\upsilon}_\varepsilon \ge \hat{\upsilon}$, while 
On $(0,+\infty)$ the function $\hat{\upsilon}_\varepsilon$ is concave, with $\hat{\upsilon}_\varepsilon \le \hat{\upsilon}$.
The concavity of $\hat{\upsilon}_\varepsilon$ is inherited from the concavity of $\hat{\upsilon}$. 
The domination can be easily proven using the piecewise linearity of $\hat{\upsilon}_\varepsilon$, the fact that the slopes are non-increasing and the definition of the mollification.\footnote{In \cref{comput:error_hat_u} we will need to estimate the difference $|\hat{\upsilon}(x) -\hat{\upsilon}_\varepsilon(x)|$, so we postpone until then the computations.}

% and infinitely differentiable on $(0,\infty)$.

\item\label{property:second_derivative_finally_decreasing} The function $\hat{\upsilon}_\varepsilon$ is infinitely differentiable.
In particular, its first derivative is positive and non-increasing due to concavity. 
\end{enumerate}



















% Summing up, for $x\in (x_0-\varepsilon, x_0+\varepsilon)$ it holds
% \begin{align*}
%   &\sup_{x\in (x_0-\varepsilon, x_0+\varepsilon)} |\hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) |\\
%     &\hspace{2em}=\max\big\{\sup_{x\in (x_0-\varepsilon, x_0]} |\hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x)|, \sup_{x\in [x_0, x_0+\varepsilon)} |\hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) |\big\}  \\
%     &\hspace{2em}=\max\Big\{\sup_{x\in (x_0-\varepsilon, x_0)} (\lambda_l-\lambda_r) \Big|\int_{[-\varepsilon,x_0-x]} y\eta_\varepsilon (y) \textup{d}y\Big|, 
%                 \sup_{x\in [x_0, x_0+\varepsilon)} (\lambda_l-\lambda_r) \Big|\int_{[x_0-x,\varepsilon]} y\eta_\varepsilon (y) \textup{d}y\Big|\Big\}  \\
%     &\hspace{2em}= (\lambda_l-\lambda_r)\cdot \Big|\int_{(0,\varepsilon)} y\eta_\varepsilon (y) \textup{d}y\Big| 
%                  = |\hat{\upsilon}(x_0) - \hat{\upsilon}_\varepsilon(x_0) |
%                  \overset{\eqref{property:bound_of_error}}{<}\frac{1}{2^4}, \text{for any }x_0.  
% \end{align*}
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
\vspace{0.5em}
The function 
\begin{align*}
  \Upsilon(x) := \int_{[0,x]} \hat{\upsilon}_\varepsilon (u) \textup{d}u, \text{ for }x\ge 0,
\end{align*}
satisfies the claimed properties: 
\begin{enumerate}
  \item[\ref{lemma:UI_Young_improvement:moderate_C2}] Since $\hat{\upsilon}_\varepsilon$ is infinitely differentiable, so is $\Upsilon$. 
  In particular, $\Upsilon$ is twice continuously differentiable.


  \vspace{0.5em}
  We prove now that $\Upsilon$ is moderate, \emph{i.e.},
  \begin{align*}
    \bar{c}_{\Upsilon} = \sup_{x>0} \frac{x \hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)} < +\infty.
  \end{align*}
  We will consider the three subintervals $(0,2-\varepsilon]$, $[2-\varepsilon,2^{k_1}]$ and $[2^{k_1},+\infty)$. 
  For $x\in(0,2-\varepsilon)$ we have 
  \begin{align*}
    \sup_{x\in(0,2-\varepsilon]} \frac{x \hat{\upsilon}(x)}{\Upsilon(x)} = \frac{\frac{1}{6}x^2}{\frac{1}{6}\frac{1}{2}x^2} = 2.
  \end{align*}
  For $x\in[2-\varepsilon,2^{k_1}]$, we have that both nominator and denominator are continuous functions, bounded away from $0$ and considered on a compact interval. 
  Hence
 \begin{align*}
    \sup_{x\in[2-\varepsilon,2^{k_1}]} \frac{x \hat{\upsilon}(x)}{\Upsilon(x)} <+\infty.
  \end{align*}
  For $x\in[2^{k_1},+\infty]$, we will initially prove that there exists a constant $K_2>1$ such that
  \begin{align}\label{property:moderate_derivative}
    \hat{\upsilon}_\varepsilon(2x) \le K_2 \hat{\upsilon}_\varepsilon(x).
  \end{align}
  Indeed, let $x\ge 2^{k_1}$.
  Then, there exists unique $n\ge 2$ such that $2x\in(2^{k_{n-1}},2^{k_{n}}]$, for $k_{n-1},k_{n}\in\mathbb{K}$.
  Then, 
  \begin{enumerate}[label=(\alph*)]
    \item  either $x\in[2^{k_{n-1}},2^{k_n})$, in which case
    \begin{align*}
        \hat{\upsilon}(2x) = \hat{\upsilon}(2x) - \hat{\upsilon}(x) + \hat{\upsilon}(x)
        \overset{\eqref{property:diff_bar_upsilon}}{<}
        \frac{1}{2} + \hat{\upsilon}(x)<2\hat{\upsilon}(x),
    \end{align*}
    \emph{i.e.}, $K_2=2$,

    \item  or $x\in[2^{k_{n-2}},2^{k_{n-1}})$, in which case
    \begin{align*}
        \hat{\upsilon}(2x) = \hat{\upsilon}(2x) - \hat{\upsilon}(2^{k_{n-1}}) + \hat{\upsilon}(2^{k_{n-1}})- \hat{\upsilon}(x) + \hat{\upsilon}(x)
        \overset{\eqref{property:diff_bar_upsilon}}{<}
        2\frac{1}{2} + \hat{\upsilon}(x)<3\hat{\upsilon}(x),
    \end{align*}
    \emph{i.e.}, $K_2=3$.
  \end{enumerate}
  In total, for $K_2=3$ we have that \eqref{property:moderate_derivative} holds for any $x\ge 2^{k_1}$.
  This allows us to derive, for $x\ge 2^{k_1}$,
  \begin{align*}
    x\hat{\upsilon}_\varepsilon(x) 
      &\le \int_{[x,2x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z 
        = \int_{[0,2x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z - \int_{[0,x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z\\
      & = \int_{[0,x]}2\hat{\upsilon}_\varepsilon(2w)\textup{d}w - \int_{[0,x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z
        \le \int_{[0,x]}2K_2\hat{\upsilon}_\varepsilon(w)\textup{d}w - \int_{[0,x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z\\
      &=(2K_2-1)\Upsilon(x),
  \end{align*}
  where in the first inequality we used that the $\hat{\upsilon}_\varepsilon$ is increasing.
  We have from the inequalities above that 
  \begin{align*}
      \sup_{x\ge 2^{k_1}} \frac{x\hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)} \le 2K_2-1=5<+\infty.
    \end{align*}
   To sum up, we have proven that 
   \begin{align*}
     \bar{c}_\Upsilon = \max\Big\{ 
          \sup_{x\in(0,2-\varepsilon]} \frac{x \hat{\upsilon}(x)}{\Upsilon(x)},
          \sup_{x\in[2-\varepsilon,2^{k_1}]} \frac{x \hat{\upsilon}(x)}{\Upsilon(x)},
          \sup_{x\ge 2^{k_1}} \frac{x\hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)}
          \Big\}
          <+\infty.
   \end{align*}




   \item[\ref{lemma:UI_Young_improvement:second_derivative_properties}] We have argued in \ref{property:second_derivative_finally_decreasing} that $\hat{\upsilon}_\varepsilon'=\Upsilon''$ is positive and finally non-increasing. 
   Its continuity allows us to conclude that $\Upsilon''$ is bounded.
   
   \vspace{0.5em}
   We proceed to prove \eqref{property:second_derivative_faster_than_identity}, we will consider three cases:
   \begin{enumerate}[label=\textbullet]
     \item 
        $x\in[2^{k_n}+\varepsilon,2^{k_{n+1}}]$, for some $n\in\mathbb{N}$:
        then, in view of \ref{property:second_derivative_finally_decreasing},
        \begin{align*}
          x\Upsilon''(x) 
            &\le  2^{k_{n+1}}\Upsilon''(2^{k_{n}}+\varepsilon)
             \le  2^{k_{n+1}}\frac{\bar{\upsilon}_{k_{n+1}}-\bar{\upsilon}_{k_{n}}}{2^{k_{n+1}} - 2^{k_{n}}}
            \overset{\eqref{property:diff_bar_upsilon}}{<}\frac{1}{1-2^{k_n-k_{n+1}}} \frac{1}{2}\le 1.
        \end{align*}

      \item 
       $x\in[2^{k_n},2^{k_n}+\varepsilon]$, for $n\in\mathbb{N}$:
        then
        \begin{align*}
          x\Upsilon''(x)
            \overset{\ref{property:second_derivative_finally_decreasing}}{<} 
            (2^{k_n} + \varepsilon) \Upsilon''(2^{k_n})
            \le 
            (2^{k_n} + \varepsilon) \frac{\bar{\upsilon}_{k_{n}}-\bar{\upsilon}_{k_{n-1}}}{2^{k_{n}} - 2^{k_{n-1}}}
            \overset{\eqref{property:diff_bar_upsilon}}{<} (\frac{1}{2}+ \frac{1}{2^3})\frac{1}{1-2^{k_{n-1}-k_n}} <2.  
        \end{align*}

      \item 
      $x\in[0,2^{k_1}]$: we recall that by definition, $k_1\ge2$ and that $\overline{\upsilon}_{k_1}=1$.
      Then, 
      \begin{align*}
        x\Upsilon''(x) \le 
        \begin{cases}
          \frac{1}{2}, &\text{for }x\in[0,2)\\
          \frac{2^{k_1}}{2(2^{k_1}-2)}, &\text{for }x\in(2,2^{k_1}]
        \end{cases}
        \le 1.
      \end{align*}
    In total, the constant $C$ for the case $p\ge 2$ is $2$.
%
%
    \item[\ref{lemma:UI_Young_improvement:submultiplicativity}] 
    We are going to utilize \citet[Chapter I, Theorem 5.2, p.32]{krasnoselskii1961},\footnote{Our construction satisfies the properties of an $N-$function, as defined in \cite[Chapter I, Section 3, p.6]{krasnoselskii1961}. In any case, the behavior of the function $\Upsilon$ in a neighborhood of $0$, does not affect the ``final'' behavior of the function $\Upsilon$.} whose hypothesis is satisfied, \emph{i.e.}, there exists $t_0>0$ such that 
    \begin{align}
        [t_0,+\infty) \ni t \mapsto \frac{t \Upsilon''(t)}{\Upsilon'(t)}=\frac{t \hat{\upsilon}_\varepsilon'(t)}{\hat{\upsilon}_\varepsilon(t)} \text{ is non-increasing}.
        \label{def:criterion_submultiplicative}
    \end{align}
    Indeed, in view of \ref{lemma:UI_Young_improvement:second_derivative_properties}, \emph{i.e.}, the nominator of the fraction is bounded, and the fact that $\hat{\upsilon}_\varepsilon$ is increasing, 
    there exists $t_0\in(2^{k_1},2^{k_2})$ such that $\hat{\upsilon}_\varepsilon(t)> 2$, where $2$ is the bound extracted in \ref{lemma:UI_Young_improvement:second_derivative_properties}.
    Therefore, the function in \eqref{def:criterion_submultiplicative} is finally decreasing.
   \end{enumerate}

\end{enumerate}



{\tiny $\blacksquare$} $p\in(0,2)$. Before we smooth the function $\hat{\upsilon}$, we will need to suitably modify it on $[0,2]$.
We have in mind that \eqref{property:second_derivative_faster_to_0} has to hold. 
To this end, we will choose the derivative $\hat{\upsilon}$ to behave in a neighborhood of $0$ as a power function, say of power $q$, so that 
\begin{align*}
  \lim_{x\downarrow 0}(x^p)^qx^{p-2}=\lim_{x\downarrow 0}(x^p)^{q-1}x^{2p-2}=0.
\end{align*}
\cref{lem:def_q_for_smoothness} verifies that there is a legitimate choice of $q$ for each $p\in(0,2)$:
% We choose $q$ so that $pq+p-2=2$, \emph{i.e.}, we define 
\begin{align}\label{def:q}
  q:=\frac{4}{p}-1, \text{ for }p\in(0,2).
\end{align}
Observe that for the choice of $q$ it holds $pq+p-2=p(q-1)+2p-2=2$.
Additionally, for 
\begin{align*}
   x_0(p):=\big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}\in(0,\frac{3}{2})
\end{align*}
and for $[0,\frac{3}{2}]\ni x\overset{f}{\mapsto} x^q$ it holds $f'(x_0)=\frac{1}{6}$.
Moreover, 
\begin{gather*}
  0<f(x_0) = x_0^q 
    = \Big(\frac{1}{6q}\Big)^{\frac{q}{q-1}} 
    =\Big(\frac{p}{6(4-p)}\Big)^{\frac{4-p}{4-2p}}
    <\frac{p}{6(4-p)}
    \le \frac{1}{6}
    \shortintertext{as well as}
  0<f(x_0) + \frac{1}{6} (\frac{5}{4}-x_0)
    <\frac{1}{6}+\frac{1}{6} \frac{5}{4} = \frac{1}{6} \frac{9}{4} = \frac{3}{8}<\frac{1}{2}
\end{gather*}
where we used that $\frac{p}{6(4-p)}<1$ and that $\frac{4-p}{4-2p}>1$.

% Furthermore, we seek the point $x_0=x_0(p)\in(0,\frac{3}{2})$ (if it exists) for which
% \begin{align*}
%    f'(x_0)=\frac{1}{6}
%    \Leftrightarrow q x_0^{q-1}=\frac{1}{6}
%    \overset{(q>1)}{\Leftrightarrow} x_0^{q-1}=\frac{1}{6q}
%    {\Leftrightarrow} x_0=\Big(\frac{1}{6q}\Big)^{\frac{1}{q-1}} = \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}.
% \end{align*}
% The point $x_0$ lies, indeed, in the domain of $f$.
% We can compute the respective limits
% \begin{align*}
%   \lim_{p\downarrow 0} x_0(p) 
%     & = \lim_{p\downarrow 0} \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}
%       = \lim_{p\downarrow 0} \exp\big(\frac{p}{4-2p}\ln(\frac{p}{6(4-p)})\big)\\
%     & = \lim_{z\downarrow 0} \exp\big(z\ln(z)\big) = 1
% \end{align*}
% and 
% \begin{align*}
%   \lim_{p\uparrow 2} x_0(p) 
%     & = \lim_{p\uparrow 2} \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}} = 0.
% \end{align*}
% Moreover, 
% \begin{gather*}
%   0<f(x_0) = x_0^q 
%     = \Big(\frac{1}{6q}\Big)^{\frac{q}{q-1}} 
%     =\Big(\frac{p}{6(4-p)}\Big)^{\frac{4-p}{4-2p}}
%     <\frac{p}{6(4-p)}
%     \le \frac{1}{6}
%     \shortintertext{as well as}
%   0<f(x_0) + \frac{1}{6} (\frac{5}{4}-x_0)
%     <\frac{1}{6}+\frac{1}{6} \frac{5}{4} = \frac{1}{6} \frac{9}{4} = \frac{3}{8}<\frac{1}{2}
% \end{gather*}
% where we used that $\frac{p}{6(4-p)}<1$ and that $\frac{4-p}{4-2p}>1$.
% The last computations will permit us to linearly interpolate, with positive slopes, on the interval $[x_0,2]$.
The above properties permit us to \emph{re}-define the function $\hat{\upsilon}$ on $[0,2]$ as follows
\begin{align}
  \hat{\upsilon}(x):=
  \begin{cases}
    f(x), &\text{for }x\in[0,x_0]\\
    f(x_0) + \frac{1}{6} (x-x_0), &\text{for }x\in(x_0,\frac{5}{4}]\\ 
    % f(x_0) + \frac{1}{6} (\frac{5}{4}-x_0) + 4[\frac{1}{2} - f(x_0) + \frac{1}{6} (\frac{5}{4}-x_0)](x-\frac{5}{4}), &\text{for }x\in(\frac{5}{4},\frac{3}{2}]\\ 
    \hat{\upsilon}(\frac{5}{4}) + \frac{4}{3}\big[\frac{1}{2} - \hat{\upsilon}(\frac{5}{4})\big](x-\frac{5}{4}), &\text{for }x\in(\frac{5}{4},2]\\ 
    % \text{as before}, &\text{for }x\ge2
  \end{cases}.
\end{align}
We can easily verify that the redefined function $\hat{\upsilon}$ is continuous on $[0,+\infty)$ and continuously differentiable on $(0,\frac{5}{4})$.
For $0<\varepsilon<\frac{1}{2^4}$ we define
\begin{align*}
\hat{\upsilon}_\varepsilon(x) :=
  \begin{cases}
    \hat{\upsilon}(x), &\text{for } x\in [0,\frac{5}{4}-\varepsilon]\\
     \displaystyle \int_{[-\varepsilon, \varepsilon]} \hat{\upsilon}_\varepsilon (x+y) \eta_\varepsilon(y)\textup{d}y, &\text{ for } x> \frac{5}{4}-\varepsilon
  \end{cases}.
\end{align*}
The function 
\begin{align*}
  \Upsilon(x) := \int_{[0,x]} \hat{\upsilon}_\varepsilon (u) \textup{d}u, \text{ for }x\ge 0,
\end{align*}
satisfies the claimed properties:\footnote{We will focus our attention on the interval $[0,2^{k_1}]$, since for the rest we can use the analogous arguments presented for the case $p\ge 2$. The only difference is the upper bound for $\varepsilon$.}
\begin{enumerate}
    \item[\ref{lemma:UI_Young_improvement:moderate_C2}]
    The function $\hat{\upsilon}_\varepsilon$ is continuously differentiable on every point of $(0,x_0]$ and infinitely differentiable on every point of $(x_0,2^{k_1}]$.
    Hence $\Upsilon$ is twice differentiable at $x_0$.

    \vspace{0.5em}
    In order to prove that $\Upsilon$ is moderate, we will work separately on the intervals $(0,x_0]$ and $[x_0,2^{k_1}]$.
    For the former interval, immediate computations verify
    \begin{align*}
      \sup_{x\in(0,x_0]}\frac{x\hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)} = q+1<+\infty.
    \end{align*}
    For the latter interval, we use the continuity of $x\mapsto x\hat{\upsilon}_\varepsilon$ and $\Upsilon$, the compactness of the interval under consideration as well as the fact that $0<\inf_{x\in[x_0,2^{k_1}]}\Upsilon(x),\sup_{x\in[x_0,2^{k_1}]}\Upsilon(x)<+\infty$.
    In total,
    \begin{align*}
        \bar{c}_{\Upsilon} =\sup_{x>0} \frac{x\hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)}<+\infty.
    \end{align*}

    \item[\ref{lemma:UI_Young_improvement:second_derivative_properties}] 
    We can readily adapt the arguments we used in the case $p\ge 2$.

    \item[\ref{lemma:UI_Young_improvement:submultiplicativity}] 
    On $[2,+\infty)$, the derivative $\hat{\upsilon}_\varepsilon$ is identical to the derivative constructed for the case $p\ge 2$.
    Therefore, for the case we are examining now we have that $x\hat{\upsilon}_\varepsilon'(x)\le 2$, for $x\in[2,+\infty)$.
    In other words, we for the same $t_0$, as in the case $p\ge 2$, the function  
    \begin{align*}
        [t_0,+\infty) \ni t \longmapsto \frac{t \Upsilon''(t)}{\Upsilon'(t)} \text{ is non-increasing}.
    \end{align*}
    We conclude in view of \citet[Chapter I, Theorem 5.2, p.32]{krasnoselskii1961}.

    \item[\ref{lemma:UI_Young_improvement:p_smaller_than_2}]
    This property is true because of the choice of $q$; see \eqref{def:q} and the comment following it.

\end{enumerate}
\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{lemma}\label{comput:error_hat_u}
  There exists $0<\varepsilon<\frac{1}{2^3}$ for which the bound \eqref{property:error_bound} holds.
\end{lemma}
\begin{proof}
Let us define the auxiliary function
\begin{align*}
  g(x):= \hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x), \text{for }x>0.
\end{align*}
Let $x_0\in\{2\}\cup\{2^{k_n}:n\in\mathbb{N}\}$.
Then for any such $x_0$ we denote by $\lambda_l x +\beta_l$ the representation of the affine part of $\hat{\upsilon}$ associated to the subinterval on the left of $x_0$ and by $\lambda_r x +\beta_r$ the representation of the affine part of $\hat{\upsilon}$ associated to the subinterval on the right of $x_0$.
Due to continuity of $\hat{\upsilon}$
\begin{align}\label{equality:lambda_beta}
  \lambda_l x_0 +\beta_l=\lambda_r x_0 +\beta_r
  \Leftrightarrow 
  \beta_l - \beta_r = (\lambda_r - \lambda_l)x_0.
\end{align}
Then, for $0<\varepsilon<\frac{1}{2^3}$
\begin{align*}
    g(x_0)=\hat{\upsilon}(x_0) - \hat{\upsilon}_\varepsilon(x_0) 
      &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
      (\lambda_l x_0 +\beta_l) - \int_{[-\varepsilon,0]} [\lambda_l (x_0+y) +\beta_l]\eta_\varepsilon(y) \textup{d}y - \int_{[0,\varepsilon]} [\lambda_r (x_0+y) +\beta_r]\eta_\varepsilon(y) \textup{d}y \\
      &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
      \int_{[-\varepsilon,\varepsilon]}[\lambda_l (x_0+y) +\beta_l]\eta_\varepsilon(y)\textup{d}y 
        - \int_{[-\varepsilon,0]} [\lambda_l (x_0+y) +\beta_l]\eta_\varepsilon(y) \textup{d}y \\
      &\hspace{1em}  - \int_{[0,\varepsilon]} [\lambda_r (x_0+y) +\beta_r]\eta_\varepsilon(y) \textup{d}y \\
      &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
      \int_{[0,\varepsilon]} [(\lambda_l - \lambda_r) (x_0+y) +(\beta_l - \beta_r)]\eta_\varepsilon(y) \textup{d}y \\
      &\overset{\eqref{equality:lambda_beta}}{=} 
      (\lambda_l - \lambda_r) \int_{[0,\varepsilon]} y\eta_\varepsilon(y) \textup{d}y \ge 0,
\end{align*}
given that $\lambda_l\ge\lambda_r$,
The quantity $g(x_0)$ can vanish only  in the case $\lambda_l=\lambda_r$.
Hence,
\begin{align*}
  0\le \lambda_l - \lambda_r
  \le \max\Big\{
    \frac{1}{4}-\frac{1}{2(2^{k_1}-2)}, 
    \sup_{n\in\mathbb{N}}\{\frac{ \bar{\upsilon}_{k_{n+1}}-\bar{\upsilon}_{k_{n}}}{2^{k_{n+1}}-2^{k_n}}
                          -\frac{ \bar{\upsilon}_{k_{n+2}}-\bar{\upsilon}_{k_{n+1}}}{2^{k_{n+2}}-2^{k_{n+1}}}\}
    \Big\}
  < \frac{1}{4}
\end{align*}
and given also that 
\begin{align*}
  \lim_{\varepsilon \downarrow 0}\int_{[0,\varepsilon]} y\eta_\varepsilon(y) \textup{d}y=0,
\end{align*}
we can chose $0<\varepsilon<\frac{1}{2^3}$ such that 
\begin{align*}
  \int_{[0,\varepsilon]} y\eta_\varepsilon(y) \textup{d}y \le \frac{1}{2^2}.
 \end{align*}
In total, we have 
\begin{align}\label{property:bound_of_error}
  \sup\{\hat{\upsilon}(x_0) - \hat{\upsilon}_\varepsilon(x_0) :x_0\in\{2\}\cup\{2^{k_n}:n\in\mathbb{N}\} \}<\frac{1}{2^4}.
\end{align}
%
%
% 
% 
% 
% 
We will proceed to estimate the function $g$ in the rest points of its domain:
\begin{enumerate}[label=\textbullet]
  \item 
For $x\in(1,2-\varepsilon)\cup(2+\varepsilon,2^{k_1}-\varepsilon) \cup \big(\bigcup_{k\in\mathbb{N}} (2^{k_n}+\varepsilon, 2^{k_{n+1}}-\varepsilon)\big)$, which is the set considered in \ref{property:identical_on_linear}, we have that $g(x)=0$. 

  \item 
For $x\in(x_0-\varepsilon,x_0]$ it holds
\begin{align*}
  g(x) = \hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) 
  &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
  \lambda_l x + \beta_l 
    - \int_{[-\varepsilon,x_0-x]} [\lambda_l(x+y)+\beta_l]\eta_\varepsilon(y)\textup{d}y
    - \int_{[x_0-x,\varepsilon]} [\lambda_r(x+y)+\beta_r]\eta_\varepsilon(y)\textup{d}y\\
  &\overset{\phantom{\eqref{equality:lambda_beta}}}{=}
   \int_{[x_0-x,\varepsilon]} [(\lambda_l-\lambda_r)(x+y)+(\beta_l-\beta_r)]\eta_\varepsilon(y)\textup{d}y\\
  &\overset{\eqref{equality:lambda_beta}}{=}
   (\lambda_l-\lambda_r) \int_{[x_0-x,\varepsilon]} [(x+y)-x_0 ]\eta_\varepsilon(y)\textup{d}y\ge0,
\end{align*}
since $(x+y)-x_0\ge 0$ for $y\in[x_0-x,\varepsilon]$ and the assumption on $x$.
Moreover, 
\begin{align*}
 g'(x) 
 &= (\lambda_l-\lambda_r) \int_{[x_0-x,\varepsilon]} \eta_\varepsilon(y)\textup{d}y
  + (\lambda_l-\lambda_r) x \eta_\varepsilon(x_0-x) +(-x)\eta_\varepsilon(x_0-x)\\
 & = (\lambda_l-\lambda_r) \int_{[x_0-x,\varepsilon]} \eta_\varepsilon(y)\textup{d}y >0,
\end{align*} 
with $\lim_{x\downarrow x_0-\varepsilon}g(x)=0$ and $\lim_{x\uparrow x_0}g(x)=g(x_0)$. 
In other words, on $(x_0-\varepsilon,x_0]$ the function $g$ attains its maximum at $x_0$. 

  \item For $x\in(x_0,x_0+\varepsilon]$ it holds
\begin{align*}
  g(x)= \hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) 
  &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
  \lambda_r x + \beta_r 
    - \int_{[-\varepsilon,x_0-x]} [\lambda_l(x+y)+\beta_l]\eta_\varepsilon(y)\textup{d}y
    - \int_{[x_0-x,\varepsilon]} [\lambda_r(x+y)+\beta_r]\eta_\varepsilon(y)\textup{d}y\\
  &\overset{\phantom{\eqref{equality:lambda_beta}}}{=}
   \int_{[-\varepsilon,x_0-x]} [(\lambda_r-\lambda_l)(x+y)+(\beta_r-\beta_l)]\eta_\varepsilon(y)\textup{d}y\\
  &\overset{\eqref{equality:lambda_beta}}{=}
   (\lambda_r-\lambda_l) \int_{[-\varepsilon,x_0-x]} [(x+y)-x_0 ]\eta_\varepsilon(y)\textup{d}y\ge0,
\end{align*}
since $\lambda_r-\lambda_l\le 0$, $(x+y)-x_0\le 0$ for $y\in[x_0-x,\varepsilon]$ and the assumption on $x$.
Moreover, 
\begin{align*}
 g'(x) 
 &= (\lambda_r-\lambda_l) \int_{[x_0-x,\varepsilon]} \eta_\varepsilon(y)\textup{d}y
  + (\lambda_r-\lambda_l) x \eta_\varepsilon(x_0-x) +(-x)\eta_\varepsilon(x_0-x)\\
 & = (\lambda_r-\lambda_l) \int_{[x_0-x,\varepsilon]} \eta_\varepsilon(y)\textup{d}y <0,
\end{align*} 
with $\lim_{x\downarrow x_0}g(x)=g(x_0)$ and $\lim_{x\uparrow x_0+\varepsilon}g(x)=g(x_0)$. 
In other words, on $[x_0,x_0+\varepsilon]$ the function $g$ attains its maximum at $x_0$. 
\end{enumerate}

Therefore,  the function $g$ is non-negative with  
\begin{align*}
  \sup_{x\ge0} g(x) 
    =\sup_{x_0 \in \{2\}\cup\{2^{k_n}:n\in\mathbb{N}\} } \sup_{x\in (x_0-\varepsilon, x_0+\varepsilon)} |\hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) | 
    =\sup_{x_0 \in \{2\}\cup\{2^{k_n}:n\in\mathbb{N}\} } |\hat{\upsilon}(x_0) - \hat{\upsilon}_\varepsilon(x_0) | 
    <\frac{1}{2^4}.
\end{align*}
\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{lemma}\label{lem:def_q_for_smoothness}
For $p\in(0,2)$, we define 
\begin{align*}
  q:=\frac{4}{p}-1 \text{ and }x_0(p):=\Big(\frac{p}{6(4-p)}\Big)^{\frac{p}{4-2p}}. 
\end{align*}
Then, $x_0(p)\in(0,\frac{3}{2})$ and for the function $[0,\frac{3}{2}]\ni x \overset{f}{\mapsto} x^q$, it holds $f'(x_0(p))=\frac{1}{6}$.
\end{lemma}
%
\begin{proof}
It is easily verified that
\begin{align*}
   f'(x_0)=\frac{1}{6}
   \Leftrightarrow q x_0^{q-1}=\frac{1}{6}
   \overset{(q>1)}{\Leftrightarrow} x_0^{q-1}=\frac{1}{6q}
   {\Leftrightarrow} x_0=\Big(\frac{1}{6q}\Big)^{\frac{1}{q-1}} = \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}.
\end{align*}
The point $x_0$ lies, indeed, in the domain of $f$.
In order to prove the last claim, we will initially prove that $(0,2)\ni p\mapsto x_0(p)\in(0,+\infty)$ is a decreasing function.
To this end, we will calculate its derivative, which is given by
\begin{align*}
  x_0'(p)&=x_0(p)\big(\frac{p}{4-2p} \ln(\frac{p}{6(4-p)})\big)'.
\end{align*}
Given that $x_0(p)>0$, for every $p\in(0,2)$, we proceed with the second factor only.
Hence,
\begin{align*}
  \big(\frac{p}{4-2p} \ln(\frac{p}{6(4-p)})\big)' 
  % = \dfrac{\left(p-4\right)\ln\left(\frac{p}{6\left(4-p\right)}\right)+2p-4}{\left(p-4\right)\left(p-2\right)^2}
  = \frac{2\ln(\frac{p}{6(4-p)})(4-p) + 2-p}{2(2-p)^2(4-p)}
\end{align*}
The denominator is positive for every $p\in(0,2)$.
The nominator remains negative in the same region of $p$, since for $p\in(0,2)$ 
\begin{align*}
 2\ln(\frac{p}{6(4-p)})(4-p) + 2-p < 2\ln(\frac{p}{6(4-p)})(4-p) + 4-p
 <(2\ln(\frac{p}{6(4-p)})+1)(4-p)<0.
\end{align*} 

Finally, we compute the limits
\begin{align*}
  \lim_{p\downarrow 0} x_0(p) 
    & = \lim_{p\downarrow 0} \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}
      = \lim_{p\downarrow 0} \exp\big(\frac{p}{4-2p}\ln(\frac{p}{6(4-p)})\big)\\
    & = \lim_{z\downarrow 0} \exp\big(z\ln(z)\big) = 1
\end{align*}
and 
\begin{align*}
  \lim_{p\uparrow 2} x_0(p) 
    & = \lim_{p\uparrow 2} \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}} = 0,
\end{align*}
which in conjunction with the monotonicity proved above, verify our claim.
% The last computations will permit us to linearly interpolate, with positive slopes, on the interval $[x_0,2]$.
\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{proof}[Proof of \cref{corollary:UI_Young_improvement:StrongerIntegrability}]
 We will adopt the notation introduced in \cref{lemma:UI_Young_improvement}. 
 The arguments presented below hold for $p>0$.

 \vspace{0.5em}
 For notational convenience we define $\bar{\upsilon}_0=\frac{1}{4},\bar{\upsilon}_{\frac{1}{2}}=\frac{1}{2}$, so that the non-decreasing sequence $(\bar{\upsilon}_n)_{n\in\{0,\frac{1}{2}\}\cup\mathbb{N}}$ associates to the right derivative $\bar{\upsilon}$.
 In view of the introduced notation, we have 
 \begin{align*}
    \overline{\Upsilon}(x)\le 
    \begin{cases}
      \bar{\upsilon}_0 x, &\text{for }x\in[0,1]\\
      \bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}}(x-1), &\text{for }x\in(1,2]\\
      \bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{k=1}^{n-1}\bar{\upsilon}_k + \bar{\upsilon}_{n}(x-n), &\text{for }x\in(n,n+1]
    \end{cases}.
 \end{align*}

 \vspace{0.5em}
 Following the arguments of the proof of \cite[Lemme]{meyer1978sur} and modifying them as in the proof of \cref{prop:UI_Young}, we can prove that for the Young function $\overline{\Upsilon}$ associated to the right-derivative $\bar{\upsilon}$, it holds
 \begin{align}\label{limit:overline_upsilon}
   \lim_{R\to+\infty}\sup_{\alpha\in\mathcal{A}}\int_{{\{z:|z|>R\}}} \overline{\Upsilon}(|z|^p)m_\alpha(\textup{d}z)=0.
 \end{align}

 Indeed, for $c>1$ and $k_0:=\min\{k\in\mathbb{N}  : \bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^k \bar{\upsilon}_q>c\}$
 \begin{align*}
   &\int_{\{z:\overline{\Upsilon}(|z|^p)>c\}} \overline{\Upsilon}(|z|^p) m_\alpha (\textup{d}z)
    \le \sum_{k=k_0}^\infty (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^k \bar{\upsilon}_q) m_\alpha(\{k< |z|^p \le k+1\})\\
    &\hspace{2em}= (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{k_0} \bar{\upsilon}_q) m_\alpha(\{|z|>k_0\}) + \sum_{k=k_0+1}^\infty \bar{\upsilon}_k m_\alpha(\{|z|^p>k\}).
    \numberthis \label{ineq:rhs_bar_upsilon}
 \end{align*}
 Let us choose an arbitrarily small $\delta>0$.
 Then, there exists $n_0$ such that for $n\ge n_0\ge 1$ it holds $ \frac{\bar{\upsilon}_n}{\upsilon_n}<\delta$.
 Bounding the right part of Inequality \eqref{ineq:rhs_bar_upsilon}, we have for $k_0>n_0$\footnote{The reader may observe that $\lim_{c\to+\infty}k_0 = +\infty$.}
 \begin{align*}
   &(\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{k_0} \bar{\upsilon}_q) m_\alpha(\{k_0 < |z|^p\le k_0+1\}) + \sum_{k=k_0+1}^\infty \bar{\upsilon}_k m_\alpha(\{k< |z|^p \le k+1\})\\
    &\hspace{2em}\le (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{n_0} \bar{\upsilon}_q) m_\alpha(\{|z|^p>k_0\}) 
                      + \delta \sum_{q=n_0+1}^{k_0} \upsilon_q m_\alpha(\{|z|^p>k_0\})
                      + \delta \sum_{k=k_0+1}^\infty \upsilon_k m_\alpha(\{|z|^p>k\})\\
    &\hspace{2em}\le (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{n_0} \bar{\upsilon}_q) m_\alpha(\{|z|^p>k_0\}) 
                      +\delta \sum_{k=n_0+1}^\infty {\upsilon}_k m_\alpha(\{|z|^p>k\}).
    \numberthis \label{ineq:rhs_limit_k0}
 \end{align*}
 From the proofs of \cref{prop:UI_Young} and \cref{lemma:UI_Young_improvement} we have for the sequence $(\upsilon_n)_{n\in\mathbb{N}}$
  \begin{align*}
    S:=\sup_{\alpha\in\mathcal{A}} \sum_{n=1}^{\infty}\upsilon_n m_\alpha(\{z:|z|^p>k\}) <+\infty. 
  \end{align*}
  In total, in view of \eqref{property:limit_for_UI}, which implies 
  \begin{align*}
    \lim_{k\to+\infty} \sup_{\alpha\in\mathcal{A}} m_\alpha(\{z:|z|^p>k\}) = 0,
  \end{align*}
  we have from \eqref{ineq:rhs_bar_upsilon}, \eqref{ineq:rhs_limit_k0} and the above limit
  \begin{align*}
    &\lim_{R\to+\infty}\sup_{\alpha\in\mathcal{A}}\int_{{\{z:|z|>R\}}} \overline{\Upsilon}(|z|^p)m_\alpha(\textup{d}z) 
    \le (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{n_0} \bar{\upsilon}_q) \lim_{k\to+\infty} \sup_{\alpha\in\mathcal{A}} m_\alpha(\{z:|z|^p>k\}) + \delta S=\delta S. 
  \end{align*}
  Since $\delta$ was chosen arbitrarily small, we have that the limit on the left hand side of the last inequality is indeed $0$.



 \vspace{0.5em}
 In view of the validity of \eqref{limit:overline_upsilon} and recalling \cref{prop:UI_Young}, there exists a Young function $\Psi$ (with right derivative $\psi$) such that 
 \begin{align*}
    \sup_{\alpha\in\mathcal{A}}\int_{\{z:|z|\ge 1\}} \Psi\big(\overline{\Upsilon}(|z|^p)\big)m_\alpha (\textup{d}z)<+\infty.
 \end{align*}
 Now, observing that $\hat{\upsilon}_\varepsilon(w)<\bar{\upsilon}(w)$, for every $w\ge 2$, we can extract a point $w_0>2$ such that
  \begin{align*}
    \Upsilon(w)<\overline{\Upsilon}(w) \text{ for every }w\ge w_0. 
  \end{align*}  
 Therefore, we get
  \begin{align*}
    &\sup_{\alpha\in\mathcal{A}}\int_{\{z:|z|\ge 1\}} \Psi\big(\Upsilon(|z|^p)\big)m_\alpha (\textup{d}z)\\
    &\hspace{1em}=\sup_{\alpha\in\mathcal{A}}\Big\{ \int_{\{z:1\le |z|^p\le w_0\}} \Psi\big(\Upsilon(|z|^p)\big)m_\alpha (\textup{d}z) + 
                                                    \int_{\{z:|z|^p> w_0\}} \Psi\big(\Upsilon(|z|^p)\big)m_\alpha (\textup{d}z)\Big\}\\
    &\hspace{1em}\le\sup_{\alpha\in\mathcal{A}}\Big\{ \int_{\{z:1\le |z|^p\le w_0\}} \psi\big(\Upsilon(w_0)\big) \Upsilon(|z|^p) m_\alpha (\textup{d}z) + 
                                                      \int_{\{z:|z|^p> w_0\}} \Psi\big(\overline{\Upsilon}(|z|^p)\big)m_\alpha (\textup{d}z)\Big\}\\
    &\hspace{1em}\le  \psi\big(\Upsilon(w_0)\big)  
                      \sup_{\alpha\in\mathcal{A}}  \int_{\{z:|z|\ge 1\}} \Upsilon(|z|^p) m_\alpha (\textup{d}z) + 
                      \sup_{\alpha\in\mathcal{A}}  \int_{\{z:|z|\ge 1\}} \Psi\big(\overline{\Upsilon}(|z|^p)\big)m_\alpha (\textup{d}z)\Big\}
    <+\infty.
  \end{align*}  
  where we have used that $\Psi(x)\le x\psi(x)$ and $\psi$ is non-decreasing.
\end{proof}


==> Proofs_YoungFunctions_Improvement_copy.tex <==
%!TEX root = main.tex

% \begin{remark}\label{rem:preparatory_proof}
  % \begin{enumerate}
  %   \item\label{rem:prep_proof:1}
      In order to prove \cref{lemma:UI_Young_improvement}, we will suitably choose the right-derivative of the Young function $\Upsilon$, denoted by $\upsilon$, based on the behavior of the family $\{m_\alpha\}_{\alpha\in\mathcal{A}}$.
      In the next lines we will try to explain intuitively the procedure.
      To this end, we follow the notation introduced in the proof of \cref{prop:UI_Young}.

      In \citet[Lemme, p. 770]{meyer1978sur} it is described how to alter the sequence $(\upsilon_n)_{n\in\mathbb{N}}$ in order to obtain the (seemingly) stronger integrability described in \cref{corollary:UI_Young_improvement:StrongerIntegrability} and to obtain a moderate Young function.
      For the former, it is chosen a new sequence which is dominated by the sequence $(\upsilon_n)_{n\in\mathbb{N}}$, \emph{i.e.}, the right derivative is ``pushed downwards''.
      For the latter, the newly chosen sequence applies to intervals of increasing length, \emph{i.e.}, the right derivative is ``stretched''. 
      Inspired by \citet[Lemme, p. 770]{meyer1978sur}, we will initially follow the arguments presented there, but we will need go beyond \citet{meyer1978sur} in order to choose more conveniently some values. 
      Following the intuition introduced in the previous lines, the idea for proving \cref{lemma:UI_Young_improvement} is to repeatedly alter the right derivative of the Young function by initially ``properly pushing it downwards'', afterwards ``stretching it'', then making it continuous and finally smoothing it.
  %   \item\label{rem:prep_proof:2}   
  %     When we will be called to prove the regularity conditions for the non-local operator under interest, the quantities 
  %     \begin{align*}
  %       \Upsilon''(|y|^p)|y|^p \text{ and }\Upsilon'(|y|^p)|y|^{p-2}
  %     \end{align*}
  %     need to be controlled.
  %     The former can be universally, \emph{i.e.}, for any $p>0$, remedied by a condition as described in \cref{lemma:UI_Young_improvement}.\ref{lemma:UI_Young_improvement:second_derivative_properties}. 
  %     The latter is innocuous for $p\ge 2$, because $\Upsilon'$ is bounded in a neighborhood of zero.
  %     Consequently $\lim_{|y|\downarrow 0}\Upsilon'(|y|^p)|y|^{p-2}=0$, for $p>2$.
  %     Therefore, due to continuity of $\Upsilon'$, the quantity $\Upsilon'(|y|^p)|y|^{p-2}$ is bounded for any $p\ge 2$ on any compact interval containing $0$.
  %     However, for $p\in(0,2)$, we wish to avoid an``explosion'' because of the term $|y|^{p-2}$.
  %     In this case, we will need to further modify the (right) derivative in a neighborhood of $0$, so that the quantity $\Upsilon'(|y|^p)$ decreases faster than $|y|^{p-2}$; this justifies the existence of \cref{lemma:UI_Young_improvement}.\ref{lemma:UI_Young_improvement:p_smaller_than_2}.    
  % \end{enumerate}
% \end{remark}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\begin{proof}[Proof of \cref{lemma:UI_Young_improvement}]
  In view of 
  the comments provided at the beginning of this subsection,
  % \cref{rem:preparatory_proof}, 
  the current proof should be seen as a continuation of the proof of \cref{prop:UI_Young}.
  To this end, we will assume that the sequence $(\upsilon_n)_{n\in\mathbb{N}}$ is the one described in the second half of the proof of \cref{prop:UI_Young}, where the sequence $(c_n)_{n\in\mathbb{N}}$ obeys to \eqref{property:c_doubling} with $c_1=1$.
  % Without loss of generality, we may assume that $\upsilon_1 =1$.
  We choose to present the construction of the (right) derivative step by step, so that it is intuitively clear to the reader the final choice of the (right) derivative.
  As a result, we sacrifice the compactness of the proof.   

\vspace{0.5em}
 Following \citet{meyer1978sur}, we ``push downwards'' the right derivative by  passing to a new sequence $(\bar{\upsilon}_n)_{n\in\mathbb{N}}$ which is defined by $\bar{\upsilon}_n:=\vartheta(\upsilon_n)$, for every $n\in\mathbb{N}$, where $\vartheta:[0,\infty) \to [0,\infty)$ is increasing and such that 
 \begin{enumerate}
 \item $\vartheta(1)=1$,
 \item $\lim_{x\to\infty}\frac{\vartheta(x)}{x}=0$ as well as $\lim_{x\to\infty}\vartheta(x)=\infty$ and 
 \item the function $[1,\infty) \ni x \longmapsto \vartheta(x+1) - \vartheta(x) \in (0,\infty)$ is (strictly) decreasing and bounded by $\frac{1}{2}$,%
 \footnote{In \citet{meyer1978sur}, it was chosen the square root function. The freedom in choosing the function $\vartheta$ allows to endow the Young function $\Upsilon$ with convenient properties. For example, passing to the sequence $(\bar{\upsilon}_n)_{n\in\mathbb{N}}$ will later allow for the property $\lim_{R\to\infty} \sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|>R\}}\Upsilon(|z|^p) m_\alpha(\textup{d}z)=0,$ \emph{i.e.}, the uniform integrability of the function $\Upsilon(|z|^p)$ with respect to the family $(m_\alpha)_{\alpha\in\mathcal{A}}$. One can verify it in the case $\vartheta$ is the square root function, by checking the proof of \cite[Lemme]{meyer1978sur} and modifying the arguments properly, \emph{i.e.}, as we did in the proof of the equivalence of \cref{prop:UI_Young}. For completeness, we provide the full details in the proof of \cref{corollary:UI_Young_improvement:StrongerIntegrability}. Other possible choices for the function $\vartheta$ are $x\longmapsto x^{\frac12(1-\alpha)}$, for $\alpha \in (0,1)$, or $x\longmapsto x^{\frac{1}{2}(2-\alpha)}$, for $\alpha \in [1,2)$. These choices will be utilized for proving \ref{lemma:UI_Young_improvement:p_smaller_than_1} and \ref{lemma:UI_Young_improvement:p_between_1_and_2}, respectively.} 
\emph{i.e.},
\begin{align*} 
\vartheta(x+1) - \vartheta(x)<\frac{1}{2}, \text{ for every }x\in[1,\infty).
\end{align*} 
 \end{enumerate}
 % \todo[inline]{Instead of the square root, use the function $[1,\infty)\ni w\longmapsto w^{0.5(\frac2p-1)}$}
 In view of \eqref{property:upsilon_inequalities} and the last required property of the function $\vartheta$, we get 
 \begin{gather*}
    \bar{\upsilon}_n \le \bar{\upsilon}_{n+1}< \bar{\upsilon}_n+\frac{1}{2}, \text{ for every }n\in\mathbb{N},
    \shortintertext{as well as}
    \bar{\upsilon}_{c_n}= \vartheta(\upsilon_{c_n}) = \vartheta(n) \text{ for every }n\in\mathbb{N}.
 \end{gather*}
 % as well as the analogous to \eqref{property:upsilon_c_RHSEquality}-\eqref{property:upsilon_c_LHSEquality} properties.
 Then, abusing notation, we define the function $\bar{\upsilon}$
  \begin{gather*}
    \bar{\upsilon}(x) := 
      \begin{cases}
        % \frac{1}{4},        &\text{ for }x\in[0,\frac{3}{2})\\
        % \frac{1}{2},        &\text{ for }x\in[\frac{3}{2},2)\\
        \frac{1}{2},        &\text{ for }x\in[0,2)\\
        \bar{\upsilon}_n,   &\text{ for }x\in[2^{n},2^{n+1}), n\in\mathbb{N}
      \end{cases}.
  \end{gather*}
 Obviously, the function $\bar{\upsilon}$ is right-continuous and non-decreasing.
 Recalling the description in 
 the comments provided at the beginning of this subsection,
 % \cref{rem:preparatory_proof}, 
 the above definition amounts to ``stretching'' the right derivative.
 For the sake of unified notation, we define $\bar{\upsilon}_0:=\frac{1}{2}$, for which choice $\bar{\upsilon}_0<\bar{\upsilon}_1=\bar{\upsilon}_0+\frac{1}{2}$.
Given the set $(c_n)_{n\in\mathbb{N}}$, we can alternatively write the function $\bar{\upsilon}$ as
 \begin{gather*}
    \bar{\upsilon}(x) := 
      \begin{cases}
        \bar{\upsilon}_{0},        &\text{ for }x\in[0,2)\\
        \bar{\upsilon}_1,   &\text{ for }x\in[2,2^{k_1})\\
        \bar{\upsilon}_{k_n},   &\text{ for }x\in[2^{k_{n-1}},2^{k_n}) \text{ and } n\ge2
      \end{cases}.
  \end{gather*}


 \vspace{0.5em}
 We proceed by constructing a continuous function which is dominated by $\bar{\upsilon}$.
 To this end, we will linearly interpolate between the right-end points of intervals of constancy of $\bar{\upsilon}$, which are determined by consecutive elements of the sequence $(c_n)_{n\in\mathbb{N}}$ as described above.
 % On the interval $[0,2]$ the origin and the point $(2,\bar{\upsilon}_0)$ will be interpolated.
 % The rest interpolation points could be described as the right-end points of intervals of constancy of $\bar{\upsilon}$.
 % The precise arguments are presented in the next lines. 
 % We start by defining the set 
 % \begin{align*}
 %   \mathbb{K}:=\{k\in\mathbb{N}\backslash\{1\} : \upsilon_{k-1}<\upsilon_{k}\}=\{k\in\mathbb{N}\backslash\{1\} : \bar{\upsilon}_{k-1}<\bar{\upsilon}_{k}\};
 % \end{align*}%
 % let $(k_n)_{n\in\mathbb{N}}$ be the ordered enumeration of $\mathbb{K}$, \emph{i.e.}, $k_{n}<k_{n+1}$ for every $n\in\mathbb{N}$.
 We define now the function
 \begin{align*}
   \hat{\upsilon}(x) :=
    \begin{cases}
      % \frac{1}{6}x,                                 &\text{for }x\in[0,\frac{3}{2})\\
      % \frac{1}{2}(x-1),                             &\text{for }x\in[\frac{3}{2},2)\\
      \frac{1}{4}x,                             &\text{for }x\in[0,2)\\
      \bar{\upsilon}_{0} + \frac{\bar{\upsilon}_1 - \bar{\upsilon}_0}{2^{k_1}-2}(x-2),   &\text{for }x\in[2,2^{k_1})\\
      \bar{\upsilon}_{k_n} +\frac{ \bar{\upsilon}_{k_{n+1}}-\bar{\upsilon}_{k_{n}}}{2^{k_{n+1}}-2^{k_n}}(x - 2^{k_n}), 
                                                    &\text{for }x\in[2^{k_n},2^{k_{n+1}}), n>1
    \end{cases},
    \numberthis\label{def:hat_upsilon_piecewise_linear}
 \end{align*}
 which is the outcome of the linear interpolation between the right-end points of intervals constancy of the function $\bar{\upsilon}$.
Some remarks are in order:
\begin{enumerate}[label=(\arabic*)]
  \item\label{property:ordered_K_bar_upsilon} $\upsilon_{1}= \bar{\upsilon}_{1}=1$, $\upsilon_{k_1}=2$ and $\upsilon_{k_{n+1}} - \upsilon_{k_n}=1,$ for every $n\in\mathbb{N}$.
  \item The function $\hat{\upsilon}$ is continuous
  % , convex on $[0,2]$ 
  and concave on $[0+\infty)$. 
  This can easily be seen, since $\hat{\upsilon}$ is piecewise linear with %increasing slopes on $(0,2)$ and 
  decreasing slopes on $(0,+\infty)$. 
  Indeed, one can see that the slopes are decreasing by examining the sequence of nominators and denominators.
  More precisely, we have (by definition) that
  \begin{align*}
       \bar{\upsilon}_{k_{n+1}} = \vartheta({\upsilon_{k_{n+1}}}) =\vartheta({\upsilon_{k_{n}}+1}), \text{ for every }n\in\mathbb{N}.  
  \end{align*}
  Given that the function $[1,+\infty)\ni x\mapsto \vartheta({x+1})-\vartheta({x})$ is decreasing and bounded between $0$ and $\frac{1}{2}$, we have that 
  \begin{align}\label{property:diff_bar_upsilon}
    0<\bar{\upsilon}_{k_{n+2}}-\bar{\upsilon}_{k_{n+1}} \le \bar{\upsilon}_{k_{n+1}} - \bar{\upsilon}_{k_{n}}<\frac{1}{2} = \frac{\bar{\upsilon}_1}{2} = \bar{\upsilon}_0, \text{ for every }n\in\mathbb{N}.
  \end{align}
  Moreover, for every $n\in\mathbb{N}$,
  \begin{gather*}
     2^{k_2}-2^{k_1}  > 2^{k_1} - 2
  \shortintertext{as well as}
    2^{k_{n+2}} - 2^{k_{n+1}} 
      = 2^{k_{n+1}}(2^{k_{n+2}-k_{n+1}} - 1) 
      > 2^{k_{n+1}}(1 - 2^{k_{n}-k_{n+1}})
      =2^{k_{n+1}} - 2^{k_{n}}.
  \end{gather*}
  Hence, $\frac{ \bar{\upsilon}_{k_{2}}-\bar{\upsilon}_{k_{1}}}{2^{k_{2}}-2^{k_1}} <\frac{ \bar{\upsilon}_{k_1}}{2(2^{k_1}-2)}\le \frac{1}{4} $ and the sequence $(\frac{ \bar{\upsilon}_{k_{n+1}}-\bar{\upsilon}_{k_{n}}}{2^{k_{n+1}}-2^{k_n}})_{n\in\mathbb{N}}$ is decreasing, since the nominators decrease and the denominators increase, as $n$ increases.
  In other words, 
  \begin{align}
  \sup_{n\in\mathbb{N}}\big\{\frac{ \bar{\upsilon}_{k_{n+1}}-\bar{\upsilon}_{k_{n}}}{2^{k_{n+1}}-2^{k_n}}
                          -\frac{ \bar{\upsilon}_{k_{n+2}}-\bar{\upsilon}_{k_{n+1}}}{2^{k_{n+2}}-2^{k_{n+1}}} \big\}
  \leq \frac{1}{4}.
  \label{upper_bound:slopes}
  \end{align}
\end{enumerate}


\vspace{0.5em}
We proceed to define the derivative of the the desired Young function, but we need to treat separately the cases $p\ge 2$ and $p\in(0,2)$:

\vspace{0.5em}
{\tiny $\blacksquare$} $p\ge 2$. We will smooth the function $\hat{\upsilon}$\footnote{The function $\hat{\upsilon}$ is continuous, but not everywhere differentiable. Hence, the associated Young function will not be twice continuously differentiable.}  by standard tools.
More precisely, for $0<\varepsilon<\frac{1}{2^3}$ we use the standard mollifier $\eta_{\varepsilon}$, \emph{i.e.},
\begin{align*}
 \eta_\varepsilon(x):= \frac{C}{\varepsilon} \exp\Big(\frac{1}{\varepsilon^{-2}x^2-1}\Big) \mathds{1}_{[-\varepsilon,\varepsilon]}(x),
\end{align*}
where $C$ is the normalizing constant.
We define
  \begin{align}\label{def:hat_upsilon_varepsilon_smooth}
   \hat{\upsilon}_\varepsilon(x) :=
   \begin{cases}
     \hat{\upsilon}(x), &\text{ for }x\in[0,1]\\
     \displaystyle \int_{[-\varepsilon, \varepsilon]} \hat{\upsilon}_\varepsilon (x+y) \eta_\varepsilon(y)\textup{d}y, &\text{ for } x> 1.
   \end{cases}
  \end{align}
Hereinafter, we \emph{fix} an $0<\varepsilon<\frac{1}{2^3}$ such that
\begin{align}\label{property:error_bound}
 | \hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x)|<\frac{1}{2^4}, \text{ for every }x\in[0,+\infty).
\end{align}
We present in \cref{comput:error_hat_u} the elementary arguments for the determination of an $\varepsilon$ with the aforementioned property, despite this can be seen as a special case of a general approximation result.
The function $\hat{\upsilon}_\varepsilon$ (for the $\varepsilon$ we fixed) will be the derivative of the desired Young function $\Upsilon$.
Before we prove that $\Upsilon$ possesses the desired properties, some remarks are in order:
\begin{enumerate}[label=(\arabic*)]
\setcounter{enumi}{2}
 \item $\hat{\upsilon}_{\varepsilon}(0)=0$ and $\hat{\upsilon}_{\varepsilon}(x)>0$ for $x>0$. 

 \item\label{property:identical_on_linear} For $x\in(1,2-\varepsilon)\cup(2+\varepsilon,2^{k_1}-\varepsilon) \cup \big(\bigcup_{k\in\mathbb{N}} (2^{k_n}+\varepsilon, 2^{k_{n+1}}-\varepsilon)\big)$ 
 it is true that $\hat{\upsilon}_\varepsilon(x)=\hat{\upsilon}(x)$, because of the linearity of $\hat{\upsilon}$ on the interval $(x-\varepsilon,x+\varepsilon)$.

\item\label{property:concavity_domination}
% On $(0,2-\varepsilon)$, the function $\hat{\upsilon}_\varepsilon$ is convex, with $\hat{\upsilon}_\varepsilon \ge \hat{\upsilon}$, while 
On $(0,+\infty)$ the function $\hat{\upsilon}_\varepsilon$ is concave, with $\hat{\upsilon}_\varepsilon \le \hat{\upsilon}$.
The concavity of $\hat{\upsilon}_\varepsilon$ is inherited from the concavity of $\hat{\upsilon}$. 
The domination can be easily proven using the piecewise linearity of $\hat{\upsilon}_\varepsilon$, the fact that the slopes are non-increasing and the definition of the mollification.\footnote{In \cref{comput:error_hat_u} we will need to estimate the difference $|\hat{\upsilon}(x) -\hat{\upsilon}_\varepsilon(x)|$, so we postpone until then the computations.}

% and infinitely differentiable on $(0,\infty)$.

\item\label{property:second_derivative_finally_decreasing} The function $\hat{\upsilon}_\varepsilon$ is infinitely differentiable.
In particular, its first derivative is positive and non-increasing due to concavity. 
\end{enumerate}



















% Summing up, for $x\in (x_0-\varepsilon, x_0+\varepsilon)$ it holds
% \begin{align*}
%   &\sup_{x\in (x_0-\varepsilon, x_0+\varepsilon)} |\hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) |\\
%     &\hspace{2em}=\max\big\{\sup_{x\in (x_0-\varepsilon, x_0]} |\hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x)|, \sup_{x\in [x_0, x_0+\varepsilon)} |\hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) |\big\}  \\
%     &\hspace{2em}=\max\Big\{\sup_{x\in (x_0-\varepsilon, x_0)} (\lambda_l-\lambda_r) \Big|\int_{[-\varepsilon,x_0-x]} y\eta_\varepsilon (y) \textup{d}y\Big|, 
%                 \sup_{x\in [x_0, x_0+\varepsilon)} (\lambda_l-\lambda_r) \Big|\int_{[x_0-x,\varepsilon]} y\eta_\varepsilon (y) \textup{d}y\Big|\Big\}  \\
%     &\hspace{2em}= (\lambda_l-\lambda_r)\cdot \Big|\int_{(0,\varepsilon)} y\eta_\varepsilon (y) \textup{d}y\Big| 
%                  = |\hat{\upsilon}(x_0) - \hat{\upsilon}_\varepsilon(x_0) |
%                  \overset{\eqref{property:bound_of_error}}{<}\frac{1}{2^4}, \text{for any }x_0.  
% \end{align*}
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
\vspace{0.5em}
The function 
\begin{align*}
  \Upsilon(x) := \int_{[0,x]} \hat{\upsilon}_\varepsilon (u) \textup{d}u, \text{ for }x\ge 0,
\end{align*}
satisfies the claimed properties: 
\begin{enumerate}
  \item[\ref{lemma:UI_Young_improvement:moderate_C2}] Since $\hat{\upsilon}_\varepsilon$ is infinitely differentiable, so is $\Upsilon$. 
  In particular, $\Upsilon$ is twice continuously differentiable.


  \vspace{0.5em}
  We prove, now, that $\Upsilon$ is moderate, \emph{i.e.}, $\bar{c}_{\Upsilon}< +\infty.$
  % \begin{align*}
  %   \bar{c}_{\Upsilon} = \sup_{x>0} \frac{x \hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)} < +\infty.
  % \end{align*}
  We will avoid explicit computations and we will make use of the aforementioned properties for $\hat{\upsilon}_{\varepsilon}$ and of known results from the theory of convex functions.
  More precisely, the concavity of $\hat{\upsilon}_{\varepsilon}$ in conjunction with the fact that $\hat{\upsilon}(0)=0$ implies its subadditivity.
  In particular,
  \begin{align*}
  \hat{\upsilon}_{\varepsilon} (2x)\leq 2 \hat{\upsilon}_{\varepsilon}(x), \text{ for every }x>0.
  % \label{property:hat_upsilon_epsilon_moderate}
  \end{align*}
  In turn, this implies
\begin{align*}
  x\hat{\upsilon}_\varepsilon(x) 
    &\le \int_{[x,2x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z 
      = \int_{[0,2x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z - \int_{[0,x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z\\
    & = \int_{[0,x]}2\hat{\upsilon}_\varepsilon(2w)\textup{d}w - \int_{[0,x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z
      \le \int_{[0,x]}4\hat{\upsilon}_\varepsilon(w)\textup{d}w - \int_{[0,x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z\\
    &=3\Upsilon(x),
\end{align*}
  where in the first inequality we used that $\hat{\upsilon}_\varepsilon$ is increasing.  
In other words,
\begin{align*}
\sup_{x>0}\frac{x\hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)}\leq 3.
\end{align*}
 %  We will consider the three subintervals $(0,2-\varepsilon]$, $[2-\varepsilon,2^{k_1}]$ and $[2^{k_1},+\infty)$. 
 %  For $x\in(0,2-\varepsilon)$ we have 
 %  \begin{align*}
 %    \sup_{x\in(0,2-\varepsilon]} \frac{x \hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)} = \frac{\frac{1}{6}x^2}{\frac{1}{6}\frac{1}{2}x^2} = 2.
 %  \end{align*}
 %  For $x\in[2-\varepsilon,2^{k_1}]$, we have that both nominator and denominator are continuous functions, bounded away from $0$ and considered on a compact interval. 
 %  Hence
 % \begin{align}
 %    \sup_{x\in[2-\varepsilon,2^{k_1}]} \frac{x \hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)} <+\infty.
 %    \label{property:moderate_initial_segment}
 %  \end{align}
 %  For $x\in[2^{k_1},+\infty]$, we will initially prove that there exists a constant $K_2>1$ such that
 %  \begin{align}\label{property:moderate_derivative}
 %    \hat{\upsilon}_\varepsilon(2x) \le K_2 \hat{\upsilon}_\varepsilon(x).
 %  \end{align}
 %  Indeed, let $x\ge 2^{k_1}$.
 %  Then, there exists unique $n\ge 2$ such that $2x\in(2^{k_{n-1}},2^{k_{n}}]$, for $k_{n-1},k_{n}\in\mathbb{K}$.
 %  Then, 
 %  \begin{enumerate}[label=(\alph*)]
 %    \item  either $x\in[2^{k_{n-1}},2^{k_n})$, in which case
 %    \begin{align*}
 %        \hat{\upsilon}(2x) = \hat{\upsilon}(2x) - \hat{\upsilon}(x) + \hat{\upsilon}(x)
 %        \overset{\eqref{property:diff_bar_upsilon}}{<}
 %        \frac{1}{2} + \hat{\upsilon}(x)<2\hat{\upsilon}(x),
 %    \end{align*}
 %    \emph{i.e.}, $K_2=2$,

 %    \item  or $x\in[2^{k_{n-2}},2^{k_{n-1}})$, in which case
 %    \begin{align*}
 %        \hat{\upsilon}(2x) = \hat{\upsilon}(2x) - \hat{\upsilon}(2^{k_{n-1}}) + \hat{\upsilon}(2^{k_{n-1}})- \hat{\upsilon}(x) + \hat{\upsilon}(x)
 %        \overset{\eqref{property:diff_bar_upsilon}}{<}
 %        2\frac{1}{2} + \hat{\upsilon}(x)<3\hat{\upsilon}(x),
 %    \end{align*}
 %    \emph{i.e.}, $K_2=3$.
 %  \end{enumerate}
 %  In total, for $K_2=3$ we have that \eqref{property:moderate_derivative} holds for any $x\ge 2^{k_1}$.
 %  This allows us to derive, for $x\ge 2^{k_1}$,
 %  \begin{align*}
 %    x\hat{\upsilon}_\varepsilon(x) 
 %      &\le \int_{[x,2x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z 
 %        = \int_{[0,2x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z - \int_{[0,x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z\\
 %      & = \int_{[0,x]}2\hat{\upsilon}_\varepsilon(2w)\textup{d}w - \int_{[0,x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z
 %        \le \int_{[0,x]}2K_2\hat{\upsilon}_\varepsilon(w)\textup{d}w - \int_{[0,x]}\hat{\upsilon}_\varepsilon(z)\textup{d}z\\
 %      &=(2K_2-1)\Upsilon(x),
 %  \end{align*}
 %  where in the first inequality we used that the $\hat{\upsilon}_\varepsilon$ is increasing.
 %  We have from the inequalities above that 
 %  \begin{align*}
 %      \sup_{x\ge 2^{k_1}} \frac{x\hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)} \le 2K_2-1=5<+\infty.
 %    \end{align*}
 %   To sum up, we have proven that 
 %   \begin{align*}
 %     \bar{c}_\Upsilon = \max\Big\{ 
 %          \sup_{x\in(0,2-\varepsilon]} \frac{x \hat{\upsilon}(x)}{\Upsilon(x)},
 %          \sup_{x\in[2-\varepsilon,2^{k_1}]} \frac{x \hat{\upsilon}(x)}{\Upsilon(x)},
 %          \sup_{x\ge 2^{k_1}} \frac{x\hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)}
 %          \Big\}
 %          <+\infty.
 %   \end{align*}




   \item[\ref{lemma:UI_Young_improvement:second_derivative_properties}] Recall from \ref{property:second_derivative_finally_decreasing} that $\hat{\upsilon}_\varepsilon'=\Upsilon''$ is continuous, positive and non-increasing.
   Moreover, $\hat{\upsilon}_\varepsilon'(x)=\frac{1}{4}$, for $x\in[0,2)$. 
   Therefore, $\Upsilon''$ is bounded.
   
   \vspace{0.5em}
   We proceed to prove \eqref{property:second_derivative_faster_than_identity}.
   The reader may recall that the value of $\varepsilon$ is fixed and smaller that $\frac{1}{2^3}$.
   We will consider the following cases:
   \begin{enumerate}[label=\textbullet]
      \item 
      $x\in[0,2]$: then, immediately $x\Upsilon''(x) \le \frac{1}{2}$.

      \item 
      $x\in(2,2+\varepsilon]$: then,
      \begin{align*}
        x\Upsilon''(x)
          \overset{\text{\ref{property:second_derivative_finally_decreasing}}}{<} 
          (2 + \varepsilon) \Upsilon''(2)
          \le 
          (2 + \varepsilon) \frac14
          \overset{\eqref{property:diff_bar_upsilon}}{<} (\frac{1}{2}+ \frac{1}{2^5}) <1.  
      \end{align*}

      \item 
      $x\in(2+\varepsilon,2^{k_1}]$: we recall that by definition, $k_1\ge2$ and that $\overline{\upsilon}_{1}=1=2\bar{\upsilon}_0$.
      Then, 
      \begin{align*}
        x\Upsilon''(x) 
          < \frac{2^{k_1} (\bar{\upsilon}_1 - \bar{\upsilon}_0)}{2^{k_1}-2}
          = \frac{2^{k_1}}{2(2^{k_1}-2)}
        \le 1.
      \end{align*}

      \item 
       $x\in(2^{k_n},2^{k_n}+\varepsilon]$, for $n\in\mathbb{N}$:
        then,
        \begin{align*}
          x\Upsilon''(x)
            \overset{\text{\ref{property:second_derivative_finally_decreasing}}}{<} 
            (2^{k_n} + \varepsilon) \Upsilon''(2^{k_n})
            \le 
            (2^{k_n} + \varepsilon) \frac{\bar{\upsilon}_{k_{n}}-\bar{\upsilon}_{k_{n-1}}}{2^{k_{n}} - 2^{k_{n-1}}}
            \overset{\eqref{property:diff_bar_upsilon}}{<} \frac{1}{2(1-2^{k_{n-1}-k_n})} + \frac{1}{2^5} <2,  
        \end{align*}
        since $k_n-k_{n-1}\ge 1$.

     \item 
        $x\in(2^{k_n}+\varepsilon,2^{k_{n+1}}]$, for some $n\in\mathbb{N}$:
        then,
        \begin{align*}
          x\Upsilon''(x) 
            \overset{\text{\ref{property:second_derivative_finally_decreasing}}}{<} 
            2^{k_{n+1}}\Upsilon''(2^{k_{n}}+\varepsilon)
             \le  2^{k_{n+1}}\frac{\bar{\upsilon}_{k_{n+1}}-\bar{\upsilon}_{k_{n}}}{2^{k_{n+1}} - 2^{k_{n}}}
            \overset{\eqref{property:diff_bar_upsilon}}{<}\frac{1}{2(1-2^{k_n-k_{n+1}})}\le 1,
        \end{align*}
        since $k_{n+1}-k_n\ge 1$.
    In total, a constant $C$ for the case $p\ge 2$ is $2$.
   \end{enumerate}
%
%
    \item[\ref{lemma:UI_Young_improvement:submultiplicativity}] 
    In view of \citet[Proposition 1]{HUDZIK1992313},\footnote{In \cite{HUDZIK1992313} the property of being ``finally submultiplicative'' is described by the term ``submultiplicative at infinity''.} it is sufficient to prove the desired property for some $R>1$, instead of $R=1$, \emph{i.e.},
    \begin{align*}
    \Upsilon(xy)\leq C \Upsilon(x) \Upsilon(y)\text{ for every }x,y\geq R.
    \end{align*}
    In order to prove this claim we will detour and we will prove the analogous claim for the Young function, denoted by $\widehat{\Upsilon}$, with  derivative $\hat{\upsilon}$ defined in \eqref{def:hat_upsilon_piecewise_linear}. 
    This detour is indeed valid in view of \cref{lemma:Young_equiv_submult}.
    From \citet[Proposition 2]{HUDZIK1992313}, $\widehat{\Upsilon}$ is finally submultiplicative if and only if $\hat{\upsilon}$ is finally submultiplicative, \emph{i.e.}, there exist $C,R>0$ such that
    \begin{align}\label{ineq:submult_derivative}
    \hat{\upsilon}(xy)\leq C \hat{\upsilon}(x) \hat{\upsilon}(y)\text{ for every }x,y\geq R.
    \end{align}

    We proceed to prove our last claim. 
    Initially, we remind the reader the properties presented in \ref{property:ordered_K_bar_upsilon}, namely 
    \begin{gather*}
    \hat{\upsilon}(2)=\bar{\upsilon}_1=\vartheta(1)=1
  \shortintertext{and}
    \hat{\upsilon} (2^{k_n})= \bar{\upsilon}_{k_n}=\vartheta(n+1), \text{ for }n\in\mathbb{N}. 
    \end{gather*}
    For notational convenience we define $k_0:=1$.
    Let, now, $x,y\geq2$. 
    Then, there exist $k_{n_x},k_{n_y}\in \mathbb{K}\cup\{k_0\}=\{k_0,k_1,k_2,\dots\}$ such that 
    \begin{align*}
    x\in [2^{k_{n_x}},2^{k_{n_x+1}}) 
    \text{ and }
    y\in [2^{k_{n_y}},2^{k_{n_y+1}}). 
    \end{align*}
    Our next claim is that it is sufficient to prove the existence of a $C>0$ such that 
    \begin{align*} 
    \hat{\upsilon}(2^{k_{n_x+1}+k_{n_y+1}}) \leq C \hat{\upsilon}(2^{k_{n_x}}) \hat{\upsilon}(2^{k_{n_y}}). 
    \end{align*} 
    Indeed, the fact that $\hat\upsilon$ is increasing, allows us to conclude \eqref{ineq:submult_derivative}. 
    %
    %
    Let $k_{n_x}\leq k_{n_y}$.
    Then, 
    \begin{align*}
    k_{n_x+1}+k_{n_y+1} \leq 2k_{n_y+1}  \leq k_{2(n_y+1)}.
    % k_{n_x+1}+k_{n_y+1} \leq k_{n_x+n_y+2},
    \end{align*}
    The last inequality is true, because $k_{n}-k_{n-1}\geq 1 $ for every $n\in\mathbb{N}$, which  
    % which is true, because $k_{n}-k_{n-1}\geq 1 $ for every $n\in\mathbb{N}$, which  
\end{enumerate}



{\tiny $\blacksquare$} $p\in(0,2)$. Before we smooth the function $\hat{\upsilon}$, we will need to suitably modify it on $[0,2]$.
We have in mind that \eqref{property:second_derivative_faster_to_0} has to hold. 
To this end, we will choose the derivative $\hat{\upsilon}$ to behave in a neighborhood of $0$ as a power function, say of power $q$, so that 
\begin{align*}
  \lim_{x\downarrow 0}(x^p)^qx^{p-2}=\lim_{x\downarrow 0}(x^p)^{q-1}x^{2p-2}=0.
\end{align*}
\cref{lem:def_q_for_smoothness} verifies that there is a legitimate choice of $q$ for each $p\in(0,2)$:
% We choose $q$ so that $pq+p-2=2$, \emph{i.e.}, we define 
\begin{align}\label{def:q}
  q:=\frac{4}{p}-1, \text{ for }p\in(0,2).
\end{align}
Observe that for the choice of $q$ it holds $pq+p-2=p(q-1)+2p-2=2$.
Additionally, for 
\begin{align*}
   x_0(p):=\big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}\in[0,1]
\end{align*}
and for $[0,\infty)\ni x\overset{f}{\mapsto} x^q$ it holds $f'(x_0)=\frac{1}{6}$.
Moreover, 
\begin{gather*}
  0<f(x_0) = x_0^q 
    = \Big(\frac{1}{6q}\Big)^{\frac{q}{q-1}} 
    =\Big(\frac{p}{6(4-p)}\Big)^{\frac{4-p}{4-2p}}
    <\frac{p}{6(4-p)}
    \le \frac{1}{6}
    \shortintertext{as well as}
  0<f(x_0) + \frac{1}{6} (\frac{5}{4}-x_0)
    <\frac{1}{6}+\frac{1}{6} \frac{5}{4} = \frac{1}{6} \frac{9}{4} = \frac{3}{8}<\frac{1}{2}
\end{gather*}
where we used that $\frac{p}{6(4-p)}<1$ and that $\frac{4-p}{4-2p}>1$.

% Furthermore, we seek the point $x_0=x_0(p)\in(0,\frac{3}{2})$ (if it exists) for which
% \begin{align*}
%    f'(x_0)=\frac{1}{6}
%    \Leftrightarrow q x_0^{q-1}=\frac{1}{6}
%    \overset{(q>1)}{\Leftrightarrow} x_0^{q-1}=\frac{1}{6q}
%    {\Leftrightarrow} x_0=\Big(\frac{1}{6q}\Big)^{\frac{1}{q-1}} = \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}.
% \end{align*}
% The point $x_0$ lies, indeed, in the domain of $f$.
% We can compute the respective limits
% \begin{align*}
%   \lim_{p\downarrow 0} x_0(p) 
%     & = \lim_{p\downarrow 0} \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}
%       = \lim_{p\downarrow 0} \exp\big(\frac{p}{4-2p}\ln(\frac{p}{6(4-p)})\big)\\
%     & = \lim_{z\downarrow 0} \exp\big(z\ln(z)\big) = 1
% \end{align*}
% and 
% \begin{align*}
%   \lim_{p\uparrow 2} x_0(p) 
%     & = \lim_{p\uparrow 2} \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}} = 0.
% \end{align*}
% Moreover, 
% \begin{gather*}
%   0<f(x_0) = x_0^q 
%     = \Big(\frac{1}{6q}\Big)^{\frac{q}{q-1}} 
%     =\Big(\frac{p}{6(4-p)}\Big)^{\frac{4-p}{4-2p}}
%     <\frac{p}{6(4-p)}
%     \le \frac{1}{6}
%     \shortintertext{as well as}
%   0<f(x_0) + \frac{1}{6} (\frac{5}{4}-x_0)
%     <\frac{1}{6}+\frac{1}{6} \frac{5}{4} = \frac{1}{6} \frac{9}{4} = \frac{3}{8}<\frac{1}{2}
% \end{gather*}
% where we used that $\frac{p}{6(4-p)}<1$ and that $\frac{4-p}{4-2p}>1$.
% The last computations will permit us to linearly interpolate, with positive slopes, on the interval $[x_0,2]$.
The above properties permit us to \emph{re}-define the function $\hat{\upsilon}$ on $[0,2]$ as follows
\begin{align}
  \hat{\upsilon}(x):=
  \begin{cases}
    f(x), &\text{for }x\in[0,x_0]\\
    f(x_0) + \frac{1}{6} (x-x_0), &\text{for }x\in(x_0,\frac{5}{4}]\\ 
    % f(x_0) + \frac{1}{6} (\frac{5}{4}-x_0) + 4[\frac{1}{2} - f(x_0) + \frac{1}{6} (\frac{5}{4}-x_0)](x-\frac{5}{4}), &\text{for }x\in(\frac{5}{4},\frac{3}{2}]\\ 
    \hat{\upsilon}(\frac{5}{4}) + \frac{4}{3}\big[\frac{1}{2} - \hat{\upsilon}(\frac{5}{4})\big](x-\frac{5}{4}), &\text{for }x\in(\frac{5}{4},2]\\ 
    % \text{as before}, &\text{for }x\ge2
  \end{cases}.
\end{align}
We can easily verify that the redefined function $\hat{\upsilon}$ is continuous on $[0,+\infty)$ and continuously differentiable on $(0,\frac{5}{4})$.
For $0<\varepsilon<\frac{1}{2^4}$ we define
\begin{align*}
\hat{\upsilon}_\varepsilon(x) :=
  \begin{cases}
    \hat{\upsilon}(x), &\text{for } x\in [0,\frac{5}{4}-\varepsilon]\\
     \displaystyle \int_{[-\varepsilon, \varepsilon]} \hat{\upsilon}_\varepsilon (x+y) \eta_\varepsilon(y)\textup{d}y, &\text{ for } x> \frac{5}{4}-\varepsilon
  \end{cases}.
\end{align*}
The function 
\begin{align*}
  \Upsilon(x) := \int_{[0,x]} \hat{\upsilon}_\varepsilon (u) \textup{d}u, \text{ for }x\ge 0,
\end{align*}
satisfies the claimed properties:\footnote{We will focus our attention on the interval $[0,2^{k_1}]$, since for the rest we can use the analogous arguments presented for the case $p\ge 2$. The only difference is the upper bound for $\varepsilon$.}
\begin{enumerate}
    \item[\ref{lemma:UI_Young_improvement:moderate_C2}]
    The function $\hat{\upsilon}_\varepsilon$ is continuously differentiable on every point of $(0,x_0]$ and infinitely differentiable on every point of $(x_0,2^{k_1}]$.
    Hence $\Upsilon$ is twice differentiable at $x_0$.

    \vspace{0.5em}
    In order to prove that $\Upsilon$ is moderate, we will work separately on the intervals $(0,x_0]$ and $[x_0,2^{k_1}]$.
    For the former interval, immediate computations verify
    \begin{align*}
      \sup_{x\in(0,x_0]}\frac{x\hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)} = q+1<+\infty.
    \end{align*}
    For the latter interval, we use the continuity of $x\mapsto x\hat{\upsilon}_\varepsilon$ and $\Upsilon$, the compactness of the interval under consideration as well as the fact that $0<\inf_{x\in[x_0,2^{k_1}]}\Upsilon(x),\sup_{x\in[x_0,2^{k_1}]}\Upsilon(x)<+\infty$.
    In total,
    \begin{align*}
        \bar{c}_{\Upsilon} =\sup_{x>0} \frac{x\hat{\upsilon}_\varepsilon(x)}{\Upsilon(x)}<+\infty.
    \end{align*}

    \item[\ref{lemma:UI_Young_improvement:second_derivative_properties}] 
    We can readily adapt the arguments we used in the case $p\ge 2$.

    \item[\ref{lemma:UI_Young_improvement:submultiplicativity}] 
    On $[2,+\infty)$, the derivative $\hat{\upsilon}_\varepsilon$ is identical to the derivative constructed for the case $p\ge 2$.
    Therefore, for the case we are examining now we have that $x\hat{\upsilon}_\varepsilon'(x)\le 2$, for $x\in[2,+\infty)$.
    In other words, we for the same $t_0$, as in the case $p\ge 2$, the function  
    \begin{align*}
        [t_0,+\infty) \ni t \longmapsto \frac{t \Upsilon''(t)}{\Upsilon'(t)} \text{ is non-increasing}.
    \end{align*}
    We conclude in view of \citet[Chapter I, Theorem 5.2, p.32]{krasnoselskii1961}.

    \item[\ref{lemma:UI_Young_improvement:p_smaller_than_2}]
    This property is true because of the choice of $q$; see \eqref{def:q} and the comment following it.

\end{enumerate}
\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{lemma}\label{lemma:Young_equiv_submult}
Let $\Upsilon$, resp. $\widehat{\Upsilon}$, be the Young function associated to the right-derivative $\hat{\upsilon}_{\varepsilon}$ defined in \eqref{def:hat_upsilon_varepsilon_smooth}, resp. $\hat{\upsilon}$ defined in \eqref{def:hat_upsilon_piecewise_linear}.
Then, the Young functions $\Upsilon$ and $\widehat{\Upsilon}$ are equivalent, \emph{i.e.},
there exist $C_1,C_2, x_0>0$ such that
\begin{align*}
\widehat{\Upsilon}(C_1x) \leq \Upsilon(x) \leq \widehat{\Upsilon}(C_2x) \text{ for every }x\geq x_0.
\end{align*}
Moreover, $\Upsilon$ is finally submultiplicative, \emph{i.e.}, there exist $C,R>0$ such that 
\begin{align*}
\Upsilon (xy) \leq C \Upsilon(x) \Upsilon(y) \text{ for all }x,y>R,
\end{align*}
 if and only if $\widehat{\Upsilon}$ is finally submultiplicative.
\end{lemma}
\begin{proof}
  In order to prove that $\Upsilon$ and $\widehat{\Upsilon}$ are equivalent we will compare their derivatives $\hat{\upsilon}_{\varepsilon}$ and $\hat{\upsilon}$.
  More precisely, from \citet[Lemma 3.2, p.18]{krasnoselskii1961} we need to check the existence and the positiveness of the limit of their ratio.
  Indeed,
  \begin{align*}
    \lim_{x\to\infty} \frac{\hat{\upsilon}(x)}{\hat{\upsilon}_{\varepsilon}(x)} = 1,
  \end{align*}
  where we used  $0\leq \hat{\upsilon}(x) - \hat{\upsilon}_{\varepsilon}(x)<\frac{1}{2^4}$ for every $x\geq0$, see \eqref{property:error_bound}, and that $\hat{\upsilon}_{\varepsilon}(x) \uparrow \infty$, as $x\uparrow \infty$.

For the validity of the second statement, the reader may consult \citet[Lemma 5.1, p30]{krasnoselskii1961} and the comments following it.
\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{lemma}\label{comput:error_hat_u}
  There exists $0<\varepsilon<\frac{1}{2^3}$ for which the bound \eqref{property:error_bound} holds.
\end{lemma}
\begin{proof}
Let us define the auxiliary function
\begin{align*}
  g(x):= \hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x), \text{for }x>0.
\end{align*}
Let $x_0\in\{2\}\cup\{2^{k_n}:n\in\mathbb{N}\}$.
Then for any such $x_0$ we denote by $\lambda_l x +\beta_l$ the representation of the affine part of $\hat{\upsilon}$ associated to the subinterval on the left of $x_0$ and by $\lambda_r x +\beta_r$ the representation of the affine part of $\hat{\upsilon}$ associated to the subinterval on the right of $x_0$.
Due to continuity of $\hat{\upsilon}$
\begin{align}\label{equality:lambda_beta}
  \lambda_l x_0 +\beta_l=\lambda_r x_0 +\beta_r
  \Leftrightarrow 
  \beta_l - \beta_r = (\lambda_r - \lambda_l)x_0.
\end{align}
Then, for $0<\varepsilon<\frac{1}{2^3}$
\begin{align*}
    g(x_0)=\hat{\upsilon}(x_0) - \hat{\upsilon}_\varepsilon(x_0) 
      &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
      (\lambda_l x_0 +\beta_l) - \int_{[-\varepsilon,0]} [\lambda_l (x_0+y) +\beta_l]\eta_\varepsilon(y) \textup{d}y - \int_{[0,\varepsilon]} [\lambda_r (x_0+y) +\beta_r]\eta_\varepsilon(y) \textup{d}y \\
      &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
      \int_{[-\varepsilon,\varepsilon]}[\lambda_l (x_0+y) +\beta_l]\eta_\varepsilon(y)\textup{d}y 
        - \int_{[-\varepsilon,0]} [\lambda_l (x_0+y) +\beta_l]\eta_\varepsilon(y) \textup{d}y \\
      &\hspace{1em}  - \int_{[0,\varepsilon]} [\lambda_r (x_0+y) +\beta_r]\eta_\varepsilon(y) \textup{d}y \\
      &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
      \int_{[0,\varepsilon]} [(\lambda_l - \lambda_r) (x_0+y) +(\beta_l - \beta_r)]\eta_\varepsilon(y) \textup{d}y \\
      &\overset{\eqref{equality:lambda_beta}}{=} 
      (\lambda_l - \lambda_r) \int_{[0,\varepsilon]} y\eta_\varepsilon(y) \textup{d}y \ge 0,
\end{align*}
given that $\lambda_l\ge\lambda_r$,
The quantity $g(x_0)$ can vanish only  in the case $\lambda_l=\lambda_r$.
Hence,
\begin{align*}
  0\le \lambda_l - \lambda_r
  \le \max\Big\{
    \frac{1}{4}-\frac{1}{2(2^{k_1}-2)}, 
    \sup_{n\in\mathbb{N}}\{\frac{ \bar{\upsilon}_{k_{n+1}}-\bar{\upsilon}_{k_{n}}}{2^{k_{n+1}}-2^{k_n}}
                          -\frac{ \bar{\upsilon}_{k_{n+2}}-\bar{\upsilon}_{k_{n+1}}}{2^{k_{n+2}}-2^{k_{n+1}}}\}
    \Big\}
  \overset{\eqref{upper_bound:slopes}}{\leq}  \frac{1}{4}
\end{align*}
and given also that 
\begin{align*}
  \lim_{\varepsilon \downarrow 0}\int_{[0,\varepsilon]} y\eta_\varepsilon(y) \textup{d}y=0,
\end{align*}
we can chose $0<\varepsilon<\frac{1}{2^3}$ such that 
\begin{align*}
  \int_{[0,\varepsilon]} y\eta_\varepsilon(y) \textup{d}y \le \frac{1}{2^2}.
 \end{align*}
In total, we have 
\begin{align}\label{property:bound_of_error}
  \sup\{\hat{\upsilon}(x_0) - \hat{\upsilon}_\varepsilon(x_0) :x_0\in\{2\}\cup\{2^{k_n}:n\in\mathbb{N}\} \}<\frac{1}{2^4}.
\end{align}
%
%
% 
% 
% 
% 
We will proceed to estimate the function $g$ in the rest points of its domain:
\begin{enumerate}[label=\textbullet]
  \item 
For $x\in(1,2-\varepsilon)\cup(2+\varepsilon,2^{k_1}-\varepsilon) \cup \big(\bigcup_{k\in\mathbb{N}} (2^{k_n}+\varepsilon, 2^{k_{n+1}}-\varepsilon)\big)$, which is the set considered in \ref{property:identical_on_linear}, we have that $g(x)=0$. 

  \item 
For $x\in(x_0-\varepsilon,x_0]$ it holds
\begin{align*}
  g(x) = \hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) 
  &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
  \lambda_l x + \beta_l 
    - \int_{[-\varepsilon,x_0-x]} [\lambda_l(x+y)+\beta_l]\eta_\varepsilon(y)\textup{d}y
    - \int_{[x_0-x,\varepsilon]} [\lambda_r(x+y)+\beta_r]\eta_\varepsilon(y)\textup{d}y\\
  &\overset{\phantom{\eqref{equality:lambda_beta}}}{=}
   \int_{[x_0-x,\varepsilon]} [(\lambda_l-\lambda_r)(x+y)+(\beta_l-\beta_r)]\eta_\varepsilon(y)\textup{d}y\\
  &\overset{\eqref{equality:lambda_beta}}{=}
   (\lambda_l-\lambda_r) \int_{[x_0-x,\varepsilon]} [(x+y)-x_0 ]\eta_\varepsilon(y)\textup{d}y\ge0,
\end{align*}
since $(x+y)-x_0\ge 0$ for $y\in[x_0-x,\varepsilon]$ and the assumption on $x$.
Moreover, 
\begin{align*}
 g'(x) 
 &= (\lambda_l-\lambda_r) \int_{[x_0-x,\varepsilon]} \eta_\varepsilon(y)\textup{d}y
  + (\lambda_l-\lambda_r) x \eta_\varepsilon(x_0-x) +(-x)\eta_\varepsilon(x_0-x)\\
 & = (\lambda_l-\lambda_r) \int_{[x_0-x,\varepsilon]} \eta_\varepsilon(y)\textup{d}y >0,
\end{align*} 
with $\lim_{x\downarrow x_0-\varepsilon}g(x)=0$ and $\lim_{x\uparrow x_0}g(x)=g(x_0)$. 
In other words, on $(x_0-\varepsilon,x_0]$ the function $g$ attains its maximum at $x_0$. 

  \item For $x\in(x_0,x_0+\varepsilon]$ it holds
\begin{align*}
  g(x)= \hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) 
  &\overset{\phantom{\eqref{equality:lambda_beta}}}{=} 
  \lambda_r x + \beta_r 
    - \int_{[-\varepsilon,x_0-x]} [\lambda_l(x+y)+\beta_l]\eta_\varepsilon(y)\textup{d}y
    - \int_{[x_0-x,\varepsilon]} [\lambda_r(x+y)+\beta_r]\eta_\varepsilon(y)\textup{d}y\\
  &\overset{\phantom{\eqref{equality:lambda_beta}}}{=}
   \int_{[-\varepsilon,x_0-x]} [(\lambda_r-\lambda_l)(x+y)+(\beta_r-\beta_l)]\eta_\varepsilon(y)\textup{d}y\\
  &\overset{\eqref{equality:lambda_beta}}{=}
   (\lambda_r-\lambda_l) \int_{[-\varepsilon,x_0-x]} [(x+y)-x_0 ]\eta_\varepsilon(y)\textup{d}y\ge0,
\end{align*}
since $\lambda_r-\lambda_l\le 0$, $(x+y)-x_0\le 0$ for $y\in[x_0-x,\varepsilon]$ and the assumption on $x$.
Moreover, 
\begin{align*}
 g'(x) 
 &= (\lambda_r-\lambda_l) \int_{[x_0-x,\varepsilon]} \eta_\varepsilon(y)\textup{d}y
  + (\lambda_r-\lambda_l) x \eta_\varepsilon(x_0-x) +(-x)\eta_\varepsilon(x_0-x)\\
 & = (\lambda_r-\lambda_l) \int_{[x_0-x,\varepsilon]} \eta_\varepsilon(y)\textup{d}y <0,
\end{align*} 
with $\lim_{x\downarrow x_0}g(x)=g(x_0)$ and $\lim_{x\uparrow x_0+\varepsilon}g(x)=g(x_0)$. 
In other words, on $[x_0,x_0+\varepsilon]$ the function $g$ attains its maximum at $x_0$. 
\end{enumerate}

Therefore,  the function $g$ is non-negative with  
\begin{align*}
  \sup_{x\ge0} g(x) 
    =\sup_{x_0 \in \{2\}\cup\{2^{k_n}:n\in\mathbb{N}\} } \sup_{x\in (x_0-\varepsilon, x_0+\varepsilon)} |\hat{\upsilon}(x) - \hat{\upsilon}_\varepsilon(x) | 
    =\sup_{x_0 \in \{2\}\cup\{2^{k_n}:n\in\mathbb{N}\} } |\hat{\upsilon}(x_0) - \hat{\upsilon}_\varepsilon(x_0) | 
    <\frac{1}{2^4}.
\end{align*}
\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{lemma}\label{lem:def_q_for_smoothness}
For $p\in(0,2)$, we define 
\begin{align*}
  q:=\frac{4}{p}-1 \text{ and }x_0(p):=\Big(\frac{p}{6(4-p)}\Big)^{\frac{p}{4-2p}}. 
\end{align*}
Then, $x_0(p)\in[0,1]$ and for the function $[0,\frac{3}{2}]\ni x \overset{f}{\mapsto} x^q$, it holds $f'(x_0(p))=\frac{1}{6}$.
\end{lemma}
%
\begin{proof}
It is easily verified that
\begin{align*}
   f'(x_0)=\frac{1}{6}
   \Leftrightarrow q x_0^{q-1}=\frac{1}{6}
   \overset{(q>1)}{\Leftrightarrow} x_0^{q-1}=\frac{1}{6q}
   {\Leftrightarrow} x_0=\Big(\frac{1}{6q}\Big)^{\frac{1}{q-1}} = \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}.
\end{align*}
The point $x_0$ lies, indeed, in the domain of $f$.
In order to prove the last claim, we will initially prove that $(0,2)\ni p\mapsto x_0(p)\in(0,+\infty)$ is a decreasing function.
To this end, we will calculate its derivative, which is given by
\begin{align*}
  x_0'(p)&=x_0(p)\big(\frac{p}{4-2p} \ln(\frac{p}{6(4-p)})\big)'.
\end{align*}
Given that $x_0(p)>0$, for every $p\in(0,2)$, we proceed with the second factor only.
Hence,
\begin{align*}
  \big(\frac{p}{4-2p} \ln(\frac{p}{6(4-p)})\big)' 
  % = \dfrac{\left(p-4\right)\ln\left(\frac{p}{6\left(4-p\right)}\right)+2p-4}{\left(p-4\right)\left(p-2\right)^2}
  = \frac{2\ln(\frac{p}{6(4-p)})(4-p) + 2-p}{2(2-p)^2(4-p)}
\end{align*}
The denominator is positive for every $p\in(0,2)$.
The nominator remains negative in the same region of $p$, since for $p\in(0,2)$ 
\begin{align*}
 2\ln(\frac{p}{6(4-p)})(4-p) + 2-p < 2\ln(\frac{p}{6(4-p)})(4-p) + 4-p
 <(2\ln(\frac{p}{6(4-p)})+1)(4-p)<0.
\end{align*} 

Finally, we compute the limits
\begin{align*}
  \lim_{p\downarrow 0} x_0(p) 
    & = \lim_{p\downarrow 0} \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}}
      = \lim_{p\downarrow 0} \exp\big(\frac{p}{4-2p}\ln(\frac{p}{6(4-p)})\big)\\
    & = \lim_{z\downarrow 0} \exp\big(z\ln(z)\big) = 1
\end{align*}
and 
\begin{align*}
  \lim_{p\uparrow 2} x_0(p) 
    & = \lim_{p\uparrow 2} \big(\frac{p}{6(4-p)}\big)^{\frac{p}{4-2p}} = 0,
\end{align*}
which in conjunction with the monotonicity proved above, verify our claim.
% The last computations will permit us to linearly interpolate, with positive slopes, on the interval $[x_0,2]$.
\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
% \begin{proof}[Proof of \cref{corollary:UI_Young_improvement:StrongerIntegrability}]
%  We will adopt the notation introduced in \cref{lemma:UI_Young_improvement}. 
%  The arguments presented below hold for $p>0$.

%  \vspace{0.5em}
%  For notational convenience we define $\bar{\upsilon}_0=\frac{1}{4},\bar{\upsilon}_{\frac{1}{2}}=\frac{1}{2}$, so that the non-decreasing sequence $(\bar{\upsilon}_n)_{n\in\{0,\frac{1}{2}\}\cup\mathbb{N}}$ associates to the right derivative $\bar{\upsilon}$.
%  In view of the introduced notation, we have 
%  \begin{align*}
%     \overline{\Upsilon}(x)\le 
%     \begin{cases}
%       \bar{\upsilon}_0 x, &\text{for }x\in[0,1]\\
%       \bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}}(x-1), &\text{for }x\in(1,2]\\
%       \bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{k=1}^{n-1}\bar{\upsilon}_k + \bar{\upsilon}_{n}(x-n), &\text{for }x\in(n,n+1]
%     \end{cases}.
%  \end{align*}

%  \vspace{0.5em}
%  Following the arguments of the proof of \cite[Lemme]{meyer1978sur} and modifying them as in the proof of \cref{prop:UI_Young}, we can prove that for the Young function $\overline{\Upsilon}$ associated to the right-derivative $\bar{\upsilon}$, it holds
%  \begin{align}\label{limit:overline_upsilon}
%    \lim_{R\to+\infty}\sup_{\alpha\in\mathcal{A}}\int_{{\{z:|z|>R\}}} \overline{\Upsilon}(|z|^p)m_\alpha(\textup{d}z)=0.
%  \end{align}

%  Indeed, for $c>1$ and $k_0:=\min\{k\in\mathbb{N}  : \bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^k \bar{\upsilon}_q>c\}$
%  \begin{align*}
%    &\int_{\{z:\overline{\Upsilon}(|z|^p)>c\}} \overline{\Upsilon}(|z|^p) m_\alpha (\textup{d}z)
%     \le \sum_{k=k_0}^\infty (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^k \bar{\upsilon}_q) m_\alpha(\{k< |z|^p \le k+1\})\\
%     &\hspace{2em}= (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{k_0} \bar{\upsilon}_q) m_\alpha(\{|z|>k_0\}) + \sum_{k=k_0+1}^\infty \bar{\upsilon}_k m_\alpha(\{|z|^p>k\}).
%     \numberthis \label{ineq:rhs_bar_upsilon}
%  \end{align*}
%  Let us choose an arbitrarily small $\delta>0$.
%  Then, there exists $n_0$ such that for $n\ge n_0\ge 1$ it holds $ \frac{\bar{\upsilon}_n}{\upsilon_n}<\delta$.
%  Bounding the right part of Inequality \eqref{ineq:rhs_bar_upsilon}, we have for $k_0>n_0$\footnote{The reader may observe that $\lim_{c\to+\infty}k_0 = +\infty$.}
%  \begin{align*}
%    &(\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{k_0} \bar{\upsilon}_q) m_\alpha(\{k_0 < |z|^p\le k_0+1\}) + \sum_{k=k_0+1}^\infty \bar{\upsilon}_k m_\alpha(\{k< |z|^p \le k+1\})\\
%     &\hspace{2em}\le (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{n_0} \bar{\upsilon}_q) m_\alpha(\{|z|^p>k_0\}) 
%                       + \delta \sum_{q=n_0+1}^{k_0} \upsilon_q m_\alpha(\{|z|^p>k_0\})
%                       + \delta \sum_{k=k_0+1}^\infty \upsilon_k m_\alpha(\{|z|^p>k\})\\
%     &\hspace{2em}\le (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{n_0} \bar{\upsilon}_q) m_\alpha(\{|z|^p>k_0\}) 
%                       +\delta \sum_{k=n_0+1}^\infty {\upsilon}_k m_\alpha(\{|z|^p>k\}).
%     \numberthis \label{ineq:rhs_limit_k0}
%  \end{align*}
%  From the proofs of \cref{prop:UI_Young} and \cref{lemma:UI_Young_improvement} we have for the sequence $(\upsilon_n)_{n\in\mathbb{N}}$
%   \begin{align*}
%     S:=\sup_{\alpha\in\mathcal{A}} \sum_{n=1}^{\infty}\upsilon_n m_\alpha(\{z:|z|^p>k\}) <+\infty. 
%   \end{align*}
%   In total, in view of \eqref{property:limit_for_UI}, which implies 
%   \begin{align*}
%     \lim_{k\to+\infty} \sup_{\alpha\in\mathcal{A}} m_\alpha(\{z:|z|^p>k\}) = 0,
%   \end{align*}
%   we have from \eqref{ineq:rhs_bar_upsilon}, \eqref{ineq:rhs_limit_k0} and the above limit
%   \begin{align*}
%     &\lim_{R\to+\infty}\sup_{\alpha\in\mathcal{A}}\int_{{\{z:|z|>R\}}} \overline{\Upsilon}(|z|^p)m_\alpha(\textup{d}z) 
%     \le (\bar{\upsilon}_0 + \bar{\upsilon}_{\frac{1}{2}} + \sum_{q=1}^{n_0} \bar{\upsilon}_q) \lim_{k\to+\infty} \sup_{\alpha\in\mathcal{A}} m_\alpha(\{z:|z|^p>k\}) + \delta S=\delta S. 
%   \end{align*}
%   Since $\delta$ was chosen arbitrarily small, we have that the limit on the left hand side of the last inequality is indeed $0$.



%  \vspace{0.5em}
%  In view of the validity of \eqref{limit:overline_upsilon} and recalling \cref{prop:UI_Young}, there exists a Young function $\Psi$ (with right derivative $\psi$) such that 
%  \begin{align*}
%     \sup_{\alpha\in\mathcal{A}}\int_{\{z:|z|\ge 1\}} \Psi\big(\overline{\Upsilon}(|z|^p)\big)m_\alpha (\textup{d}z)<+\infty.
%  \end{align*}
%  Now, observing that $\hat{\upsilon}_\varepsilon(w)<\bar{\upsilon}(w)$, for every $w\ge 2$, we can extract a point $w_0>2$ such that
%   \begin{align*}
%     \Upsilon(w)<\overline{\Upsilon}(w) \text{ for every }w\ge w_0. 
%   \end{align*}  
%  Therefore, we get
%   \begin{align*}
%     &\sup_{\alpha\in\mathcal{A}}\int_{\{z:|z|\ge 1\}} \Psi\big(\Upsilon(|z|^p)\big)m_\alpha (\textup{d}z)\\
%     &\hspace{1em}=\sup_{\alpha\in\mathcal{A}}\Big\{ \int_{\{z:1\le |z|^p\le w_0\}} \Psi\big(\Upsilon(|z|^p)\big)m_\alpha (\textup{d}z) + 
%                                                     \int_{\{z:|z|^p> w_0\}} \Psi\big(\Upsilon(|z|^p)\big)m_\alpha (\textup{d}z)\Big\}\\
%     &\hspace{1em}\le\sup_{\alpha\in\mathcal{A}}\Big\{ \int_{\{z:1\le |z|^p\le w_0\}} \psi\big(\Upsilon(w_0)\big) \Upsilon(|z|^p) m_\alpha (\textup{d}z) + 
%                                                       \int_{\{z:|z|^p> w_0\}} \Psi\big(\overline{\Upsilon}(|z|^p)\big)m_\alpha (\textup{d}z)\Big\}\\
%     &\hspace{1em}\le  \psi\big(\Upsilon(w_0)\big)  
%                       \sup_{\alpha\in\mathcal{A}}  \int_{\{z:|z|\ge 1\}} \Upsilon(|z|^p) m_\alpha (\textup{d}z) + 
%                       \sup_{\alpha\in\mathcal{A}}  \int_{\{z:|z|\ge 1\}} \Psi\big(\overline{\Upsilon}(|z|^p)\big)m_\alpha (\textup{d}z)\Big\}
%     <+\infty.
%   \end{align*}  
%   where we have used that $\Psi(x)\le x\psi(x)$ and $\psi$ is non-decreasing.
% \end{proof}


==> ViscosityFramework.tex <==
%!TEX root = main.tex

% \section{Existence and uniqueness of solutions of nonlocal degenerate elliptic equations}
\section{Hamilton--Jacobi--Bellman Equations}\label{sec:HJB_Equations}

\begin{definition}[Regularity Condition]\label{def:regularity_condition}
  Suppose that $p>0$ and $T>0$, that $u_i^\varepsilon\in \textup{USC}_p([0,T]\times \mathbb{R}^d)$ is the supremal convolution in space of some $u_i\in \textup{USC}_p([0,T]\times \mathbb{R}^d)$ for $\varepsilon>0$ and $i\in\{1,\ldots,k\}$ with $k\in\mathbb{N}$, and that 
  \begin{align*}
    \phi_\gamma^\lambda(t,x) := \frac{\delta}{T-t} + \lambda \sum_{i<j} |x_i-x_j|^2 + \gamma e^{\mu t}\sum_{i=1}^k \Upsilon(|x_i|^p)
  \end{align*}
  for $(t,x):=(t,x_1,\ldots,x_k)\in[0,T)\times\mathbb{R}^{kd}$ with $\gamma,\delta,\mu,\lambda \ge 0$ and $\Upsilon$ a twice continuously differentiable Young function.
  A family of operators 
  \begin{align*}
    G_i:(0,T)\times \mathbb{R}^d \times \mathbb{R} \times \mathbb{R}^d \times \mathbb{S}^{d\times d}\times C^2_p(\mathbb{R}^d)\longrightarrow \mathbb{R}
  \end{align*}
  for $i\in\{1,\ldots,k\}$ satisfies a regularity condition for $\beta_,\ldots,\beta_k>0$, if there exists $C'>0$ and $\omega:[0,+\infty)\rightarrow [0,+\infty)$ with $\lim_{t\downarrow 0}\omega(t) = \omega(0)=0$ such that the following implication holds:

  If the function 
  \begin{align*}
    (0,T)\times\mathbb{R}^{kd}\ni (t,x) = (t,x_1,\ldots,x_k)\longmapsto \sum_{i=1}^k\beta_i u_i^\varepsilon(t,x_i) - \phi_\gamma^\lambda(t,x),
  \end{align*}
  has a global maximum in $(\bar{t},\bar{x})=(\bar{t}^{(\gamma,\lambda,\varepsilon)},\bar{x}^{(\gamma,\lambda,\varepsilon)})\in(0,T)\times \mathbb{R}^{kd}$ with
  \begin{align*}
    \sup_{(t,x)\in(0,T)\times \mathbb{R}^{kd}} \bigg(\sum_{i=1}^k\beta_i u_i^\varepsilon(t,x_i) - \phi_\gamma^\lambda(t,x)\bigg) = \sum_{i=1}^k\beta_i u_i^\varepsilon(\bar{t},\bar{x}_i) - \phi_\gamma^\lambda(\bar{t},\bar{x})\ge0
  \end{align*}
  and if $X_i = X_i^{(\gamma,\lambda,\varepsilon)}\in\mathbb{S}^{d\times d}$ for $i\in\{1,\ldots,k\}$ satisfy
  \begin{align*}
    &\textup{diag}(X_1,\ldots,X_k)
      \le 4\lambda J_{k,d}\\ 
        &\hspace{2em}+ C'\gamma e^{\mu t}\textup{diag}\left[
              (\Upsilon''(|\bar{x}_1|^{p}) |\bar{x}_1|^{p}+\Upsilon'(|\bar{x}_1|^{p} )) |\bar{x}_1|^{p-2} I,
                \ldots, 
              (\Upsilon''(|\bar{x}_k|^{p}) |\bar{x}_k|^{p}+\Upsilon'(|\bar{x}_k|^{p} ) |\bar{x}_k|^{p-2} I
            \right],
  \end{align*}
  then the following inequality holds in the ordinary sense
  \begin{align*}
    &-\sum_{i=1}^k \beta_i \triangle_\phi^\varepsilon [G^\kappa_i]\big(\bar{t}\bar{x}_i,u_i^\varepsilon(\bar{t},\bar{x}_i),\beta_i^{-1}D_{x_i}\phi_\gamma^\lambda(\bar{t},\bar{x}),X_i,u_i^\varepsilon(\bar{t},\cdot), \beta_i^{-1}\phi_\gamma^\lambda(\bar{t},\bar{x}_1,,\ldots,\bar{x}_{i-1},\cdot,\bar{x}_{i+1},\ldots,\bar{x}_\big)\\
    &\le \omega\bigg(\Big(\sum_{i<j}|x_i-x_j|\Big)\Big(1+\sum_{i=1}^k |\bar{x}_i|^p\Big)\bigg)
          +C'\lambda \sum_{i<j}|\bar{x}_i - \bar{x}_j|^2 
          +C' \gamma e^{\mu t}\Big(1 + \sum_{i=1}^k \Upsilon(|\bar{x}_i|^p)\Big) 
          +\varrho_{\gamma,\lambda,\varepsilon,\kappa}
  \end{align*}
  for a remainder $\varrho_{\gamma,\lambda,\varepsilon,\kappa}$ with
  \begin{align*}
    \limsup_{\gamma \downarrow 0} \limsup_{\lambda\to+\infty}\limsup_{\varepsilon\downarrow 0}\limsup_{\kappa\downarrow 0}\varrho_{\gamma,\lambda,\varepsilon,\kappa}\le 0.
  \end{align*}
\end{definition}




\begin{definition}[Hamilton--Jacobi--Bellman Equations]\label{def:HJB}
A nonlinear, parabolic,second-order nonlocal equation in $(0,T)\times\mathbb{R}^d$ with time horizon $T>0$
\begin{align}\label{equation:HJB}
\partial_t u (t,x) + G\left(t,x,u (t,x),Du (t,x),D^2u (t,x),u (t,\cdot)\right)
\tag{HJB}
\end{align}
is called \emph{Hamilton--Jacobi--Bellman equation} (or HJB equation  for short) if 
\begin{gather*}
G(t,x,r,p,X,\phi) = G^\kappa (t,x,r,p,X,\phi,\phi)\\ 
G^\kappa(t,x,r,p,X,u,\phi) = \inf_{\alpha\in\mathcal{A}} G_\alpha^\kappa (t,x,r,p,X,u,\phi)
\end{gather*}
for a family $(G_\alpha^\kappa(t,x,r,p,X,u,\phi,))_{\alpha\in\mathcal{A}}$ of linear operators
\begin{align*}
  G^\kappa_\alpha :(0,T)\times \mathbb{R}^d\times \mathbb{R}\times \mathbb{R}^d\times \mathbb{S}^{d\times d}\times \textup{SC}_p(\mathbb{R}^d) \times C^2(\mathbb{R}^d) \longrightarrow \mathbb{R}
\end{align*}
with $p\ge 1$ and $0<\kappa<1$ of the form
\begin{align*}
G_\alpha^\kappa(t,x,r,p,X,u,\phi) 
  &= f_\alpha(t,x) - \mathcal{L}_\alpha(t,x,r,p,X) 
    - \mathcal{I}_\alpha^\kappa(t,x,u,\phi)\\
\mathcal{L}_\alpha(t,x,r,p,X) 
  & =c_\alpha(t,x)r + b_\alpha^T(t,x)p 
    + \textup{tr}\left(\sigma_\alpha(t,x)\sigma^T(t,x)X\right)\\
\mathcal{I}_\alpha^\kappa(t,x,u,\phi) 
  & =\check{\mathcal{I}}_\alpha^\kappa(t,x,\phi) 
    + \overline{\mathcal{I}}_\alpha^\kappa(t,x,u,\phi) 
    +\hat{\mathcal{I}}_\alpha (t,x,u,\phi),
\end{align*}
where $f_\alpha(t,x)$, $c_\alpha(t,x)\in\mathbb{R}$, $b_\alpha(t,x)\in\mathbb{R}^d$, $\sigma_\alpha\in\mathbb{S}^{d\times d}$ and 
\begin{align*}
  \check{\mathcal{I}}_\alpha^\kappa(t,x,\phi) 
    &:= \int_{\{z:|z|\le \kappa\}} \left(\phi(x+j_\alpha(t,x,z))-\phi(t,x) - D\phi(x)j_\alpha(t,x,z)\right) m_\alpha(\textup{d}z)   \\
  \overline{\mathcal{I}}_\alpha^\kappa(t,x,u,\phi) 
    &:= \int_{\{z:\kappa\le |z|\le 1\}} \left(u(x+j_\alpha(t,x,z))-u(t,x) - D\phi(x)j_\alpha(t,x,z)\right) m_\alpha(\textup{d}z) \\
  \hat{\mathcal{I}}_\alpha (t,x,u,\phi) 
    &:=\int_{\{z:1\le |z|\}} \left(u(x+j_\alpha(t,x,z))-u(t,x) - D\phi(x)j_\alpha(t,x,z)\right) m_\alpha(\textup{d}z) 
\end{align*}
with Borel measures $m_\alpha:\mathcal{B}(\mathbb{R}^d)\rightarrow [0,+\infty)$ and $j_\alpha(t,x,z)\in\mathbb{R}^d$.
\end{definition}
% 
% 
% 
% 
% 
% 
\begin{remark}
  We have slightly deviated from the classical definition of the HJB operator by allowing the presence of the term $D\psi(x)j_\alpha(t,x,z)$ in the segment $\hat{\mathcal{I}}_\alpha$ of the nonlocal part of the operator.
  Comparing to the classical case, which uses $\mathds{1}_{\{z:|z|\le 1\}}$ as truncation function, we use instead the identity.  
  The reason is that we are mainly interested in the case where the linear operators $G_\alpha^\kappa$ are operators associated to integrable martingales when $j_\alpha(t,x,\cdot)=\textup{Id}$, for $\textup{Id}$ the identtity on $\mathbb{R}$ \emph{i.e.}, the motivation comes from the probabilistic interpretation of the nonlocal operator.
  However, we will demonstrate how the use of Young functions can also be applied to the classical case, \emph{i.e.}, when the truncation function $\mathds{1}_{\{z:|z|\le 1\}}$ is used, which associates to semimartingales.
\end{remark}
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
\begin{assumption}[on HJB Coefficients]\label{assumption:HJB_coefficients_assumption}
Suppose that $(G_\alpha)_{\alpha\in\mathcal{A}}$ is a family of Hamilton--Jacobi--Bellman operators as defined in \cref{def:HJB} with $p\ge 1$ and $T>0$.
Throughout this section we will assume that the following condition hold:
\begin{enumerate}[label=(B\arabic*)]
  \item\label{HJB:coeff_boundedness} (Boundedness) 
    The coefficients of the local part are bounded
    \begin{align*}
      \sup_{\alpha\in\mathcal{A}}\left(|f_\alpha(t,x)|+|c_\alpha(t,x)| + |b_\alpha(t,x)|+|\sigma_\alpha(t,x)|\right)<+\infty
    \end{align*}
    in every $(t,x)\in(0,T)\times \mathbb{R}^d$, and the family of measures of the nonlocal part meet
    \begin{align*}
      \sup_{\alpha \in\mathcal{A}} \int_{\mathbb{R}^d}\left(|z|^2\mathds{1}_{\{z:|z|\le 1\}}(z) + |z|^p\mathds{1}_{\{z:|z|>1\}}(z)\right) m_\alpha(\textup{d}z)<+\infty.
    \end{align*} 


  \item\label{HJB:UI} (Uniform integrability) The family of measures of the nonlocal part satisfies
    \begin{align*}
      \lim_{\kappa\downarrow 0}\sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|\le \kappa\}} = 0 =\lim_{R\to+\infty} \sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|>R\}} |z|^pm_\alpha(\textup{d}z). 
    \end{align*}


  \item\label{HJB:coef_continuity} (Continuity)
    There exists a constant $C>0$ and a function $\omega:\mathbb{R}_+\rightarrow \mathbb{R}_+$ with $\omega(0)=\lim_{h\downarrow 0}\omega(h)=0$ such that 
    \begin{align*}
      \sup_{\alpha\in\mathcal{A}} \left( |\sigma_\alpha(t,x) - \sigma_\alpha(s,y)| + |b_\alpha(t,x) - b_\alpha(s,y)| \right) &\le \omega(|t-s|)+C|x-y|\\
      \sup_{\alpha\in\mathcal{A}} \left( |f_\alpha(t,x) - f_\alpha(s,y)| + |c_\alpha(t,x) - c_\alpha(s,y)| \right) &\le \omega(|t-s|)+\omega(|x-y|)\\
      \sup_{\alpha\in\mathcal{A}}  |j_\alpha(t,x,z) - j_\alpha(s,y,z)|  &\le |z|\left(\omega(|t-s|)+C|x-y|\right)
    \end{align*}
    for all $t,s\in(0,T)$ and $x,y,z\in\mathbb{R}^d$.


  \item\label{HJB:jump_at_most_linear} (Growth condition) The jump-height coefficients of the nonlocal part have at most linear grwoth in space, \emph{i.e.}, there exists $C>0$ such that
      \begin{align*}
        \sup_{\alpha\in\mathcal{A}}  |j_\alpha(t,x,z)|\le C(1+|x|)|z|
      \end{align*}
      for all $t\in(0,T)$ and $x,z\in\mathbb{R}^d$.


  \item\label{HJB:c_non-positive} (Non-positiveness) The codomain coefficients are non-positive
      \begin{align*}
        \sup_{\alpha\in\mathcal{A}}c_\alpha(t,x)\le 0
      \end{align*}
      for all $t\in(0,T)$ and $x\in \mathbb{R}^d$.
\end{enumerate}
\end{assumption}


\begin{remark}\label{remark:explanation_for_regularity_condition}
Let us compare the presented framework with that adopted in \citet[Definition 2.21, Definition 2.27, Remark 2.28]{Hollender2017}.
In particular, we will argue that the regularity condition required in \cref{def:regularity_condition} is significantly weaker than \citet[Definition 2.21]{Hollender2017}, thus allowing us to use sharp integrability conditions as well as to consider all the cases which were previously excluded.
\begin{enumerate}
  \item We can recover the regularity condition used in \citet[Definition 2.21]{Hollender2017} from \cref{def:regularity_condition} by using the Young function $\Upsilon$, where 
  \begin{align*}
    \Upsilon(y):=y^{\frac{q}{p}}, \text{ for }y\ge 0, q>p \text{ and }q\ge 2.
  \end{align*}
  The reader should pay attention to the fact that the restriction $q\ge 2$ can be disregarded under the framework adopted in the current work, allowing thus considering a family of measures for which 
  \begin{align*}
    \sup_{\alpha\in\mathcal{A}} \int_{\{z:|z|^p>1\}} |z|^p m_{\alpha}(\textup{d}z) <+\infty, \text{ for }0<p<q\le 2.
  \end{align*} 
  These cases have been excluded in \citet{Hollender2017}.
  Additionally, we will see in the next remarks that \cref{def:regularity_condition} allows for sharp choices, namely, we will not need the presence of the auxiliary power $q$.  
  \item Following the notation introduced  in the previous remark, the conditions on $q$ required in \citet[Definition 2.21]{Hollender2017}, \emph{i.e.}, $q>p$ and $q\ge 2$, dictate the use of a family of measures which are at least square integrable on $\{z:|z|>1\}$.
  Naturally, one would require the value $q$ to be ``as close to $p$ as possible'', \emph{i.e.}, $q=p+\delta$ for $\delta >0$ and arbitrarily small.
  These natural assumptions allow us to assume that $q<2p$.
  In this case, we have that $\Upsilon'(y) =\frac{q}{p} y^{\frac{q}{p}-1}$ with $\frac{q}{p}-1>0$ and $\Upsilon''(y) = \frac{q}{p} (\frac{q}{p}-1) y^{\frac{q}{p}-2}$, with $\frac{q}{p}-2<0$. 
  In other words, we have the following properties (for $w=w(z)=x+j_\alpha(t,x,z)$, where $t\in(0,T),x\in\mathbb{R}^d$ may be assumed fixed for simplicity)
  \begin{align*}
    \Upsilon'(|w|^p) |w|^{p-2} = C |w|^{q-2} \text{ and }
    \big[\Upsilon''(|w|^p) |w|^{p}\big] |w|^{p-2}= C|w|^{q-2} \text{ for }z\in\mathbb{R}^d,
  \end{align*}
  with $q-2\ge 0$ and $q-p>0$ and some $C>0$.
  These quantities appear in the computation of the second derivative of the function $\mathbb{R}^d \ni y\mapsto |y|^q$, once we require a representation of it in terms of $|y|^{p-2}$.
  Thus, examining the regularity condition described in \cref{def:regularity_condition}, the terms $\Upsilon'(|z|^p)$ and $\Upsilon''(|z|^p) |z|^{p}$ naturally appear in the block diagonal form of the upper bound of the second derivative of $\phi_\gamma^\lambda$.

  Returning to \citet[Definition 2.21]{Hollender2017}, these additional terms are innocuous given that $q\ge 2$.
  Indeed,  in the case $\Upsilon(y)=y^{\frac{q}{p}}$,
   % since $\frac{q}{p}-2<0\Leftrightarrow q<2p$, 
  \begin{align*}
      \Upsilon''(|w|^p) |w|^{2p-2} = |w|^{q-2} \text{ for }w\in\mathbb{R}^d
  \end{align*}
  and 
  \begin{align*}
      \Upsilon'(|w|^p) |w|^{p-2} = |w|^{q-2} \text{ for }w\in\mathbb{R}^d.
  \end{align*}
  However, when $p\in(0,2)$ the limits 
  \begin{align*}
      \liminf_{|w|\to 0}\Upsilon'(|w|^p) |w|^{p-2}  \text{ and }
      \liminf_{|w|\to 0}\Upsilon''(|w|^p) |w|^{2p-2}
  \end{align*}
  may pose unwanted inconveniences.

  In order to remedy all the aforementioned special cases, will prove that the Young function may be chosen to possess nice properties.
  The problematic situations stemmed from the fact that we restricted ourselves in Young functions in power form.
  Since there are plenty of Young functions which grow slower than any power function, the challenge is to choose a twice continuously differentiable young function $\Upsilon$ for which there exists $C>0$ such that
  \begin{align*}
      0< x\Upsilon''(x) <C, \text{ for }x>1
  \end{align*} 
  and
  \begin{gather*}
      \lim_{x\downarrow 0} \Upsilon''(x^p)x^{2p-2}
      = \lim_{x\downarrow 0} \Upsilon'(x^p)x^{p-2} 
      = 0 
  \end{gather*}

  It is \cref{lemma:UI_Young_improvement} which verifies that this is possible, while the Young function possesses additional useful properties which further allow recovering the initially assumed integrability condition.

  \item \Cref{assumption:HJB_coefficients_assumption} is identical to \citet[Remark 2.28]{Hollender2017}.
  However, in \cite{Hollender2017} when the author is called to prove that the HJB operators satisfy the regularity condition \cite[Definition 2.21]{Hollender2017}, see \cite[Proposition 2.33]{Hollender2017}, the presence of the auxiliary power $q\ge 2$ is needed, requiring thus stronger integrability properties for the family of Borel measures $(m_\alpha)_{\alpha\in\mathcal{A}}$. 
  In the current work, this gap is bridged, since no additional condition is required for proving that the HJB operator satisfies the regularity condition described in \cref{def:regularity_condition}. 
  % Of course, one can easily verify that the ``classical'' HJB operator, \emph{i.e.}, without the presence of $D\phi(x)j_\alpha(t,x,z)$ in the $\hat{\mathcal{I}}_\alpha$ segment of the nonlocal part for every $\alpha\in\mathcal{A}$, verifies the regularity condition described in \cref{def:regularity_condition}. 

  \item We describe the Condition \ref{HJB:UI} as ``uniform integrability'' instead of ``tightness'', as we prefer to interpret these conditions as the property of the family of measures to uniformly integrate the tails of the functions $\mathbb{R}^d\ni z\mapsto |z|^2$ and $\mathbb{R}^d\ni z\mapsto |z|^p$ on the respective domains. 
  The notion of tightness can be also used to describe the property that the family 
  $(\{|z|^2\mathds{1}_{\{z:|z|\le 1\}} + |z|^p\mathds{1}_{\{z:|z|>1\}}\}m_\alpha(\textup{d}z) )_{\alpha\in\mathcal{A}}$ is tight, but -given the nature of the framework- it is regarded misleading.  
\end{enumerate}
\end{remark}

